Privacy Preference Signals: Past, Present and Future

Privacy preference signals are digital representations of how users want their personal data to be processed. Such signals must be adopted by both the sender (users) and intended recipients (data processors). Adoption represents a coordination problem that remains unsolved despite efforts dating back to the 1990s. Browsers implemented standards like the Platform for Privacy Preferences (P3P) and Do Not Track (DNT), but vendors profiting from personal data faced few incentives to receive and respect the expressed wishes of data subjects. In the wake of recent privacy laws, a coalition of AdTech firms published the Transparency and Consent Framework (TCF), which defines an opt-in consent signal. This paper integrates post-GDPR developments into the wider history of privacy preference signals. Our main contribution is a high-frequency longitudinal study describing how TCF signal gained dominance as of February 2021. We explore which factors correlate with adoption at the website level. Both the number of third parties on a website and the presence of Google Ads are associated with higher adoption of TCF. Further, we show that vendors acted as early adopters of TCF 2.0 and provide two case-studies describing how Consent Management Providers shifted existing customers to TCF 2.0. We sketch ways forward for a pro-privacy signal.

==> data/gvl/gvl_switch/stacked/v1.tex <==
\draw (18.2959, 14) -- (18.3151, 37) -- (18.3342, 75) -- (18.3534, 113) -- (18.3726, 166) -- (18.3918, 258) -- (18.411, 297) -- (18.4301, 322) -- (18.4493, 338) -- (18.4685, 353) -- (18.4877, 370) -- (18.5068, 376) -- (18.526, 389) -- (18.5452, 394) -- (18.5644, 406) -- (18.5836, 409) -- (18.6027, 414) -- (18.6219, 422) -- (18.6411, 425) -- (18.6603, 428) -- (18.6795, 429) -- (18.6986, 433) -- (18.7178, 435) -- (18.737, 440) -- (18.7562, 442) -- (18.7753, 448) -- (18.7945, 448) -- (18.8137, 449) -- (18.8329, 453) -- (18.8521, 455) -- (18.8712, 456) -- (18.8904, 458) -- (18.9096, 459) -- (18.9288, 460) -- (18.9479, 460) -- (18.9671, 461) -- (18.9863, 462) -- (19.0055, 462) -- (19.0247, 464) -- (19.0438, 466) -- (19.063, 469) -- (19.0822, 470) -- (19.1014, 472) -- (19.1205, 476) -- (19.1397, 479) -- (19.1589, 484) -- (19.1781, 486) -- (19.1973, 488) -- (19.2164, 490) -- (19.2356, 490) -- (19.2548, 495) -- (19.274, 496) -- (19.2932, 500) -- (19.3123, 500) -- (19.3315, 502) -- (19.3507, 504) -- (19.3699, 509) -- (19.389, 508) -- (19.4082, 509) -- (19.4274, 509) -- (19.4466, 511) -- (19.4658, 510) -- (19.4849, 508) -- (19.5041, 507) -- (19.5233, 510) -- (19.5425, 515) -- (19.5616, 512) -- (19.5808, 514) -- (19.6, 509) -- (19.6192, 506) -- (19.6384, 504) -- (19.6575, 502) -- (19.6767, 502) -- (19.6959, 499) -- (19.7151, 486) -- (19.7342, 480) -- (19.7534, 465) -- (19.7726, 455) -- (19.7918, 453) -- (19.811, 453) -- (19.8301, 452) -- (19.8493, 447) -- (19.8685, 449) -- (19.8877, 443) -- (19.9068, 441) -- (19.926, 442) -- (19.9452, 435) -- (19.9644, 432) -- (19.9836, 426) -- (20.0027, 427) -- (20.0219, 425) -- (20.041, 423) -- (20.0601, 419) -- (20.0792, 410) -- (20.0984, 405) -- (20.1175, 387) -- (20.1366, 376) -- (20.1557, 361) -- (20.1749, 353) -- (20.194, 339) -- (20.2131, 330) -- (20.2322, 315) -- (20.2514, 286) -- (20.2705, 277) -- (20.2896, 272) -- (20.3087, 263) -- (20.3279, 250) -- (20.347, 230) -- (20.3661, 220) -- (20.3852, 210) -- (20.4044, 203) -- (20.4235, 191) -- (20.4426, 181) -- (20.4617, 174) -- (20.4809, 164) -- (20.5, 151) -- (20.5191, 139) -- (20.5383, 134) -- (20.5574, 113) -- (20.5765, 99) -- (20.5956, 87) -- (20.6148, 73) -- (20.6339, 64) -- (20.653, 61) -- (20.6721, 60) -- (20.6913, 58) -- (20.7104, 56) -- (20.7295, 55) -- (20.7486, 49) -- (20.7678, 46) -- (20.7869, 45) -- (20.806, 46) -- (20.8251, 45) -- (20.8443, 46) -- (20.8634, 45) -- (20.8825, 46) -- (20.9016, 45) -- (20.9208, 45) -- (20.9399, 45) -- (20.959, 45) -- (20.9781, 44) -- (20.9973, 44) -- (21.0164, 44) -- (21.0356, 43) -- (21.0548, 43) -- (21.074, 43) -- (21.0932, 43) -- (21.1123, 43) -- (21.1315, 40) -- (21.1315, 0) -- (18.2959, 0) -- cycle;

==> data/gvl/gvl_switch/stacked/v2-new.tex <==
\draw (18.2959, 14) -- (18.3151, 37) -- (18.3342, 75) -- (18.3534, 113) -- (18.3726, 166) -- (18.3918, 258) -- (18.411, 297) -- (18.4301, 322) -- (18.4493, 338) -- (18.4685, 353) -- (18.4877, 370) -- (18.5068, 376) -- (18.526, 389) -- (18.5452, 394) -- (18.5644, 406) -- (18.5836, 409) -- (18.6027, 414) -- (18.6219, 422) -- (18.6411, 425) -- (18.6603, 428) -- (18.6795, 429) -- (18.6986, 433) -- (18.7178, 435) -- (18.737, 440) -- (18.7562, 442) -- (18.7753, 448) -- (18.7945, 448) -- (18.8137, 449) -- (18.8329, 453) -- (18.8521, 455) -- (18.8712, 456) -- (18.8904, 458) -- (18.9096, 459) -- (18.9288, 460) -- (18.9479, 460) -- (18.9671, 461) -- (18.9863, 462) -- (19.0055, 462) -- (19.0247, 464) -- (19.0438, 466) -- (19.063, 469) -- (19.0822, 470) -- (19.1014, 472) -- (19.1205, 476) -- (19.1397, 479) -- (19.1589, 484) -- (19.1781, 486) -- (19.1973, 488) -- (19.2164, 490) -- (19.2356, 490) -- (19.2548, 495) -- (19.274, 496) -- (19.2932, 500) -- (19.3123, 500) -- (19.3315, 502) -- (19.3507, 504) -- (19.3699, 509) -- (19.389, 508) -- (19.4082, 509) -- (19.4274, 509) -- (19.4466, 511) -- (19.4658, 510) -- (19.4849, 508) -- (19.5041, 507) -- (19.5233, 510) -- (19.5425, 515) -- (19.5616, 512) -- (19.5808, 514) -- (19.6, 509) -- (19.6192, 506) -- (19.6384, 504) -- (19.6575, 502) -- (19.6767, 502) -- (19.6959, 499) -- (19.7151, 494) -- (19.7342, 496) -- (19.7534, 488) -- (19.7726, 490) -- (19.7918, 492) -- (19.811, 495) -- (19.8301, 495) -- (19.8493, 498) -- (19.8685, 505) -- (19.8877, 506) -- (19.9068, 510) -- (19.926, 511) -- (19.9452, 514) -- (19.9644, 516) -- (19.9836, 514) -- (20.0027, 515) -- (20.0219, 517) -- (20.041, 519) -- (20.0601, 516) -- (20.0792, 518) -- (20.0984, 520) -- (20.1175, 522) -- (20.1366, 524) -- (20.1557, 527) -- (20.1749, 529) -- (20.194, 531) -- (20.2131, 535) -- (20.2322, 538) -- (20.2514, 539) -- (20.2705, 543) -- (20.2896, 544) -- (20.3087, 541) -- (20.3279, 543) -- (20.347, 544) -- (20.3661, 544) -- (20.3852, 546) -- (20.4044, 547) -- (20.4235, 549) -- (20.4426, 550) -- (20.4617, 549) -- (20.4809, 551) -- (20.5, 551) -- (20.5191, 550) -- (20.5383, 554) -- (20.5574, 547) -- (20.5765, 554) -- (20.5956, 558) -- (20.6148, 567) -- (20.6339, 575) -- (20.653, 578) -- (20.6721, 584) -- (20.6913, 596) -- (20.7104, 607) -- (20.7295, 619) -- (20.7486, 624) -- (20.7678, 633) -- (20.7869, 641) -- (20.806, 649) -- (20.8251, 652) -- (20.8443, 659) -- (20.8634, 664) -- (20.8825, 666) -- (20.9016, 670) -- (20.9208, 673) -- (20.9399, 673) -- (20.959, 677) -- (20.9781, 679) -- (20.9973, 681) -- (21.0164, 684) -- (21.0356, 686) -- (21.0548, 691) -- (21.074, 694) -- (21.0932, 700) -- (21.1123, 707) -- (21.1315, 710) -- (21.1315, 0) -- (18.2959, 0) -- cycle;

==> data/gvl/gvl_switch/stacked/v2-switch.tex <==
\draw (18.2959, 14) -- (18.3151, 37) -- (18.3342, 75) -- (18.3534, 113) -- (18.3726, 166) -- (18.3918, 258) -- (18.411, 297) -- (18.4301, 322) -- (18.4493, 338) -- (18.4685, 353) -- (18.4877, 370) -- (18.5068, 376) -- (18.526, 389) -- (18.5452, 394) -- (18.5644, 406) -- (18.5836, 409) -- (18.6027, 414) -- (18.6219, 422) -- (18.6411, 425) -- (18.6603, 428) -- (18.6795, 429) -- (18.6986, 433) -- (18.7178, 435) -- (18.737, 440) -- (18.7562, 442) -- (18.7753, 448) -- (18.7945, 448) -- (18.8137, 449) -- (18.8329, 453) -- (18.8521, 455) -- (18.8712, 456) -- (18.8904, 458) -- (18.9096, 459) -- (18.9288, 460) -- (18.9479, 460) -- (18.9671, 461) -- (18.9863, 462) -- (19.0055, 462) -- (19.0247, 464) -- (19.0438, 466) -- (19.063, 469) -- (19.0822, 470) -- (19.1014, 472) -- (19.1205, 476) -- (19.1397, 479) -- (19.1589, 484) -- (19.1781, 486) -- (19.1973, 488) -- (19.2164, 490) -- (19.2356, 490) -- (19.2548, 495) -- (19.274, 496) -- (19.2932, 500) -- (19.3123, 500) -- (19.3315, 502) -- (19.3507, 504) -- (19.3699, 509) -- (19.389, 508) -- (19.4082, 509) -- (19.4274, 509) -- (19.4466, 511) -- (19.4658, 510) -- (19.4849, 508) -- (19.5041, 507) -- (19.5233, 510) -- (19.5425, 515) -- (19.5616, 512) -- (19.5808, 514) -- (19.6, 509) -- (19.6192, 506) -- (19.6384, 504) -- (19.6575, 502) -- (19.6767, 502) -- (19.6959, 499) -- (19.7151, 494) -- (19.7342, 496) -- (19.7534, 488) -- (19.7726, 490) -- (19.7918, 492) -- (19.811, 494) -- (19.8301, 494) -- (19.8493, 496) -- (19.8685, 502) -- (19.8877, 503) -- (19.9068, 506) -- (19.926, 507) -- (19.9452, 510) -- (19.9644, 512) -- (19.9836, 510) -- (20.0027, 511) -- (20.0219, 512) -- (20.041, 513) -- (20.0601, 510) -- (20.0792, 511) -- (20.0984, 512) -- (20.1175, 514) -- (20.1366, 516) -- (20.1557, 518) -- (20.1749, 520) -- (20.194, 522) -- (20.2131, 525) -- (20.2322, 527) -- (20.2514, 527) -- (20.2705, 529) -- (20.2896, 530) -- (20.3087, 527) -- (20.3279, 528) -- (20.347, 529) -- (20.3661, 529) -- (20.3852, 530) -- (20.4044, 531) -- (20.4235, 532) -- (20.4426, 531) -- (20.4617, 530) -- (20.4809, 530) -- (20.5, 529) -- (20.5191, 525) -- (20.5383, 526) -- (20.5574, 517) -- (20.5765, 517) -- (20.5956, 516) -- (20.6148, 520) -- (20.6339, 522) -- (20.653, 522) -- (20.6721, 522) -- (20.6913, 522) -- (20.7104, 522) -- (20.7295, 524) -- (20.7486, 525) -- (20.7678, 526) -- (20.7869, 526) -- (20.806, 527) -- (20.8251, 527) -- (20.8443, 527) -- (20.8634, 527) -- (20.8825, 527) -- (20.9016, 527) -- (20.9208, 527) -- (20.9399, 527) -- (20.959, 527) -- (20.9781, 527) -- (20.9973, 527) -- (21.0164, 527) -- (21.0356, 527) -- (21.0548, 527) -- (21.074, 528) -- (21.0932, 529) -- (21.1123, 529) -- (21.1315, 529) -- (21.1315, 0) -- (18.2959, 0) -- cycle;

==> data/gvl/heatmap.tex <==
\heatmapGvl{18.3041}{0}
\heatmapGvl{18.3233}{0}
\heatmapGvl{18.3425}{0}
\heatmapGvl{18.3616}{0}
\heatmapGvl{18.3808}{0}
\heatmapGvl{18.4}{0}
\heatmapGvl{18.4192}{0}
\heatmapGvl{18.4384}{0}
\heatmapGvl{18.4575}{0}
\heatmapGvl{18.4767}{0}
\heatmapGvl{18.4959}{0}
\heatmapGvl{18.5151}{0}
\heatmapGvl{18.5342}{0}
\heatmapGvl{18.5534}{0}
\heatmapGvl{18.5726}{0}
\heatmapGvl{18.5918}{0}
\heatmapGvl{18.611}{0}
\heatmapGvl{18.6301}{0}
\heatmapGvl{18.6493}{0}
\heatmapGvl{18.6685}{0}
\heatmapGvl{18.6877}{0}
\heatmapGvl{18.7068}{0}
\heatmapGvl{18.726}{0}
\heatmapGvl{18.7452}{0}
\heatmapGvl{18.7644}{0}
\heatmapGvl{18.7836}{0}
\heatmapGvl{18.8027}{0}
\heatmapGvl{18.8219}{0}
\heatmapGvl{18.8411}{0}
\heatmapGvl{18.8603}{0}
\heatmapGvl{18.8795}{0}
\heatmapGvl{18.8986}{0}
\heatmapGvl{18.9178}{0}
\heatmapGvl{18.937}{0}
\heatmapGvl{18.9562}{0}
\heatmapGvl{18.9753}{0}
\heatmapGvl{18.9945}{0}
\heatmapGvl{19.0137}{0}
\heatmapGvl{19.0329}{0}
\heatmapGvl{19.0521}{0}
\heatmapGvl{19.0712}{0}
\heatmapGvl{19.0904}{0}
\heatmapGvl{19.1096}{0}
\heatmapGvl{19.1288}{0}
\heatmapGvl{19.1479}{0}
\heatmapGvl{19.1671}{0}
\heatmapGvl{19.1863}{0}
\heatmapGvl{19.2055}{0}
\heatmapGvl{19.2247}{0}
\heatmapGvl{19.2438}{0}
\heatmapGvl{19.263}{0}
\heatmapGvl{19.2822}{0}
\heatmapGvl{19.3014}{0}
\heatmapGvl{19.3205}{0}
\heatmapGvl{19.3397}{0}
\heatmapGvl{19.3589}{0}
\heatmapGvl{19.3781}{0}
\heatmapGvl{19.3973}{0}
\heatmapGvl{19.4164}{0}
\heatmapGvl{19.4356}{0}
\heatmapGvl{19.4548}{0}
\heatmapGvl{19.474}{0}
\heatmapGvl{19.4932}{0}
\heatmapGvl{19.5123}{0}
\heatmapGvl{19.5315}{0}
\heatmapGvl{19.5507}{0}
\heatmapGvl{19.5699}{0}
\heatmapGvl{19.589}{0}
\heatmapGvl{19.6082}{0}
\heatmapGvl{19.6274}{0}
\heatmapGvl{19.6466}{0}
\heatmapGvl{19.6658}{0}
\heatmapGvl{19.6849}{0}
\heatmapGvl{19.7041}{0}
\heatmapGvl{19.7233}{0.0161943}
\heatmapGvl{19.7425}{0.0322581}
\heatmapGvl{19.7616}{0.0471311}
\heatmapGvl{19.7808}{0.0714286}
\heatmapGvl{19.8}{0.0792683}
\heatmapGvl{19.8192}{0.0848485}
\heatmapGvl{19.8384}{0.0868687}
\heatmapGvl{19.8575}{0.10241}
\heatmapGvl{19.8767}{0.110891}
\heatmapGvl{19.8959}{0.124506}
\heatmapGvl{19.9151}{0.135294}
\heatmapGvl{19.9342}{0.135029}
\heatmapGvl{19.9534}{0.153696}
\heatmapGvl{19.9726}{0.162791}
\heatmapGvl{19.9918}{0.171206}
\heatmapGvl{20.0109}{0.170874}
\heatmapGvl{20.0301}{0.17795}
\heatmapGvl{20.0492}{0.184971}
\heatmapGvl{20.0683}{0.187984}
\heatmapGvl{20.0874}{0.208494}
\heatmapGvl{20.1066}{0.221154}
\heatmapGvl{20.1257}{0.258621}
\heatmapGvl{20.1448}{0.282443}
\heatmapGvl{20.1639}{0.314991}
\heatmapGvl{20.1831}{0.332703}
\heatmapGvl{20.2022}{0.361582}
\heatmapGvl{20.2213}{0.383178}
\heatmapGvl{20.2404}{0.414498}
\heatmapGvl{20.2596}{0.469388}
\heatmapGvl{20.2787}{0.489871}
\heatmapGvl{20.2978}{0.5}
\heatmapGvl{20.3169}{0.513863}
\heatmapGvl{20.3361}{0.539595}
\heatmapGvl{20.3552}{0.577206}
\heatmapGvl{20.3743}{0.595588}
\heatmapGvl{20.3934}{0.615385}
\heatmapGvl{20.4126}{0.628885}
\heatmapGvl{20.4317}{0.652095}
\heatmapGvl{20.4508}{0.670909}
\heatmapGvl{20.4699}{0.68306}
\heatmapGvl{20.4891}{0.702359}
\heatmapGvl{20.5082}{0.725953}
\heatmapGvl{20.5273}{0.747273}
\heatmapGvl{20.5464}{0.758123}
\heatmapGvl{20.5656}{0.793419}
\heatmapGvl{20.5847}{0.8213}
\heatmapGvl{20.6038}{0.844086}
\heatmapGvl{20.623}{0.871252}
\heatmapGvl{20.6421}{0.888696}
\heatmapGvl{20.6612}{0.894464}
\heatmapGvl{20.6803}{0.89726}
\heatmapGvl{20.6995}{0.902685}
\heatmapGvl{20.7186}{0.907743}
\heatmapGvl{20.7377}{0.911147}
\heatmapGvl{20.7568}{0.921474}
\heatmapGvl{20.776}{0.92733}
\heatmapGvl{20.7951}{0.929797}
\heatmapGvl{20.8142}{0.929122}
\heatmapGvl{20.8333}{0.930982}
\heatmapGvl{20.8525}{0.930197}
\heatmapGvl{20.8716}{0.932229}
\heatmapGvl{20.8907}{0.930931}
\heatmapGvl{20.9098}{0.932836}
\heatmapGvl{20.929}{0.933135}
\heatmapGvl{20.9481}{0.933135}
\heatmapGvl{20.9672}{0.93353}
\heatmapGvl{20.9863}{0.935199}
\heatmapGvl{21.0055}{0.935389}
\heatmapGvl{21.0247}{0.935673}
\heatmapGvl{21.0438}{0.937318}
\heatmapGvl{21.063}{0.937771}
\heatmapGvl{21.0822}{0.93804}
\heatmapGvl{21.1014}{0.938571}
\heatmapGvl{21.1205}{0.93918}
\heatmapGvl{21.1397}{0.943662}


==> data/tcf2-transition/category_tcf_dist/business.tex <==
\tcfDist{0.853018}{0.557023}{0.381753}{0.00720288}{0.0540216}


==> data/tcf2-transition/category_tcf_dist/education.tex <==
\tcfDist{0.899582}{0.600551}{0.371901}{0.00964187}{0.0179063}


==> data/tcf2-transition/category_tcf_dist/government.tex <==
\tcfDist{0.740223}{0.879397}{0.10804}{0.00251256}{0.0100503}


==> data/tcf2-transition/category_tcf_dist/news.tex <==
\tcfDist{0.919687}{0.469673}{0.254988}{0.0123703}{0.262969}


==> data/tcf2-transition/category_tcf_dist/shopping.tex <==
\tcfDist{0.891613}{0.557107}{0.383249}{0.00380711}{0.0558376}


==> data/tcf2-transition/category_tcf_dist/technology.tex <==
\tcfDist{0.833091}{0.53455}{0.396349}{0.00912647}{0.0599739}


==> data/tcf2-transition/cmp-share-toplist.tex <==
%
\tcfShare{0}{143}{150}{28}{72}{56}{49}{192}{690}
\tcfShare{1}{125}{104}{22}{45}{51}{34}{157}{538}
\tcfShare{2}{145}{71}{32}{37}{37}{27}{148}{497}
\tcfShare{3}{109}{76}{39}{41}{36}{43}{136}{480}
\tcfShare{4}{114}{56}{49}{41}{38}{28}{148}{474}
\tcfShare{5}{115}{65}{50}{35}{25}{20}{138}{448}
\tcfShare{6}{107}{55}{44}{20}{30}{25}{137}{418}
\tcfShare{7}{103}{35}{47}{29}{29}{29}{117}{389}
\tcfShare{8}{84}{45}{38}{34}{17}{17}{125}{360}
\tcfShare{9}{99}{49}{39}{22}{15}{17}{111}{352}
\tcfShare{10}{71}{35}{56}{23}{15}{21}{122}{343}
\tcfShare{11}{73}{41}{52}{25}{16}{20}{92}{319}
\tcfShare{12}{76}{38}{53}{14}{8}{14}{102}{305}
\tcfShare{13}{87}{36}{44}{22}{20}{15}{104}{328}
\tcfShare{14}{48}{24}{51}{25}{12}{19}{105}{284}
\tcfShare{15}{73}{33}{36}{24}{18}{15}{96}{295}
\tcfShare{16}{59}{20}{42}{20}{24}{14}{96}{275}
\tcfShare{17}{70}{28}{40}{11}{8}{18}{73}{248}
\tcfShare{18}{54}{29}{42}{17}{10}{14}{102}{268}
\tcfShare{19}{62}{25}{49}{12}{14}{8}{101}{271}


==> data/tcf2-transition/heatmap.tex <==
\heatmap{18.3041}{2}{0}
\heatmap{18.3233}{2}{0}
\heatmap{18.3425}{2}{0}
\heatmap{18.3616}{2}{0}
\heatmap{18.3808}{2}{0}
\heatmap{18.4}{2}{0}
\heatmap{18.4192}{2}{0}
\heatmap{18.4384}{2}{0}
\heatmap{18.4575}{2}{0}
\heatmap{18.4767}{2}{0}
\heatmap{18.4959}{2}{0}
\heatmap{18.5151}{2}{0}
\heatmap{18.5342}{2}{0}
\heatmap{18.5534}{2}{0}
\heatmap{18.5726}{2}{0}
\heatmap{18.5918}{2}{0.0857143}
\heatmap{18.611}{2}{0.1}
\heatmap{18.6301}{2}{0.1}
\heatmap{18.6493}{2}{0.1}
\heatmap{18.6685}{2}{0.1}
\heatmap{18.6877}{2}{0.1}
\heatmap{18.7068}{2}{0.1}
\heatmap{18.726}{2}{0.1}
\heatmap{18.7452}{2}{0.1}
\heatmap{18.7644}{2}{0.1}
\heatmap{18.7836}{2}{0.1}
\heatmap{18.8027}{2}{0.1}
\heatmap{18.8219}{2}{0.0887755}
\heatmap{18.8411}{2}{0.0714286}
\heatmap{18.8603}{2}{0.0714286}
\heatmap{18.8795}{2}{0.0714286}
\heatmap{18.8986}{2}{0.0714286}
\heatmap{18.9178}{2}{0.0714286}
\heatmap{18.937}{2}{0.067602}
\heatmap{18.9562}{2}{0.0625}
\heatmap{18.9753}{2}{0.0605159}
\heatmap{18.9945}{2}{0.031746}
\heatmap{19.0137}{2}{0}
\heatmap{19.0329}{2}{0}
\heatmap{19.0521}{2}{0}
\heatmap{19.0712}{2}{0}
\heatmap{19.0904}{2}{0.0142857}
\heatmap{19.1096}{2}{0.05}
\heatmap{19.1288}{2}{0.05}
\heatmap{19.1479}{2}{0.05}
\heatmap{19.1671}{2}{0.05}
\heatmap{19.1863}{2}{0.0857143}
\heatmap{19.2055}{2}{0.142857}
\heatmap{19.2247}{2}{0.114286}
\heatmap{19.2438}{2}{0.150649}
\heatmap{19.263}{2}{0.136364}
\heatmap{19.2822}{2}{0.136364}
\heatmap{19.3014}{2}{0.12987}
\heatmap{19.3205}{2}{0.0909091}
\heatmap{19.3397}{2}{0.0909091}
\heatmap{19.3589}{2}{0.0909091}
\heatmap{19.3781}{2}{0.0974026}
\heatmap{19.3973}{2}{0.136364}
\heatmap{19.4164}{2}{0.162338}
\heatmap{19.4356}{2}{0.162338}
\heatmap{19.4548}{2}{0.136364}
\heatmap{19.474}{2}{0.114286}
\heatmap{19.4932}{2}{0.1}
\heatmap{19.5123}{2}{0.05}
\heatmap{19.5315}{2}{0.0461039}
\heatmap{19.5507}{2}{0.0974026}
\heatmap{19.5699}{2}{0.149351}
\heatmap{19.589}{2}{0.181818}
\heatmap{19.6082}{2}{0.176948}
\heatmap{19.6274}{2}{0.208333}
\heatmap{19.6466}{2}{0.208333}
\heatmap{19.6658}{2}{0.208333}
\heatmap{19.6849}{2}{0.202381}
\heatmap{19.7041}{2}{0.196429}
\heatmap{19.7233}{2}{0.202381}
\heatmap{19.7425}{2}{0.216991}
\heatmap{19.7616}{2}{0.155844}
\heatmap{19.7808}{2}{0.136364}
\heatmap{19.8}{2}{0.136364}
\heatmap{19.8192}{2}{0.136364}
\heatmap{19.8384}{2}{0.158442}
\heatmap{19.8575}{2}{0.207143}
\heatmap{19.8767}{2}{0.2}
\heatmap{19.8959}{2}{0.2}
\heatmap{19.9151}{2}{0.207143}
\heatmap{19.9342}{2}{0.2}
\heatmap{19.9534}{2}{0.2}
\heatmap{19.9726}{2}{0.2}
\heatmap{19.9918}{2}{0.2}
\heatmap{20.0109}{2}{0.207143}
\heatmap{20.0301}{2}{0.2}
\heatmap{20.0492}{2}{0.2}
\heatmap{20.0683}{2}{0.2}
\heatmap{20.0874}{2}{0.178571}
\heatmap{20.1066}{2}{0.164286}
\heatmap{20.1257}{2}{0.15873}
\heatmap{20.1448}{2}{0.222222}
\heatmap{20.1639}{2}{0.222222}
\heatmap{20.1831}{2}{0.222222}
\heatmap{20.2022}{2}{0.222222}
\heatmap{20.2213}{2}{0.219048}
\heatmap{20.2404}{2}{0.2}
\heatmap{20.2596}{2}{0.194805}
\heatmap{20.2787}{2}{0.220779}
\heatmap{20.2978}{2}{0.233766}
\heatmap{20.3169}{2}{0.181818}
\heatmap{20.3361}{2}{0.181818}
\heatmap{20.3552}{2}{0.181818}
\heatmap{20.3743}{2}{0.207792}
\heatmap{20.3934}{2}{0.288311}
\heatmap{20.4126}{2}{0.330766}
\heatmap{20.4317}{2}{0.249603}
\heatmap{20.4508}{2}{0.239524}
\heatmap{20.4699}{2}{0.281786}
\heatmap{20.4891}{2}{0.299451}
\heatmap{20.5082}{2}{0.325165}
\heatmap{20.5273}{2}{0.368571}
\heatmap{20.5464}{2}{0.382857}
\heatmap{20.5656}{2}{0.382857}
\heatmap{20.5847}{2}{0.362198}
\heatmap{20.6038}{2}{0.406593}
\heatmap{20.623}{2}{0.472527}
\heatmap{20.6421}{2}{0.565934}
\heatmap{20.6612}{2}{0.574176}
\heatmap{20.6803}{2}{0.585165}
\heatmap{20.6995}{2}{0.587912}
\heatmap{20.7186}{2}{0.604396}
\heatmap{20.7377}{2}{0.598901}
\heatmap{20.7568}{2}{0.605718}
\heatmap{20.776}{2}{0.64}
\heatmap{20.7951}{2}{0.660099}
\heatmap{20.8142}{2}{0.67734}
\heatmap{20.8333}{2}{0.699507}
\heatmap{20.8525}{2}{0.70197}
\heatmap{20.8716}{2}{0.70197}
\heatmap{20.8907}{2}{0.730952}
\heatmap{20.9098}{2}{0.756568}
\heatmap{20.929}{2}{0.788177}
\heatmap{20.9481}{2}{0.837438}
\heatmap{20.9672}{2}{0.795567}
\heatmap{20.9863}{2}{0.817734}
\heatmap{21.0055}{2}{0.847291}
\heatmap{21.0247}{2}{0.839901}
\heatmap{21.0438}{2}{0.869458}
\heatmap{21.063}{2}{0.847291}
\heatmap{21.0822}{2}{0.857143}
\heatmap{21.1014}{2}{0.881773}
\heatmap{21.1205}{2}{0.874384}
\heatmap{21.1397}{2}{0.884881}
\heatmap{18.3041}{3}{0}
\heatmap{18.3233}{3}{0}
\heatmap{18.3425}{3}{0}
\heatmap{18.3616}{3}{0}
\heatmap{18.3808}{3}{0}
\heatmap{18.4}{3}{0}
\heatmap{18.4192}{3}{0}
\heatmap{18.4384}{3}{0}
\heatmap{18.4575}{3}{0}
\heatmap{18.4767}{3}{0.0238095}
\heatmap{18.4959}{3}{0.0333333}
\heatmap{18.5151}{3}{0.0333333}
\heatmap{18.5342}{3}{0.0619048}
\heatmap{18.5534}{3}{0.0318803}
\heatmap{18.5726}{3}{0.0289449}
\heatmap{18.5918}{3}{0.0273601}
\heatmap{18.611}{3}{0.0239796}
\heatmap{18.6301}{3}{0.0238095}
\heatmap{18.6493}{3}{0.0436127}
\heatmap{18.6685}{3}{0.0213509}
\heatmap{18.6877}{3}{0.0207143}
\heatmap{18.7068}{3}{0.02}
\heatmap{18.726}{3}{0.0192308}
\heatmap{18.7452}{3}{0.0192308}
\heatmap{18.7644}{3}{0.0192308}
\heatmap{18.7836}{3}{0.0192308}
\heatmap{18.8027}{3}{0.0192308}
\heatmap{18.8219}{3}{0.019129}
\heatmap{18.8411}{3}{0.0175932}
\heatmap{18.8603}{3}{0.0148959}
\heatmap{18.8795}{3}{0.0131177}
\heatmap{18.8986}{3}{0.0155008}
\heatmap{18.9178}{3}{0.0232558}
\heatmap{18.937}{3}{0.0232558}
\heatmap{18.9562}{3}{0.0225142}
\heatmap{18.9753}{3}{0.0218081}
\heatmap{18.9945}{3}{0.021607}
\heatmap{19.0137}{3}{0.0212766}
\heatmap{19.0329}{3}{0.0208359}
\heatmap{19.0521}{3}{0.0130612}
\heatmap{19.0712}{3}{0.00994398}
\heatmap{19.0904}{3}{0.00969619}
\heatmap{19.1096}{3}{0.00958947}
\heatmap{19.1288}{3}{0.00930917}
\heatmap{19.1479}{3}{0.00925926}
\heatmap{19.1671}{3}{0.00925926}
\heatmap{19.1863}{3}{0.00904453}
\heatmap{19.2055}{3}{0.016425}
\heatmap{19.2247}{3}{0.0106571}
\heatmap{19.2438}{3}{0.0163934}
\heatmap{19.263}{3}{0.0161668}
\heatmap{19.2822}{3}{0.0211217}
\heatmap{19.3014}{3}{0.0282384}
\heatmap{19.3205}{3}{0.02917}
\heatmap{19.3397}{3}{0.028808}
\heatmap{19.3589}{3}{0.0280588}
\heatmap{19.3781}{3}{0.0276147}
\heatmap{19.3973}{3}{0.0293542}
\heatmap{19.4164}{3}{0.0342466}
\heatmap{19.4356}{3}{0.0337838}
\heatmap{19.4548}{3}{0.0345863}
\heatmap{19.474}{3}{0.0395945}
\heatmap{19.4932}{3}{0.0333333}
\heatmap{19.5123}{3}{0.0409524}
\heatmap{19.5315}{3}{0.0466667}
\heatmap{19.5507}{3}{0.0541729}
\heatmap{19.5699}{3}{0.0596617}
\heatmap{19.589}{3}{0.0593233}
\heatmap{19.6082}{3}{0.0598872}
\heatmap{19.6274}{3}{0.060695}
\heatmap{19.6466}{3}{0.0608108}
\heatmap{19.6658}{3}{0.0627413}
\heatmap{19.6849}{3}{0.0749061}
\heatmap{19.7041}{3}{0.0753425}
\heatmap{19.7233}{3}{0.0762394}
\heatmap{19.7425}{3}{0.0763158}
\heatmap{19.7616}{3}{0.0810811}
\heatmap{19.7808}{3}{0.0847075}
\heatmap{19.8}{3}{0.0853694}
\heatmap{19.8192}{3}{0.0855418}
\heatmap{19.8384}{3}{0.084852}
\heatmap{19.8575}{3}{0.0857143}
\heatmap{19.8767}{3}{0.092377}
\heatmap{19.8959}{3}{0.0933759}
\heatmap{19.9151}{3}{0.0872229}
\heatmap{19.9342}{3}{0.101471}
\heatmap{19.9534}{3}{0.102478}
\heatmap{19.9726}{3}{0.100732}
\heatmap{19.9918}{3}{0.114619}
\heatmap{20.0109}{3}{0.114764}
\heatmap{20.0301}{3}{0.111208}
\heatmap{20.0492}{3}{0.116058}
\heatmap{20.0683}{3}{0.121378}
\heatmap{20.0874}{3}{0.135185}
\heatmap{20.1066}{3}{0.151604}
\heatmap{20.1257}{3}{0.154689}
\heatmap{20.1448}{3}{0.154689}
\heatmap{20.1639}{3}{0.154689}
\heatmap{20.1831}{3}{0.154611}
\heatmap{20.2022}{3}{0.158228}
\heatmap{20.2213}{3}{0.161134}
\heatmap{20.2404}{3}{0.159097}
\heatmap{20.2596}{3}{0.159097}
\heatmap{20.2787}{3}{0.159731}
\heatmap{20.2978}{3}{0.169929}
\heatmap{20.3169}{3}{0.177359}
\heatmap{20.3361}{3}{0.193196}
\heatmap{20.3552}{3}{0.207275}
\heatmap{20.3743}{3}{0.227679}
\heatmap{20.3934}{3}{0.253529}
\heatmap{20.4126}{3}{0.274002}
\heatmap{20.4317}{3}{0.258412}
\heatmap{20.4508}{3}{0.265872}
\heatmap{20.4699}{3}{0.277391}
\heatmap{20.4891}{3}{0.271227}
\heatmap{20.5082}{3}{0.293616}
\heatmap{20.5273}{3}{0.315468}
\heatmap{20.5464}{3}{0.32902}
\heatmap{20.5656}{3}{0.354695}
\heatmap{20.5847}{3}{0.384034}
\heatmap{20.6038}{3}{0.40102}
\heatmap{20.623}{3}{0.466869}
\heatmap{20.6421}{3}{0.538701}
\heatmap{20.6612}{3}{0.580316}
\heatmap{20.6803}{3}{0.5983}
\heatmap{20.6995}{3}{0.625865}
\heatmap{20.7186}{3}{0.636447}
\heatmap{20.7377}{3}{0.652509}
\heatmap{20.7568}{3}{0.66404}
\heatmap{20.776}{3}{0.663116}
\heatmap{20.7951}{3}{0.69707}
\heatmap{20.8142}{3}{0.712084}
\heatmap{20.8333}{3}{0.723497}
\heatmap{20.8525}{3}{0.729572}
\heatmap{20.8716}{3}{0.727745}
\heatmap{20.8907}{3}{0.738684}
\heatmap{20.9098}{3}{0.748344}
\heatmap{20.929}{3}{0.794021}
\heatmap{20.9481}{3}{0.829104}
\heatmap{20.9672}{3}{0.833643}
\heatmap{20.9863}{3}{0.844005}
\heatmap{21.0055}{3}{0.847589}
\heatmap{21.0247}{3}{0.854346}
\heatmap{21.0438}{3}{0.857221}
\heatmap{21.063}{3}{0.862121}
\heatmap{21.0822}{3}{0.85803}
\heatmap{21.1014}{3}{0.858902}
\heatmap{21.1205}{3}{0.874876}
\heatmap{21.1397}{3}{0.872732}
\heatmap{18.3041}{4}{0}
\heatmap{18.3233}{4}{0}
\heatmap{18.3425}{4}{0}
\heatmap{18.3616}{4}{0}
\heatmap{18.3808}{4}{0}
\heatmap{18.4}{4}{0}
\heatmap{18.4192}{4}{0}
\heatmap{18.4384}{4}{0}
\heatmap{18.4575}{4}{0}
\heatmap{18.4767}{4}{0}
\heatmap{18.4959}{4}{0}
\heatmap{18.5151}{4}{0}
\heatmap{18.5342}{4}{0.00537975}
\heatmap{18.5534}{4}{0.000840336}
\heatmap{18.5726}{4}{0.0116284}
\heatmap{18.5918}{4}{0.0103531}
\heatmap{18.611}{4}{0.0101533}
\heatmap{18.6301}{4}{0.0108198}
\heatmap{18.6493}{4}{0.0149606}
\heatmap{18.6685}{4}{0.0123907}
\heatmap{18.6877}{4}{0.0152619}
\heatmap{18.7068}{4}{0.0150437}
\heatmap{18.726}{4}{0.0146875}
\heatmap{18.7452}{4}{0.0143053}
\heatmap{18.7644}{4}{0.0142472}
\heatmap{18.7836}{4}{0.0138714}
\heatmap{18.8027}{4}{0.0137436}
\heatmap{18.8219}{4}{0.0135486}
\heatmap{18.8411}{4}{0.0130568}
\heatmap{18.8603}{4}{0.0118982}
\heatmap{18.8795}{4}{0.0107456}
\heatmap{18.8986}{4}{0.0099459}
\heatmap{18.9178}{4}{0.0125304}
\heatmap{18.937}{4}{0.0094859}
\heatmap{18.9562}{4}{0.00913129}
\heatmap{18.9753}{4}{0.0126728}
\heatmap{18.9945}{4}{0.0143936}
\heatmap{19.0137}{4}{0.0138904}
\heatmap{19.0329}{4}{0.0150136}
\heatmap{19.0521}{4}{0.0155913}
\heatmap{19.0712}{4}{0.0150375}
\heatmap{19.0904}{4}{0.0142876}
\heatmap{19.1096}{4}{0.016336}
\heatmap{19.1288}{4}{0.0193962}
\heatmap{19.1479}{4}{0.0192433}
\heatmap{19.1671}{4}{0.0196016}
\heatmap{19.1863}{4}{0.0241}
\heatmap{19.2055}{4}{0.0280401}
\heatmap{19.2247}{4}{0.0300827}
\heatmap{19.2438}{4}{0.0298511}
\heatmap{19.263}{4}{0.0320102}
\heatmap{19.2822}{4}{0.0311366}
\heatmap{19.3014}{4}{0.0323554}
\heatmap{19.3205}{4}{0.0323514}
\heatmap{19.3397}{4}{0.0353338}
\heatmap{19.3589}{4}{0.0330702}
\heatmap{19.3781}{4}{0.0326145}
\heatmap{19.3973}{4}{0.0357708}
\heatmap{19.4164}{4}{0.0414163}
\heatmap{19.4356}{4}{0.0463584}
\heatmap{19.4548}{4}{0.045933}
\heatmap{19.474}{4}{0.0530593}
\heatmap{19.4932}{4}{0.0515353}
\heatmap{19.5123}{4}{0.0532994}
\heatmap{19.5315}{4}{0.0539212}
\heatmap{19.5507}{4}{0.0536751}
\heatmap{19.5699}{4}{0.0570746}
\heatmap{19.589}{4}{0.0569658}
\heatmap{19.6082}{4}{0.0574714}
\heatmap{19.6274}{4}{0.0653657}
\heatmap{19.6466}{4}{0.0749166}
\heatmap{19.6658}{4}{0.0810291}
\heatmap{19.6849}{4}{0.0882503}
\heatmap{19.7041}{4}{0.0918332}
\heatmap{19.7233}{4}{0.0948117}
\heatmap{19.7425}{4}{0.0995266}
\heatmap{19.7616}{4}{0.100805}
\heatmap{19.7808}{4}{0.105275}
\heatmap{19.8}{4}{0.107819}
\heatmap{19.8192}{4}{0.104727}
\heatmap{19.8384}{4}{0.108539}
\heatmap{19.8575}{4}{0.108197}
\heatmap{19.8767}{4}{0.113009}
\heatmap{19.8959}{4}{0.116891}
\heatmap{19.9151}{4}{0.114221}
\heatmap{19.9342}{4}{0.117035}
\heatmap{19.9534}{4}{0.117174}
\heatmap{19.9726}{4}{0.115348}
\heatmap{19.9918}{4}{0.117852}
\heatmap{20.0109}{4}{0.117435}
\heatmap{20.0301}{4}{0.116794}
\heatmap{20.0492}{4}{0.120479}
\heatmap{20.0683}{4}{0.12713}
\heatmap{20.0874}{4}{0.132188}
\heatmap{20.1066}{4}{0.140682}
\heatmap{20.1257}{4}{0.143324}
\heatmap{20.1448}{4}{0.149826}
\heatmap{20.1639}{4}{0.154966}
\heatmap{20.1831}{4}{0.150545}
\heatmap{20.2022}{4}{0.154168}
\heatmap{20.2213}{4}{0.158464}
\heatmap{20.2404}{4}{0.156296}
\heatmap{20.2596}{4}{0.156598}
\heatmap{20.2787}{4}{0.165941}
\heatmap{20.2978}{4}{0.173112}
\heatmap{20.3169}{4}{0.175899}
\heatmap{20.3361}{4}{0.180933}
\heatmap{20.3552}{4}{0.184267}
\heatmap{20.3743}{4}{0.187942}
\heatmap{20.3934}{4}{0.203374}
\heatmap{20.4126}{4}{0.226989}
\heatmap{20.4317}{4}{0.227454}
\heatmap{20.4508}{4}{0.226559}
\heatmap{20.4699}{4}{0.237501}
\heatmap{20.4891}{4}{0.254882}
\heatmap{20.5082}{4}{0.282257}
\heatmap{20.5273}{4}{0.308366}
\heatmap{20.5464}{4}{0.317166}
\heatmap{20.5656}{4}{0.343857}
\heatmap{20.5847}{4}{0.377022}
\heatmap{20.6038}{4}{0.420438}
\heatmap{20.623}{4}{0.495439}
\heatmap{20.6421}{4}{0.551617}
\heatmap{20.6612}{4}{0.575295}
\heatmap{20.6803}{4}{0.598653}
\heatmap{20.6995}{4}{0.617572}
\heatmap{20.7186}{4}{0.644198}
\heatmap{20.7377}{4}{0.661968}
\heatmap{20.7568}{4}{0.677367}
\heatmap{20.776}{4}{0.680387}
\heatmap{20.7951}{4}{0.704367}
\heatmap{20.8142}{4}{0.711795}
\heatmap{20.8333}{4}{0.727121}
\heatmap{20.8525}{4}{0.742734}
\heatmap{20.8716}{4}{0.765401}
\heatmap{20.8907}{4}{0.773897}
\heatmap{20.9098}{4}{0.787823}
\heatmap{20.929}{4}{0.80444}
\heatmap{20.9481}{4}{0.8322}
\heatmap{20.9672}{4}{0.840829}
\heatmap{20.9863}{4}{0.848023}
\heatmap{21.0055}{4}{0.855945}
\heatmap{21.0247}{4}{0.863703}
\heatmap{21.0438}{4}{0.868529}
\heatmap{21.063}{4}{0.876339}
\heatmap{21.0822}{4}{0.884505}
\heatmap{21.1014}{4}{0.887989}
\heatmap{21.1205}{4}{0.889836}
\heatmap{21.1397}{4}{0.876715}
\heatmap{18.3041}{5}{0}
\heatmap{18.3233}{5}{0}
\heatmap{18.3425}{5}{0}
\heatmap{18.3616}{5}{0}
\heatmap{18.3808}{5}{0}
\heatmap{18.4}{5}{0}
\heatmap{18.4192}{5}{0.00419663}
\heatmap{18.4384}{5}{0.00532335}
\heatmap{18.4575}{5}{0.00521961}
\heatmap{18.4767}{5}{0.00756977}
\heatmap{18.4959}{5}{0.00797185}
\heatmap{18.5151}{5}{0.00954461}
\heatmap{18.5342}{5}{0.0182269}
\heatmap{18.5534}{5}{0.0087374}
\heatmap{18.5726}{5}{0.00805518}
\heatmap{18.5918}{5}{0.00550812}
\heatmap{18.611}{5}{0.00465252}
\heatmap{18.6301}{5}{0.00536545}
\heatmap{18.6493}{5}{0.00619675}
\heatmap{18.6685}{5}{0.00477422}
\heatmap{18.6877}{5}{0.0039629}
\heatmap{18.7068}{5}{0.00474255}
\heatmap{18.726}{5}{0.00500921}
\heatmap{18.7452}{5}{0.00493133}
\heatmap{18.7644}{5}{0.00607651}
\heatmap{18.7836}{5}{0.0059852}
\heatmap{18.8027}{5}{0.00589432}
\heatmap{18.8219}{5}{0.00579493}
\heatmap{18.8411}{5}{0.00548935}
\heatmap{18.8603}{5}{0.00425126}
\heatmap{18.8795}{5}{0.00596993}
\heatmap{18.8986}{5}{0.00741672}
\heatmap{18.9178}{5}{0.00915204}
\heatmap{18.937}{5}{0.00673464}
\heatmap{18.9562}{5}{0.00755997}
\heatmap{18.9753}{5}{0.00779052}
\heatmap{18.9945}{5}{0.0068739}
\heatmap{19.0137}{5}{0.0071833}
\heatmap{19.0329}{5}{0.00710489}
\heatmap{19.0521}{5}{0.00739712}
\heatmap{19.0712}{5}{0.0102325}
\heatmap{19.0904}{5}{0.00885047}
\heatmap{19.1096}{5}{0.00869283}
\heatmap{19.1288}{5}{0.00991399}
\heatmap{19.1479}{5}{0.00899822}
\heatmap{19.1671}{5}{0.00956095}
\heatmap{19.1863}{5}{0.0108475}
\heatmap{19.2055}{5}{0.011158}
\heatmap{19.2247}{5}{0.0133051}
\heatmap{19.2438}{5}{0.015358}
\heatmap{19.263}{5}{0.0172021}
\heatmap{19.2822}{5}{0.028663}
\heatmap{19.3014}{5}{0.0339888}
\heatmap{19.3205}{5}{0.0343067}
\heatmap{19.3397}{5}{0.034181}
\heatmap{19.3589}{5}{0.035437}
\heatmap{19.3781}{5}{0.0369657}
\heatmap{19.3973}{5}{0.0388853}
\heatmap{19.4164}{5}{0.0402186}
\heatmap{19.4356}{5}{0.0396056}
\heatmap{19.4548}{5}{0.0406738}
\heatmap{19.474}{5}{0.0432661}
\heatmap{19.4932}{5}{0.0437213}
\heatmap{19.5123}{5}{0.0439929}
\heatmap{19.5315}{5}{0.0454467}
\heatmap{19.5507}{5}{0.0452496}
\heatmap{19.5699}{5}{0.0459632}
\heatmap{19.589}{5}{0.0434825}
\heatmap{19.6082}{5}{0.042818}
\heatmap{19.6274}{5}{0.0450258}
\heatmap{19.6466}{5}{0.0448329}
\heatmap{19.6658}{5}{0.0537955}
\heatmap{19.6849}{5}{0.0759884}
\heatmap{19.7041}{5}{0.0761489}
\heatmap{19.7233}{5}{0.0781189}
\heatmap{19.7425}{5}{0.0795407}
\heatmap{19.7616}{5}{0.0815548}
\heatmap{19.7808}{5}{0.084489}
\heatmap{19.8}{5}{0.0849847}
\heatmap{19.8192}{5}{0.0861455}
\heatmap{19.8384}{5}{0.0874765}
\heatmap{19.8575}{5}{0.0885586}
\heatmap{19.8767}{5}{0.0908975}
\heatmap{19.8959}{5}{0.0910632}
\heatmap{19.9151}{5}{0.0931652}
\heatmap{19.9342}{5}{0.0951354}
\heatmap{19.9534}{5}{0.0968009}
\heatmap{19.9726}{5}{0.0961997}
\heatmap{19.9918}{5}{0.0950404}
\heatmap{20.0109}{5}{0.0944626}
\heatmap{20.0301}{5}{0.0968572}
\heatmap{20.0492}{5}{0.102562}
\heatmap{20.0683}{5}{0.112463}
\heatmap{20.0874}{5}{0.114701}
\heatmap{20.1066}{5}{0.119861}
\heatmap{20.1257}{5}{0.126143}
\heatmap{20.1448}{5}{0.129715}
\heatmap{20.1639}{5}{0.13304}
\heatmap{20.1831}{5}{0.134054}
\heatmap{20.2022}{5}{0.140613}
\heatmap{20.2213}{5}{0.155}
\heatmap{20.2404}{5}{0.16093}
\heatmap{20.2596}{5}{0.166677}
\heatmap{20.2787}{5}{0.173425}
\heatmap{20.2978}{5}{0.176819}
\heatmap{20.3169}{5}{0.181254}
\heatmap{20.3361}{5}{0.18672}
\heatmap{20.3552}{5}{0.192343}
\heatmap{20.3743}{5}{0.201423}
\heatmap{20.3934}{5}{0.216788}
\heatmap{20.4126}{5}{0.230483}
\heatmap{20.4317}{5}{0.244355}
\heatmap{20.4508}{5}{0.257941}
\heatmap{20.4699}{5}{0.267149}
\heatmap{20.4891}{5}{0.278635}
\heatmap{20.5082}{5}{0.296934}
\heatmap{20.5273}{5}{0.318153}
\heatmap{20.5464}{5}{0.329892}
\heatmap{20.5656}{5}{0.352848}
\heatmap{20.5847}{5}{0.387036}
\heatmap{20.6038}{5}{0.427433}
\heatmap{20.623}{5}{0.511994}
\heatmap{20.6421}{5}{0.591232}
\heatmap{20.6612}{5}{0.624855}
\heatmap{20.6803}{5}{0.647511}
\heatmap{20.6995}{5}{0.669061}
\heatmap{20.7186}{5}{0.688802}
\heatmap{20.7377}{5}{0.704111}
\heatmap{20.7568}{5}{0.722415}
\heatmap{20.776}{5}{0.72803}
\heatmap{20.7951}{5}{0.751959}
\heatmap{20.8142}{5}{0.770314}
\heatmap{20.8333}{5}{0.785679}
\heatmap{20.8525}{5}{0.79445}
\heatmap{20.8716}{5}{0.807824}
\heatmap{20.8907}{5}{0.821768}
\heatmap{20.9098}{5}{0.828989}
\heatmap{20.929}{5}{0.837637}
\heatmap{20.9481}{5}{0.848089}
\heatmap{20.9672}{5}{0.85399}
\heatmap{20.9863}{5}{0.860019}
\heatmap{21.0055}{5}{0.865757}
\heatmap{21.0247}{5}{0.872505}
\heatmap{21.0438}{5}{0.879061}
\heatmap{21.063}{5}{0.88574}
\heatmap{21.0822}{5}{0.890728}
\heatmap{21.1014}{5}{0.899173}
\heatmap{21.1205}{5}{0.906861}
\heatmap{21.1397}{5}{0.899024}
\heatmap{18.3041}{6}{0}
\heatmap{18.3233}{6}{0}
\heatmap{18.3425}{6}{0}
\heatmap{18.3616}{6}{0}
\heatmap{18.3808}{6}{0}
\heatmap{18.4}{6}{0.00227513}
\heatmap{18.4192}{6}{0.0115308}
\heatmap{18.4384}{6}{0.0102258}
\heatmap{18.4575}{6}{0.0120855}
\heatmap{18.4767}{6}{0.01753}
\heatmap{18.4959}{6}{0.0267971}
\heatmap{18.5151}{6}{0.0392762}
\heatmap{18.5342}{6}{0.0472839}
\heatmap{18.5534}{6}{0.0306341}
\heatmap{18.5726}{6}{0.0224513}
\heatmap{18.5918}{6}{0.0200774}
\heatmap{18.611}{6}{0.0169514}
\heatmap{18.6301}{6}{0.0158025}
\heatmap{18.6493}{6}{0.0154801}
\heatmap{18.6685}{6}{0.0136784}
\heatmap{18.6877}{6}{0.0111688}
\heatmap{18.7068}{6}{0.00971811}
\heatmap{18.726}{6}{0.00899002}
\heatmap{18.7452}{6}{0.00856745}
\heatmap{18.7644}{6}{0.00871876}
\heatmap{18.7836}{6}{0.00932641}
\heatmap{18.8027}{6}{0.00910487}
\heatmap{18.8219}{6}{0.00885687}
\heatmap{18.8411}{6}{0.00858689}
\heatmap{18.8603}{6}{0.00795628}
\heatmap{18.8795}{6}{0.00809999}
\heatmap{18.8986}{6}{0.00878558}
\heatmap{18.9178}{6}{0.0103988}
\heatmap{18.937}{6}{0.00956405}
\heatmap{18.9562}{6}{0.0105558}
\heatmap{18.9753}{6}{0.0111579}
\heatmap{18.9945}{6}{0.0103846}
\heatmap{19.0137}{6}{0.0108238}
\heatmap{19.0329}{6}{0.0109657}
\heatmap{19.0521}{6}{0.0111258}
\heatmap{19.0712}{6}{0.011293}
\heatmap{19.0904}{6}{0.0109586}
\heatmap{19.1096}{6}{0.0110019}
\heatmap{19.1288}{6}{0.0104784}
\heatmap{19.1479}{6}{0.010111}
\heatmap{19.1671}{6}{0.0102207}
\heatmap{19.1863}{6}{0.0103291}
\heatmap{19.2055}{6}{0.0119803}
\heatmap{19.2247}{6}{0.0136232}
\heatmap{19.2438}{6}{0.0165954}
\heatmap{19.263}{6}{0.0148857}
\heatmap{19.2822}{6}{0.0167968}
\heatmap{19.3014}{6}{0.0183363}
\heatmap{19.3205}{6}{0.0199205}
\heatmap{19.3397}{6}{0.0215599}
\heatmap{19.3589}{6}{0.0230063}
\heatmap{19.3781}{6}{0.0241943}
\heatmap{19.3973}{6}{0.0249611}
\heatmap{19.4164}{6}{0.0252895}
\heatmap{19.4356}{6}{0.0259878}
\heatmap{19.4548}{6}{0.0266302}
\heatmap{19.474}{6}{0.0267862}
\heatmap{19.4932}{6}{0.0266778}
\heatmap{19.5123}{6}{0.0266387}
\heatmap{19.5315}{6}{0.026922}
\heatmap{19.5507}{6}{0.0275182}
\heatmap{19.5699}{6}{0.0279984}
\heatmap{19.589}{6}{0.0282329}
\heatmap{19.6082}{6}{0.0292432}
\heatmap{19.6274}{6}{0.0310227}
\heatmap{19.6466}{6}{0.0321719}
\heatmap{19.6658}{6}{0.0340363}
\heatmap{19.6849}{6}{0.0364872}
\heatmap{19.7041}{6}{0.0384417}
\heatmap{19.7233}{6}{0.0433825}
\heatmap{19.7425}{6}{0.043534}
\heatmap{19.7616}{6}{0.046474}
\heatmap{19.7808}{6}{0.0494057}
\heatmap{19.8}{6}{0.050062}
\heatmap{19.8192}{6}{0.0510016}
\heatmap{19.8384}{6}{0.0521008}
\heatmap{19.8575}{6}{0.0535919}
\heatmap{19.8767}{6}{0.055841}
\heatmap{19.8959}{6}{0.0575051}
\heatmap{19.9151}{6}{0.0600056}
\heatmap{19.9342}{6}{0.0622112}
\heatmap{19.9534}{6}{0.0630176}
\heatmap{19.9726}{6}{0.0638943}
\heatmap{19.9918}{6}{0.0655544}
\heatmap{20.0109}{6}{0.0676414}
\heatmap{20.0301}{6}{0.0686081}
\heatmap{20.0492}{6}{0.0713743}
\heatmap{20.0683}{6}{0.075924}
\heatmap{20.0874}{6}{0.0795021}
\heatmap{20.1066}{6}{0.082527}
\heatmap{20.1257}{6}{0.0873792}
\heatmap{20.1448}{6}{0.090084}
\heatmap{20.1639}{6}{0.0917957}
\heatmap{20.1831}{6}{0.0932108}
\heatmap{20.2022}{6}{0.0981611}
\heatmap{20.2213}{6}{0.115318}
\heatmap{20.2404}{6}{0.126762}
\heatmap{20.2596}{6}{0.136537}
\heatmap{20.2787}{6}{0.141253}
\heatmap{20.2978}{6}{0.143878}
\heatmap{20.3169}{6}{0.146632}
\heatmap{20.3361}{6}{0.150038}
\heatmap{20.3552}{6}{0.154952}
\heatmap{20.3743}{6}{0.162622}
\heatmap{20.3934}{6}{0.176048}
\heatmap{20.4126}{6}{0.191148}
\heatmap{20.4317}{6}{0.204434}
\heatmap{20.4508}{6}{0.213358}
\heatmap{20.4699}{6}{0.222933}
\heatmap{20.4891}{6}{0.23624}
\heatmap{20.5082}{6}{0.250103}
\heatmap{20.5273}{6}{0.265313}
\heatmap{20.5464}{6}{0.280174}
\heatmap{20.5656}{6}{0.302846}
\heatmap{20.5847}{6}{0.335209}
\heatmap{20.6038}{6}{0.372259}
\heatmap{20.623}{6}{0.432499}
\heatmap{20.6421}{6}{0.498344}
\heatmap{20.6612}{6}{0.534294}
\heatmap{20.6803}{6}{0.563435}
\heatmap{20.6995}{6}{0.587517}
\heatmap{20.7186}{6}{0.61042}
\heatmap{20.7377}{6}{0.628545}
\heatmap{20.7568}{6}{0.648077}
\heatmap{20.776}{6}{0.662314}
\heatmap{20.7951}{6}{0.685913}
\heatmap{20.8142}{6}{0.704494}
\heatmap{20.8333}{6}{0.721048}
\heatmap{20.8525}{6}{0.735824}
\heatmap{20.8716}{6}{0.750576}
\heatmap{20.8907}{6}{0.769241}
\heatmap{20.9098}{6}{0.780083}
\heatmap{20.929}{6}{0.792554}
\heatmap{20.9481}{6}{0.806077}
\heatmap{20.9672}{6}{0.814951}
\heatmap{20.9863}{6}{0.823468}
\heatmap{21.0055}{6}{0.830607}
\heatmap{21.0247}{6}{0.837486}
\heatmap{21.0438}{6}{0.846997}
\heatmap{21.063}{6}{0.856318}
\heatmap{21.0822}{6}{0.86536}
\heatmap{21.1014}{6}{0.87394}
\heatmap{21.1205}{6}{0.880681}
\heatmap{21.1397}{6}{0.880437}
\heatmap{18.3041}{7}{0}
\heatmap{18.3233}{7}{0}
\heatmap{18.3425}{7}{0}
\heatmap{18.3616}{7}{0}
\heatmap{18.3808}{7}{0}
\heatmap{18.4}{7}{0}
\heatmap{18.4192}{7}{0}
\heatmap{18.4384}{7}{0.00521422}
\heatmap{18.4575}{7}{0.00399335}
\heatmap{18.4767}{7}{0.0032964}
\heatmap{18.4959}{7}{0.00269894}
\heatmap{18.5151}{7}{0.00230008}
\heatmap{18.5342}{7}{0.00316191}
\heatmap{18.5534}{7}{0.00484522}
\heatmap{18.5726}{7}{0.0046397}
\heatmap{18.5918}{7}{0.00431089}
\heatmap{18.611}{7}{0.00331545}
\heatmap{18.6301}{7}{0.00233273}
\heatmap{18.6493}{7}{0.0021646}
\heatmap{18.6685}{7}{0.00199733}
\heatmap{18.6877}{7}{0.00184533}
\heatmap{18.7068}{7}{0.00109392}
\heatmap{18.726}{7}{0.000780848}
\heatmap{18.7452}{7}{0.00215646}
\heatmap{18.7644}{7}{0.00303215}
\heatmap{18.7836}{7}{0.00325325}
\heatmap{18.8027}{7}{0.00356669}
\heatmap{18.8219}{7}{0.00374024}
\heatmap{18.8411}{7}{0.00387637}
\heatmap{18.8603}{7}{0.00331307}
\heatmap{18.8795}{7}{0.00346621}
\heatmap{18.8986}{7}{0.00451528}
\heatmap{18.9178}{7}{0.0047432}
\heatmap{18.937}{7}{0.00535695}
\heatmap{18.9562}{7}{0.00545403}
\heatmap{18.9753}{7}{0.00583758}
\heatmap{18.9945}{7}{0.00555189}
\heatmap{19.0137}{7}{0.00538329}
\heatmap{19.0329}{7}{0.00548539}
\heatmap{19.0521}{7}{0.0056698}
\heatmap{19.0712}{7}{0.00639362}
\heatmap{19.0904}{7}{0.006841}
\heatmap{19.1096}{7}{0.00696184}
\heatmap{19.1288}{7}{0.00706605}
\heatmap{19.1479}{7}{0.00735015}
\heatmap{19.1671}{7}{0.00748128}
\heatmap{19.1863}{7}{0.00787749}
\heatmap{19.2055}{7}{0.00847003}
\heatmap{19.2247}{7}{0.010369}
\heatmap{19.2438}{7}{0.0127632}
\heatmap{19.263}{7}{0.00928477}
\heatmap{19.2822}{7}{0.00899508}
\heatmap{19.3014}{7}{0.00847756}
\heatmap{19.3205}{7}{0.00829469}
\heatmap{19.3397}{7}{0.00814301}
\heatmap{19.3589}{7}{0.00797035}
\heatmap{19.3781}{7}{0.00801262}
\heatmap{19.3973}{7}{0.00859603}
\heatmap{19.4164}{7}{0.00986752}
\heatmap{19.4356}{7}{0.0105642}
\heatmap{19.4548}{7}{0.0112845}
\heatmap{19.474}{7}{0.0116341}
\heatmap{19.4932}{7}{0.0118758}
\heatmap{19.5123}{7}{0.0122652}
\heatmap{19.5315}{7}{0.0129735}
\heatmap{19.5507}{7}{0.0134202}
\heatmap{19.5699}{7}{0.0136889}
\heatmap{19.589}{7}{0.0135195}
\heatmap{19.6082}{7}{0.0135844}
\heatmap{19.6274}{7}{0.0148154}
\heatmap{19.6466}{7}{0.0154064}
\heatmap{19.6658}{7}{0.0158607}
\heatmap{19.6849}{7}{0.0161627}
\heatmap{19.7041}{7}{0.017069}
\heatmap{19.7233}{7}{0.0204544}
\heatmap{19.7425}{7}{0.0219669}
\heatmap{19.7616}{7}{0.0229266}
\heatmap{19.7808}{7}{0.0243923}
\heatmap{19.8}{7}{0.0263713}
\heatmap{19.8192}{7}{0.0280789}
\heatmap{19.8384}{7}{0.0296283}
\heatmap{19.8575}{7}{0.0304707}
\heatmap{19.8767}{7}{0.0316069}
\heatmap{19.8959}{7}{0.0335379}
\heatmap{19.9151}{7}{0.0354581}
\heatmap{19.9342}{7}{0.0377451}
\heatmap{19.9534}{7}{0.0390535}
\heatmap{19.9726}{7}{0.0401874}
\heatmap{19.9918}{7}{0.0412409}
\heatmap{20.0109}{7}{0.0426534}
\heatmap{20.0301}{7}{0.044564}
\heatmap{20.0492}{7}{0.0474657}
\heatmap{20.0683}{7}{0.0478784}
\heatmap{20.0874}{7}{0.0489276}
\heatmap{20.1066}{7}{0.0502823}
\heatmap{20.1257}{7}{0.0521998}
\heatmap{20.1448}{7}{0.0533626}
\heatmap{20.1639}{7}{0.0543007}
\heatmap{20.1831}{7}{0.0557346}
\heatmap{20.2022}{7}{0.0575479}
\heatmap{20.2213}{7}{0.060776}
\heatmap{20.2404}{7}{0.0649479}
\heatmap{20.2596}{7}{0.0675742}
\heatmap{20.2787}{7}{0.0697211}
\heatmap{20.2978}{7}{0.0722032}
\heatmap{20.3169}{7}{0.0741306}
\heatmap{20.3361}{7}{0.0763358}
\heatmap{20.3552}{7}{0.079229}
\heatmap{20.3743}{7}{0.0835335}
\heatmap{20.3934}{7}{0.0914636}
\heatmap{20.4126}{7}{0.0988804}
\heatmap{20.4317}{7}{0.108455}
\heatmap{20.4508}{7}{0.115311}
\heatmap{20.4699}{7}{0.121387}
\heatmap{20.4891}{7}{0.129515}
\heatmap{20.5082}{7}{0.141979}
\heatmap{20.5273}{7}{0.152926}
\heatmap{20.5464}{7}{0.165817}
\heatmap{20.5656}{7}{0.184191}
\heatmap{20.5847}{7}{0.212281}
\heatmap{20.6038}{7}{0.242922}
\heatmap{20.623}{7}{0.278939}
\heatmap{20.6421}{7}{0.318588}
\heatmap{20.6612}{7}{0.350666}
\heatmap{20.6803}{7}{0.380027}
\heatmap{20.6995}{7}{0.406928}
\heatmap{20.7186}{7}{0.429353}
\heatmap{20.7377}{7}{0.454576}
\heatmap{20.7568}{7}{0.480513}
\heatmap{20.776}{7}{0.497727}
\heatmap{20.7951}{7}{0.524265}
\heatmap{20.8142}{7}{0.548758}
\heatmap{20.8333}{7}{0.570755}
\heatmap{20.8525}{7}{0.591237}
\heatmap{20.8716}{7}{0.612621}
\heatmap{20.8907}{7}{0.641327}
\heatmap{20.9098}{7}{0.659229}
\heatmap{20.929}{7}{0.677087}
\heatmap{20.9481}{7}{0.69209}
\heatmap{20.9672}{7}{0.705005}
\heatmap{20.9863}{7}{0.717209}
\heatmap{21.0055}{7}{0.727106}
\heatmap{21.0247}{7}{0.737134}
\heatmap{21.0438}{7}{0.746624}
\heatmap{21.063}{7}{0.762584}
\heatmap{21.0822}{7}{0.779049}
\heatmap{21.1014}{7}{0.793825}
\heatmap{21.1205}{7}{0.804526}
\heatmap{21.1397}{7}{0.807058}


==> data/tcf2-transition/onetrust/stacked/transition.tex <==
\draw (19.6466, 1) -- (19.6548, 2) -- (19.6575, 3) -- (19.6603, 3) -- (19.6658, 3) -- (19.674, 3) -- (19.6767, 3) -- (19.7808, 4) -- (19.7973, 4) -- (19.8, 4) -- (19.8137, 4) -- (19.8192, 4) -- (19.8247, 5) -- (19.8274, 5) -- (19.8329, 5) -- (19.8356, 5) -- (19.8384, 5) -- (19.8466, 5) -- (19.8493, 5) -- (19.8521, 8) -- (19.8548, 8) -- (19.8575, 8) -- (19.8658, 8) -- (19.8685, 8) -- (19.8712, 9) -- (19.874, 10) -- (19.8767, 10) -- (19.8849, 11) -- (19.8877, 11) -- (19.8904, 12) -- (19.8932, 17) -- (19.8959, 28) -- (19.8986, 28) -- (19.9014, 28) -- (19.9041, 28) -- (19.9068, 29) -- (19.9096, 29) -- (19.9123, 29) -- (19.9151, 31) -- (19.9178, 33) -- (19.9205, 33) -- (19.9233, 33) -- (19.9288, 34) -- (19.9315, 34) -- (19.9342, 34) -- (19.937, 34) -- (19.9425, 34) -- (19.9452, 34) -- (19.9479, 34) -- (19.9507, 34) -- (19.9534, 34) -- (19.9562, 34) -- (19.9589, 36) -- (19.9616, 36) -- (19.9644, 38) -- (19.9671, 41) -- (19.9699, 45) -- (19.9726, 46) -- (19.9781, 47) -- (19.9808, 47) -- (19.9836, 47) -- (19.9863, 47) -- (19.989, 48) -- (19.9918, 48) -- (19.9945, 48) -- (19.9973, 48) -- (20, 48) -- (20.0027, 49) -- (20.0055, 51) -- (20.0082, 52) -- (20.0109, 55) -- (20.0137, 55) -- (20.0164, 55) -- (20.0191, 55) -- (20.0219, 56) -- (20.0246, 57) -- (20.0273, 57) -- (20.0301, 65) -- (20.0328, 65) -- (20.0355, 66) -- (20.0383, 67) -- (20.041, 68) -- (20.0437, 69) -- (20.0464, 70) -- (20.0492, 70) -- (20.0546, 70) -- (20.0574, 71) -- (20.0601, 71) -- (20.0628, 71) -- (20.0656, 72) -- (20.0683, 72) -- (20.0738, 72) -- (20.0792, 72) -- (20.082, 72) -- (20.0847, 72) -- (20.0874, 72) -- (20.0929, 72) -- (20.1011, 73) -- (20.1038, 73) -- (20.1066, 74) -- (20.1093, 74) -- (20.112, 74) -- (20.1175, 74) -- (20.1202, 74) -- (20.123, 75) -- (20.1257, 75) -- (20.1284, 75) -- (20.1339, 75) -- (20.1366, 75) -- (20.1393, 75) -- (20.1421, 76) -- (20.1448, 76) -- (20.1475, 76) -- (20.1503, 77) -- (20.153, 77) -- (20.1585, 77) -- (20.1612, 77) -- (20.1639, 78) -- (20.1667, 78) -- (20.1694, 78) -- (20.1721, 78) -- (20.1749, 79) -- (20.1776, 79) -- (20.1803, 79) -- (20.1831, 79) -- (20.1858, 79) -- (20.1885, 79) -- (20.1913, 80) -- (20.194, 81) -- (20.1967, 82) -- (20.1995, 83) -- (20.2022, 85) -- (20.2077, 86) -- (20.2104, 90) -- (20.2131, 92) -- (20.2158, 94) -- (20.2186, 97) -- (20.2213, 99) -- (20.224, 101) -- (20.2268, 102) -- (20.2295, 103) -- (20.2322, 104) -- (20.235, 105) -- (20.2377, 106) -- (20.2404, 108) -- (20.2432, 109) -- (20.2459, 109) -- (20.2486, 109) -- (20.2514, 111) -- (20.2541, 113) -- (20.2568, 114) -- (20.2596, 114) -- (20.2623, 115) -- (20.265, 118) -- (20.2678, 120) -- (20.2705, 122) -- (20.2732, 123) -- (20.276, 126) -- (20.2787, 128) -- (20.2814, 129) -- (20.2842, 129) -- (20.2869, 130) -- (20.2896, 132) -- (20.2923, 132) -- (20.2951, 134) -- (20.2978, 135) -- (20.3005, 135) -- (20.3033, 136) -- (20.306, 138) -- (20.3087, 140) -- (20.3115, 141) -- (20.3142, 142) -- (20.3169, 144) -- (20.3197, 144) -- (20.3224, 145) -- (20.3251, 148) -- (20.3279, 150) -- (20.3306, 150) -- (20.3333, 150) -- (20.3361, 152) -- (20.3388, 153) -- (20.3415, 153) -- (20.3443, 158) -- (20.347, 159) -- (20.3497, 163) -- (20.3525, 169) -- (20.3552, 169) -- (20.3579, 174) -- (20.3607, 175) -- (20.3634, 179) -- (20.3661, 179) -- (20.3689, 181) -- (20.3716, 184) -- (20.3743, 184) -- (20.377, 189) -- (20.3798, 190) -- (20.3825, 192) -- (20.3852, 192) -- (20.388, 194) -- (20.3907, 194) -- (20.3934, 195) -- (20.3962, 198) -- (20.3989, 200) -- (20.4016, 202) -- (20.4044, 202) -- (20.4071, 203) -- (20.4098, 203) -- (20.4126, 204) -- (20.4153, 205) -- (20.418, 206) -- (20.4208, 206) -- (20.4235, 206) -- (20.4262, 207) -- (20.429, 208) -- (20.4317, 208) -- (20.4344, 208) -- (20.4372, 208) -- (20.4399, 207) -- (20.4426, 211) -- (20.4454, 214) -- (20.4481, 217) -- (20.4508, 217) -- (20.4536, 217) -- (20.4563, 218) -- (20.459, 221) -- (20.4617, 222) -- (20.4645, 223) -- (20.4672, 224) -- (20.4699, 226) -- (20.4727, 227) -- (20.4754, 228) -- (20.4781, 228) -- (20.4809, 231) -- (20.4836, 238) -- (20.4863, 240) -- (20.4891, 241) -- (20.4918, 242) -- (20.4945, 245) -- (20.4973, 248) -- (20.5, 248) -- (20.5027, 249) -- (20.5055, 248) -- (20.5082, 249) -- (20.5109, 250) -- (20.5137, 251) -- (20.5164, 252) -- (20.5191, 252) -- (20.5219, 253) -- (20.5246, 254) -- (20.5273, 254) -- (20.5301, 254) -- (20.5328, 256) -- (20.5355, 256) -- (20.5383, 257) -- (20.541, 262) -- (20.5437, 263) -- (20.5464, 262) -- (20.5492, 262) -- (20.5519, 262) -- (20.5546, 267) -- (20.5574, 270) -- (20.5601, 273) -- (20.5628, 277) -- (20.5656, 282) -- (20.5683, 282) -- (20.571, 285) -- (20.5738, 285) -- (20.5765, 287) -- (20.5792, 291) -- (20.582, 295) -- (20.5847, 301) -- (20.5874, 300) -- (20.5902, 301) -- (20.5929, 305) -- (20.5956, 306) -- (20.5984, 307) -- (20.6011, 307) -- (20.6038, 298) -- (20.6066, 295) -- (20.6093, 290) -- (20.612, 284) -- (20.6148, 280) -- (20.6175, 260) -- (20.6202, 244) -- (20.623, 235) -- (20.6257, 231) -- (20.6284, 228) -- (20.6311, 219) -- (20.6339, 215) -- (20.6366, 205) -- (20.6393, 201) -- (20.6421, 193) -- (20.6448, 188) -- (20.6475, 188) -- (20.6503, 185) -- (20.653, 183) -- (20.6557, 183) -- (20.6585, 182) -- (20.6612, 179) -- (20.6639, 177) -- (20.6667, 176) -- (20.6694, 175) -- (20.6721, 175) -- (20.6749, 174) -- (20.6776, 171) -- (20.6803, 171) -- (20.6831, 170) -- (20.6858, 167) -- (20.6885, 166) -- (20.6913, 162) -- (20.694, 161) -- (20.6967, 161) -- (20.6995, 160) -- (20.7022, 158) -- (20.7049, 149) -- (20.7077, 141) -- (20.7104, 141) -- (20.7131, 140) -- (20.7158, 140) -- (20.7186, 140) -- (20.7213, 139) -- (20.724, 138) -- (20.7268, 137) -- (20.7295, 136) -- (20.7322, 136) -- (20.735, 135) -- (20.7377, 134) -- (20.7404, 134) -- (20.7432, 133) -- (20.7459, 132) -- (20.7486, 131) -- (20.7514, 130) -- (20.7541, 128) -- (20.7568, 127) -- (20.7623, 126) -- (20.765, 125) -- (20.7678, 126) -- (20.7705, 124) -- (20.7732, 123) -- (20.776, 123) -- (20.7787, 122) -- (20.7814, 121) -- (20.7842, 119) -- (20.7869, 118) -- (20.7896, 115) -- (20.7923, 115) -- (20.7951, 113) -- (20.7978, 113) -- (20.8005, 112) -- (20.8033, 110) -- (20.806, 110) -- (20.8087, 109) -- (20.8115, 108) -- (20.8142, 108) -- (20.8169, 107) -- (20.8197, 106) -- (20.8224, 107) -- (20.8251, 107) -- (20.8279, 107) -- (20.8306, 106) -- (20.8333, 106) -- (20.8361, 106) -- (20.8388, 106) -- (20.8415, 106) -- (20.8443, 106) -- (20.847, 105) -- (20.8497, 104) -- (20.8525, 103) -- (20.8552, 101) -- (20.8579, 101) -- (20.8607, 100) -- (20.8634, 101) -- (20.8661, 101) -- (20.8689, 100) -- (20.8716, 100) -- (20.8743, 98) -- (20.877, 97) -- (20.8798, 97) -- (20.8825, 97) -- (20.8852, 97) -- (20.888, 97) -- (20.8907, 97) -- (20.8934, 97) -- (20.8962, 97) -- (20.8989, 97) -- (20.9016, 96) -- (20.9044, 96) -- (20.9071, 96) -- (20.9098, 95) -- (20.9126, 94) -- (20.9153, 92) -- (20.918, 92) -- (20.9208, 91) -- (20.9235, 90) -- (20.9262, 90) -- (20.929, 86) -- (20.9317, 86) -- (20.9344, 86) -- (20.9372, 84) -- (20.9399, 84) -- (20.9426, 84) -- (20.9454, 84) -- (20.9481, 84) -- (20.9508, 84) -- (20.9536, 83) -- (20.9563, 83) -- (20.959, 82) -- (20.9617, 82) -- (20.9645, 80) -- (20.9672, 79) -- (20.9699, 78) -- (20.9727, 77) -- (20.9754, 76) -- (20.9781, 75) -- (20.9809, 74) -- (20.9836, 74) -- (20.9863, 74) -- (20.9891, 74) -- (20.9918, 73) -- (20.9945, 72) -- (20.9973, 72) -- (21, 71) -- (21.0027, 71) -- (21.0055, 71) -- (21.0082, 71) -- (21.011, 70) -- (21.0137, 70) -- (21.0164, 70) -- (21.0192, 70) -- (21.0219, 70) -- (21.0247, 69) -- (21.0274, 69) -- (21.0301, 69) -- (21.0329, 68) -- (21.0356, 65) -- (21.0384, 65) -- (21.0411, 64) -- (21.0438, 63) -- (21.0466, 62) -- (21.0493, 62) -- (21.0521, 59) -- (21.0548, 59) -- (21.0575, 58) -- (21.0603, 58) -- (21.063, 58) -- (21.0658, 58) -- (21.0685, 58) -- (21.0712, 58) -- (21.074, 57) -- (21.0767, 57) -- (21.0795, 57) -- (21.0822, 57) -- (21.0849, 55) -- (21.0877, 55) -- (21.0904, 53) -- (21.0932, 52) -- (21.0959, 52) -- (21.0986, 52) -- (21.1014, 52) -- (21.1041, 51) -- (21.1068, 51) -- (21.1096, 51) -- (21.1123, 51) -- (21.1151, 50) -- (21.1178, 48) -- (21.1205, 48) -- (21.1233, 47) -- (21.126, 46) -- (21.1288, 46) -- (21.1315, 45) -- (21.1342, 42) -- (21.1342, 0) -- (19.6466, 0) -- cycle;

==> data/tcf2-transition/onetrust/stacked/v1.tex <==
\draw (19.6466, 1) -- (19.6548, 2) -- (19.6575, 3) -- (19.6603, 3) -- (19.6658, 3) -- (19.674, 3) -- (19.6767, 3) -- (19.7808, 4) -- (19.7973, 4) -- (19.8, 4) -- (19.8137, 4) -- (19.8192, 4) -- (19.8247, 5) -- (19.8274, 5) -- (19.8329, 5) -- (19.8356, 5) -- (19.8384, 5) -- (19.8466, 5) -- (19.8493, 5) -- (19.8521, 8) -- (19.8548, 8) -- (19.8575, 8) -- (19.8658, 8) -- (19.8685, 8) -- (19.8712, 9) -- (19.874, 10) -- (19.8767, 10) -- (19.8849, 11) -- (19.8877, 11) -- (19.8904, 12) -- (19.8932, 17) -- (19.8959, 28) -- (19.8986, 28) -- (19.9014, 28) -- (19.9041, 28) -- (19.9068, 29) -- (19.9096, 29) -- (19.9123, 29) -- (19.9151, 31) -- (19.9178, 33) -- (19.9205, 33) -- (19.9233, 33) -- (19.9288, 34) -- (19.9315, 34) -- (19.9342, 34) -- (19.937, 34) -- (19.9425, 34) -- (19.9452, 34) -- (19.9479, 34) -- (19.9507, 34) -- (19.9534, 34) -- (19.9562, 34) -- (19.9589, 36) -- (19.9616, 36) -- (19.9644, 38) -- (19.9671, 41) -- (19.9699, 45) -- (19.9726, 46) -- (19.9781, 47) -- (19.9808, 47) -- (19.9836, 47) -- (19.9863, 47) -- (19.989, 48) -- (19.9918, 48) -- (19.9945, 48) -- (19.9973, 48) -- (20, 48) -- (20.0027, 49) -- (20.0055, 50) -- (20.0082, 51) -- (20.0109, 54) -- (20.0137, 54) -- (20.0164, 54) -- (20.0191, 54) -- (20.0219, 55) -- (20.0246, 56) -- (20.0273, 56) -- (20.0301, 64) -- (20.0328, 64) -- (20.0355, 65) -- (20.0383, 66) -- (20.041, 67) -- (20.0437, 68) -- (20.0464, 69) -- (20.0492, 69) -- (20.0546, 69) -- (20.0574, 70) -- (20.0601, 70) -- (20.0628, 70) -- (20.0656, 71) -- (20.0683, 71) -- (20.0738, 71) -- (20.0792, 71) -- (20.082, 71) -- (20.0847, 71) -- (20.0874, 71) -- (20.0929, 71) -- (20.1011, 72) -- (20.1038, 72) -- (20.1066, 73) -- (20.1093, 73) -- (20.112, 73) -- (20.1175, 72) -- (20.1202, 72) -- (20.123, 73) -- (20.1257, 73) -- (20.1284, 73) -- (20.1339, 73) -- (20.1366, 73) -- (20.1393, 73) -- (20.1421, 74) -- (20.1448, 74) -- (20.1475, 74) -- (20.1503, 75) -- (20.153, 75) -- (20.1585, 75) -- (20.1612, 75) -- (20.1639, 76) -- (20.1667, 76) -- (20.1694, 76) -- (20.1721, 76) -- (20.1749, 77) -- (20.1776, 77) -- (20.1803, 77) -- (20.1831, 77) -- (20.1858, 77) -- (20.1885, 77) -- (20.1913, 78) -- (20.194, 79) -- (20.1967, 80) -- (20.1995, 80) -- (20.2022, 82) -- (20.2077, 83) -- (20.2104, 87) -- (20.2131, 88) -- (20.2158, 90) -- (20.2186, 93) -- (20.2213, 95) -- (20.224, 97) -- (20.2268, 98) -- (20.2295, 99) -- (20.2322, 100) -- (20.235, 101) -- (20.2377, 102) -- (20.2404, 104) -- (20.2432, 105) -- (20.2459, 105) -- (20.2486, 105) -- (20.2514, 107) -- (20.2541, 109) -- (20.2568, 110) -- (20.2596, 110) -- (20.2623, 111) -- (20.265, 114) -- (20.2678, 116) -- (20.2705, 117) -- (20.2732, 118) -- (20.276, 120) -- (20.2787, 121) -- (20.2814, 122) -- (20.2842, 122) -- (20.2869, 123) -- (20.2896, 125) -- (20.2923, 124) -- (20.2951, 126) -- (20.2978, 127) -- (20.3005, 127) -- (20.3033, 128) -- (20.306, 130) -- (20.3087, 131) -- (20.3115, 132) -- (20.3142, 132) -- (20.3169, 133) -- (20.3197, 131) -- (20.3224, 132) -- (20.3251, 134) -- (20.3279, 136) -- (20.3306, 136) -- (20.3333, 136) -- (20.3361, 138) -- (20.3388, 138) -- (20.3415, 137) -- (20.3443, 141) -- (20.347, 141) -- (20.3497, 145) -- (20.3525, 150) -- (20.3552, 151) -- (20.3579, 156) -- (20.3607, 157) -- (20.3634, 160) -- (20.3661, 158) -- (20.3689, 160) -- (20.3716, 163) -- (20.3743, 164) -- (20.377, 169) -- (20.3798, 169) -- (20.3825, 168) -- (20.3852, 167) -- (20.388, 169) -- (20.3907, 169) -- (20.3934, 170) -- (20.3962, 173) -- (20.3989, 175) -- (20.4016, 177) -- (20.4044, 176) -- (20.4071, 176) -- (20.4098, 176) -- (20.4126, 177) -- (20.4153, 177) -- (20.418, 178) -- (20.4208, 177) -- (20.4235, 177) -- (20.4262, 178) -- (20.429, 179) -- (20.4317, 179) -- (20.4344, 179) -- (20.4372, 179) -- (20.4399, 179) -- (20.4426, 183) -- (20.4454, 185) -- (20.4481, 186) -- (20.4508, 186) -- (20.4536, 186) -- (20.4563, 187) -- (20.459, 190) -- (20.4617, 188) -- (20.4645, 188) -- (20.4672, 187) -- (20.4699, 189) -- (20.4727, 190) -- (20.4754, 191) -- (20.4781, 190) -- (20.4809, 193) -- (20.4836, 200) -- (20.4863, 200) -- (20.4891, 200) -- (20.4918, 201) -- (20.4945, 203) -- (20.4973, 203) -- (20.5, 200) -- (20.5027, 202) -- (20.5055, 201) -- (20.5082, 204) -- (20.5109, 204) -- (20.5137, 204) -- (20.5164, 203) -- (20.5191, 203) -- (20.5219, 205) -- (20.5246, 205) -- (20.5273, 205) -- (20.5301, 204) -- (20.5328, 204) -- (20.5355, 204) -- (20.5383, 205) -- (20.541, 210) -- (20.5437, 209) -- (20.5464, 206) -- (20.5492, 205) -- (20.5519, 205) -- (20.5546, 209) -- (20.5574, 212) -- (20.5601, 215) -- (20.5628, 216) -- (20.5656, 221) -- (20.5683, 213) -- (20.571, 215) -- (20.5738, 212) -- (20.5765, 214) -- (20.5792, 218) -- (20.582, 219) -- (20.5847, 220) -- (20.5874, 210) -- (20.5902, 209) -- (20.5929, 210) -- (20.5956, 203) -- (20.5984, 198) -- (20.6011, 189) -- (20.6038, 174) -- (20.6066, 143) -- (20.6093, 139) -- (20.612, 138) -- (20.6148, 133) -- (20.6175, 121) -- (20.6202, 116) -- (20.623, 115) -- (20.6257, 114) -- (20.6284, 113) -- (20.6311, 113) -- (20.6339, 112) -- (20.6366, 108) -- (20.6393, 106) -- (20.6421, 106) -- (20.6448, 106) -- (20.6475, 108) -- (20.6503, 107) -- (20.653, 106) -- (20.6557, 107) -- (20.6585, 107) -- (20.6612, 107) -- (20.6639, 107) -- (20.6667, 107) -- (20.6694, 107) -- (20.6721, 105) -- (20.6749, 105) -- (20.6776, 104) -- (20.6803, 103) -- (20.6831, 103) -- (20.6858, 103) -- (20.6885, 103) -- (20.6913, 102) -- (20.694, 101) -- (20.6967, 98) -- (20.6995, 97) -- (20.7022, 96) -- (20.7049, 89) -- (20.7077, 89) -- (20.7104, 89) -- (20.7131, 89) -- (20.7158, 89) -- (20.7186, 89) -- (20.7213, 89) -- (20.724, 90) -- (20.7268, 90) -- (20.7295, 90) -- (20.7322, 90) -- (20.735, 90) -- (20.7377, 90) -- (20.7404, 90) -- (20.7432, 90) -- (20.7459, 90) -- (20.7486, 90) -- (20.7514, 89) -- (20.7541, 88) -- (20.7568, 88) -- (20.7623, 88) -- (20.765, 87) -- (20.7678, 88) -- (20.7705, 88) -- (20.7732, 88) -- (20.776, 88) -- (20.7787, 88) -- (20.7814, 87) -- (20.7842, 87) -- (20.7869, 86) -- (20.7896, 84) -- (20.7923, 84) -- (20.7951, 84) -- (20.7978, 84) -- (20.8005, 84) -- (20.8033, 82) -- (20.806, 82) -- (20.8087, 81) -- (20.8115, 81) -- (20.8142, 81) -- (20.8169, 81) -- (20.8197, 80) -- (20.8224, 81) -- (20.8251, 81) -- (20.8279, 80) -- (20.8306, 80) -- (20.8333, 80) -- (20.8361, 80) -- (20.8388, 80) -- (20.8415, 80) -- (20.8443, 80) -- (20.847, 80) -- (20.8497, 80) -- (20.8525, 79) -- (20.8552, 79) -- (20.8579, 79) -- (20.8607, 78) -- (20.8634, 79) -- (20.8661, 79) -- (20.8689, 79) -- (20.8716, 79) -- (20.8743, 79) -- (20.877, 78) -- (20.8798, 78) -- (20.8825, 78) -- (20.8852, 78) -- (20.888, 78) -- (20.8907, 78) -- (20.8934, 78) -- (20.8962, 78) -- (20.8989, 78) -- (20.9016, 78) -- (20.9044, 78) -- (20.9071, 78) -- (20.9098, 77) -- (20.9126, 77) -- (20.9153, 76) -- (20.918, 76) -- (20.9208, 75) -- (20.9235, 75) -- (20.9262, 75) -- (20.929, 71) -- (20.9317, 71) -- (20.9344, 71) -- (20.9372, 71) -- (20.9399, 71) -- (20.9426, 72) -- (20.9454, 72) -- (20.9481, 72) -- (20.9508, 72) -- (20.9536, 71) -- (20.9563, 71) -- (20.959, 70) -- (20.9617, 70) -- (20.9645, 70) -- (20.9672, 70) -- (20.9699, 69) -- (20.9727, 68) -- (20.9754, 67) -- (20.9781, 66) -- (20.9809, 66) -- (20.9836, 66) -- (20.9863, 66) -- (20.9891, 66) -- (20.9918, 66) -- (20.9945, 65) -- (20.9973, 65) -- (21, 64) -- (21.0027, 64) -- (21.0055, 64) -- (21.0082, 64) -- (21.011, 63) -- (21.0137, 63) -- (21.0164, 63) -- (21.0192, 63) -- (21.0219, 63) -- (21.0247, 62) -- (21.0274, 62) -- (21.0301, 62) -- (21.0329, 61) -- (21.0356, 59) -- (21.0384, 59) -- (21.0411, 58) -- (21.0438, 57) -- (21.0466, 56) -- (21.0493, 56) -- (21.0521, 55) -- (21.0548, 55) -- (21.0575, 55) -- (21.0603, 55) -- (21.063, 55) -- (21.0658, 55) -- (21.0685, 55) -- (21.0712, 55) -- (21.074, 54) -- (21.0767, 54) -- (21.0795, 54) -- (21.0822, 54) -- (21.0849, 53) -- (21.0877, 53) -- (21.0904, 52) -- (21.0932, 51) -- (21.0959, 51) -- (21.0986, 51) -- (21.1014, 51) -- (21.1041, 50) -- (21.1068, 50) -- (21.1096, 50) -- (21.1123, 50) -- (21.1151, 50) -- (21.1178, 48) -- (21.1205, 48) -- (21.1233, 47) -- (21.126, 46) -- (21.1288, 46) -- (21.1315, 45) -- (21.1342, 42) -- (21.1342, 0) -- (19.6466, 0) -- cycle;

==> data/tcf2-transition/onetrust/stacked/v2-new.tex <==
\draw (19.6466, 1) -- (19.6548, 2) -- (19.6575, 3) -- (19.6603, 3) -- (19.6658, 3) -- (19.674, 3) -- (19.6767, 3) -- (19.7808, 4) -- (19.7973, 4) -- (19.8, 4) -- (19.8137, 4) -- (19.8192, 4) -- (19.8247, 5) -- (19.8274, 5) -- (19.8329, 5) -- (19.8356, 5) -- (19.8384, 5) -- (19.8466, 5) -- (19.8493, 5) -- (19.8521, 8) -- (19.8548, 8) -- (19.8575, 8) -- (19.8658, 8) -- (19.8685, 8) -- (19.8712, 9) -- (19.874, 10) -- (19.8767, 10) -- (19.8849, 11) -- (19.8877, 11) -- (19.8904, 12) -- (19.8932, 17) -- (19.8959, 28) -- (19.8986, 28) -- (19.9014, 28) -- (19.9041, 28) -- (19.9068, 29) -- (19.9096, 29) -- (19.9123, 29) -- (19.9151, 31) -- (19.9178, 33) -- (19.9205, 33) -- (19.9233, 33) -- (19.9288, 34) -- (19.9315, 34) -- (19.9342, 34) -- (19.937, 34) -- (19.9425, 34) -- (19.9452, 34) -- (19.9479, 34) -- (19.9507, 34) -- (19.9534, 34) -- (19.9562, 34) -- (19.9589, 36) -- (19.9616, 36) -- (19.9644, 38) -- (19.9671, 41) -- (19.9699, 45) -- (19.9726, 46) -- (19.9781, 47) -- (19.9808, 47) -- (19.9836, 47) -- (19.9863, 47) -- (19.989, 48) -- (19.9918, 48) -- (19.9945, 48) -- (19.9973, 48) -- (20, 48) -- (20.0027, 49) -- (20.0055, 51) -- (20.0082, 52) -- (20.0109, 55) -- (20.0137, 55) -- (20.0164, 55) -- (20.0191, 55) -- (20.0219, 56) -- (20.0246, 57) -- (20.0273, 57) -- (20.0301, 65) -- (20.0328, 65) -- (20.0355, 66) -- (20.0383, 67) -- (20.041, 68) -- (20.0437, 69) -- (20.0464, 70) -- (20.0492, 70) -- (20.0546, 70) -- (20.0574, 71) -- (20.0601, 71) -- (20.0628, 71) -- (20.0656, 72) -- (20.0683, 72) -- (20.0738, 72) -- (20.0792, 72) -- (20.082, 72) -- (20.0847, 72) -- (20.0874, 72) -- (20.0929, 72) -- (20.1011, 73) -- (20.1038, 73) -- (20.1066, 74) -- (20.1093, 74) -- (20.112, 74) -- (20.1175, 74) -- (20.1202, 74) -- (20.123, 75) -- (20.1257, 75) -- (20.1284, 75) -- (20.1339, 75) -- (20.1366, 75) -- (20.1393, 75) -- (20.1421, 76) -- (20.1448, 76) -- (20.1475, 76) -- (20.1503, 77) -- (20.153, 77) -- (20.1585, 77) -- (20.1612, 77) -- (20.1639, 78) -- (20.1667, 78) -- (20.1694, 78) -- (20.1721, 78) -- (20.1749, 79) -- (20.1776, 79) -- (20.1803, 79) -- (20.1831, 79) -- (20.1858, 79) -- (20.1885, 79) -- (20.1913, 80) -- (20.194, 81) -- (20.1967, 82) -- (20.1995, 83) -- (20.2022, 85) -- (20.2077, 86) -- (20.2104, 90) -- (20.2131, 92) -- (20.2158, 94) -- (20.2186, 97) -- (20.2213, 99) -- (20.224, 101) -- (20.2268, 102) -- (20.2295, 103) -- (20.2322, 104) -- (20.235, 105) -- (20.2377, 106) -- (20.2404, 108) -- (20.2432, 109) -- (20.2459, 109) -- (20.2486, 109) -- (20.2514, 111) -- (20.2541, 113) -- (20.2568, 114) -- (20.2596, 114) -- (20.2623, 115) -- (20.265, 118) -- (20.2678, 120) -- (20.2705, 122) -- (20.2732, 123) -- (20.276, 126) -- (20.2787, 128) -- (20.2814, 129) -- (20.2842, 129) -- (20.2869, 130) -- (20.2896, 132) -- (20.2923, 132) -- (20.2951, 134) -- (20.2978, 135) -- (20.3005, 135) -- (20.3033, 136) -- (20.306, 138) -- (20.3087, 140) -- (20.3115, 141) -- (20.3142, 142) -- (20.3169, 144) -- (20.3197, 144) -- (20.3224, 145) -- (20.3251, 148) -- (20.3279, 150) -- (20.3306, 150) -- (20.3333, 150) -- (20.3361, 152) -- (20.3388, 153) -- (20.3415, 153) -- (20.3443, 159) -- (20.347, 161) -- (20.3497, 165) -- (20.3525, 171) -- (20.3552, 172) -- (20.3579, 177) -- (20.3607, 178) -- (20.3634, 182) -- (20.3661, 182) -- (20.3689, 185) -- (20.3716, 189) -- (20.3743, 190) -- (20.377, 195) -- (20.3798, 196) -- (20.3825, 198) -- (20.3852, 198) -- (20.388, 200) -- (20.3907, 201) -- (20.3934, 202) -- (20.3962, 205) -- (20.3989, 207) -- (20.4016, 210) -- (20.4044, 211) -- (20.4071, 212) -- (20.4098, 213) -- (20.4126, 215) -- (20.4153, 216) -- (20.418, 217) -- (20.4208, 218) -- (20.4235, 218) -- (20.4262, 220) -- (20.429, 221) -- (20.4317, 221) -- (20.4344, 221) -- (20.4372, 221) -- (20.4399, 221) -- (20.4426, 225) -- (20.4454, 228) -- (20.4481, 232) -- (20.4508, 232) -- (20.4536, 232) -- (20.4563, 233) -- (20.459, 236) -- (20.4617, 238) -- (20.4645, 241) -- (20.4672, 242) -- (20.4699, 244) -- (20.4727, 245) -- (20.4754, 249) -- (20.4781, 251) -- (20.4809, 258) -- (20.4836, 269) -- (20.4863, 275) -- (20.4891, 276) -- (20.4918, 279) -- (20.4945, 285) -- (20.4973, 289) -- (20.5, 291) -- (20.5027, 298) -- (20.5055, 302) -- (20.5082, 308) -- (20.5109, 310) -- (20.5137, 313) -- (20.5164, 316) -- (20.5191, 316) -- (20.5219, 321) -- (20.5246, 323) -- (20.5273, 323) -- (20.5301, 323) -- (20.5328, 325) -- (20.5355, 326) -- (20.5383, 327) -- (20.541, 332) -- (20.5437, 336) -- (20.5464, 337) -- (20.5492, 338) -- (20.5519, 339) -- (20.5546, 350) -- (20.5574, 362) -- (20.5601, 371) -- (20.5628, 385) -- (20.5656, 398) -- (20.5683, 402) -- (20.571, 409) -- (20.5738, 416) -- (20.5765, 422) -- (20.5792, 434) -- (20.582, 446) -- (20.5847, 461) -- (20.5874, 463) -- (20.5902, 471) -- (20.5929, 480) -- (20.5956, 486) -- (20.5984, 495) -- (20.6011, 499) -- (20.6038, 508) -- (20.6066, 510) -- (20.6093, 523) -- (20.612, 543) -- (20.6148, 570) -- (20.6175, 598) -- (20.6202, 624) -- (20.623, 653) -- (20.6257, 659) -- (20.6284, 672) -- (20.6311, 683) -- (20.6339, 693) -- (20.6366, 704) -- (20.6393, 712) -- (20.6421, 721) -- (20.6448, 729) -- (20.6475, 739) -- (20.6503, 744) -- (20.653, 747) -- (20.6557, 754) -- (20.6585, 758) -- (20.6612, 764) -- (20.6639, 771) -- (20.6667, 780) -- (20.6694, 792) -- (20.6721, 799) -- (20.6749, 807) -- (20.6776, 809) -- (20.6803, 813) -- (20.6831, 820) -- (20.6858, 824) -- (20.6885, 840) -- (20.6913, 846) -- (20.694, 856) -- (20.6967, 863) -- (20.6995, 865) -- (20.7022, 872) -- (20.7049, 878) -- (20.7077, 885) -- (20.7104, 895) -- (20.7131, 900) -- (20.7158, 904) -- (20.7186, 910) -- (20.7213, 915) -- (20.724, 918) -- (20.7268, 923) -- (20.7295, 929) -- (20.7322, 939) -- (20.735, 951) -- (20.7377, 960) -- (20.7404, 966) -- (20.7432, 976) -- (20.7459, 984) -- (20.7486, 995) -- (20.7514, 1005) -- (20.7541, 1017) -- (20.7568, 1024) -- (20.7623, 1047) -- (20.765, 1061) -- (20.7678, 1073) -- (20.7705, 1082) -- (20.7732, 1087) -- (20.776, 1093) -- (20.7787, 1098) -- (20.7814, 1101) -- (20.7842, 1107) -- (20.7869, 1110) -- (20.7896, 1117) -- (20.7923, 1120) -- (20.7951, 1124) -- (20.7978, 1129) -- (20.8005, 1131) -- (20.8033, 1136) -- (20.806, 1143) -- (20.8087, 1151) -- (20.8115, 1155) -- (20.8142, 1158) -- (20.8169, 1169) -- (20.8197, 1175) -- (20.8224, 1183) -- (20.8251, 1189) -- (20.8279, 1196) -- (20.8306, 1202) -- (20.8333, 1204) -- (20.8361, 1208) -- (20.8388, 1215) -- (20.8415, 1221) -- (20.8443, 1230) -- (20.847, 1237) -- (20.8497, 1243) -- (20.8525, 1246) -- (20.8552, 1253) -- (20.8579, 1262) -- (20.8607, 1265) -- (20.8634, 1273) -- (20.8661, 1278) -- (20.8689, 1283) -- (20.8716, 1291) -- (20.8743, 1299) -- (20.877, 1302) -- (20.8798, 1315) -- (20.8825, 1322) -- (20.8852, 1326) -- (20.888, 1330) -- (20.8907, 1333) -- (20.8934, 1339) -- (20.8962, 1341) -- (20.8989, 1345) -- (20.9016, 1348) -- (20.9044, 1352) -- (20.9071, 1361) -- (20.9098, 1364) -- (20.9126, 1370) -- (20.9153, 1372) -- (20.918, 1375) -- (20.9208, 1380) -- (20.9235, 1384) -- (20.9262, 1390) -- (20.929, 1389) -- (20.9317, 1393) -- (20.9344, 1397) -- (20.9372, 1405) -- (20.9399, 1412) -- (20.9426, 1421) -- (20.9454, 1428) -- (20.9481, 1433) -- (20.9508, 1439) -- (20.9536, 1445) -- (20.9563, 1448) -- (20.959, 1450) -- (20.9617, 1455) -- (20.9645, 1458) -- (20.9672, 1462) -- (20.9699, 1466) -- (20.9727, 1472) -- (20.9754, 1479) -- (20.9781, 1480) -- (20.9809, 1482) -- (20.9836, 1488) -- (20.9863, 1491) -- (20.9891, 1495) -- (20.9918, 1499) -- (20.9945, 1501) -- (20.9973, 1505) -- (21, 1506) -- (21.0027, 1510) -- (21.0055, 1511) -- (21.0082, 1514) -- (21.011, 1518) -- (21.0137, 1522) -- (21.0164, 1526) -- (21.0192, 1530) -- (21.0219, 1534) -- (21.0247, 1536) -- (21.0274, 1542) -- (21.0301, 1549) -- (21.0329, 1558) -- (21.0356, 1560) -- (21.0384, 1567) -- (21.0411, 1576) -- (21.0438, 1581) -- (21.0466, 1584) -- (21.0493, 1593) -- (21.0521, 1601) -- (21.0548, 1605) -- (21.0575, 1613) -- (21.0603, 1615) -- (21.063, 1620) -- (21.0658, 1629) -- (21.0685, 1634) -- (21.0712, 1639) -- (21.074, 1642) -- (21.0767, 1651) -- (21.0795, 1656) -- (21.0822, 1656) -- (21.0849, 1656) -- (21.0877, 1659) -- (21.0904, 1663) -- (21.0932, 1668) -- (21.0959, 1670) -- (21.0986, 1675) -- (21.1014, 1678) -- (21.1041, 1678) -- (21.1068, 1681) -- (21.1096, 1684) -- (21.1123, 1687) -- (21.1151, 1692) -- (21.1178, 1691) -- (21.1205, 1692) -- (21.1233, 1692) -- (21.126, 1693) -- (21.1288, 1699) -- (21.1315, 1701) -- (21.1342, 1704) -- (21.1342, 0) -- (19.6466, 0) -- cycle;

==> data/tcf2-transition/onetrust/stacked/v2-switch.tex <==
\draw (19.6466, 1) -- (19.6548, 2) -- (19.6575, 3) -- (19.6603, 3) -- (19.6658, 3) -- (19.674, 3) -- (19.6767, 3) -- (19.7808, 4) -- (19.7973, 4) -- (19.8, 4) -- (19.8137, 4) -- (19.8192, 4) -- (19.8247, 5) -- (19.8274, 5) -- (19.8329, 5) -- (19.8356, 5) -- (19.8384, 5) -- (19.8466, 5) -- (19.8493, 5) -- (19.8521, 8) -- (19.8548, 8) -- (19.8575, 8) -- (19.8658, 8) -- (19.8685, 8) -- (19.8712, 9) -- (19.874, 10) -- (19.8767, 10) -- (19.8849, 11) -- (19.8877, 11) -- (19.8904, 12) -- (19.8932, 17) -- (19.8959, 28) -- (19.8986, 28) -- (19.9014, 28) -- (19.9041, 28) -- (19.9068, 29) -- (19.9096, 29) -- (19.9123, 29) -- (19.9151, 31) -- (19.9178, 33) -- (19.9205, 33) -- (19.9233, 33) -- (19.9288, 34) -- (19.9315, 34) -- (19.9342, 34) -- (19.937, 34) -- (19.9425, 34) -- (19.9452, 34) -- (19.9479, 34) -- (19.9507, 34) -- (19.9534, 34) -- (19.9562, 34) -- (19.9589, 36) -- (19.9616, 36) -- (19.9644, 38) -- (19.9671, 41) -- (19.9699, 45) -- (19.9726, 46) -- (19.9781, 47) -- (19.9808, 47) -- (19.9836, 47) -- (19.9863, 47) -- (19.989, 48) -- (19.9918, 48) -- (19.9945, 48) -- (19.9973, 48) -- (20, 48) -- (20.0027, 49) -- (20.0055, 51) -- (20.0082, 52) -- (20.0109, 55) -- (20.0137, 55) -- (20.0164, 55) -- (20.0191, 55) -- (20.0219, 56) -- (20.0246, 57) -- (20.0273, 57) -- (20.0301, 65) -- (20.0328, 65) -- (20.0355, 66) -- (20.0383, 67) -- (20.041, 68) -- (20.0437, 69) -- (20.0464, 70) -- (20.0492, 70) -- (20.0546, 70) -- (20.0574, 71) -- (20.0601, 71) -- (20.0628, 71) -- (20.0656, 72) -- (20.0683, 72) -- (20.0738, 72) -- (20.0792, 72) -- (20.082, 72) -- (20.0847, 72) -- (20.0874, 72) -- (20.0929, 72) -- (20.1011, 73) -- (20.1038, 73) -- (20.1066, 74) -- (20.1093, 74) -- (20.112, 74) -- (20.1175, 74) -- (20.1202, 74) -- (20.123, 75) -- (20.1257, 75) -- (20.1284, 75) -- (20.1339, 75) -- (20.1366, 75) -- (20.1393, 75) -- (20.1421, 76) -- (20.1448, 76) -- (20.1475, 76) -- (20.1503, 77) -- (20.153, 77) -- (20.1585, 77) -- (20.1612, 77) -- (20.1639, 78) -- (20.1667, 78) -- (20.1694, 78) -- (20.1721, 78) -- (20.1749, 79) -- (20.1776, 79) -- (20.1803, 79) -- (20.1831, 79) -- (20.1858, 79) -- (20.1885, 79) -- (20.1913, 80) -- (20.194, 81) -- (20.1967, 82) -- (20.1995, 83) -- (20.2022, 85) -- (20.2077, 86) -- (20.2104, 90) -- (20.2131, 92) -- (20.2158, 94) -- (20.2186, 97) -- (20.2213, 99) -- (20.224, 101) -- (20.2268, 102) -- (20.2295, 103) -- (20.2322, 104) -- (20.235, 105) -- (20.2377, 106) -- (20.2404, 108) -- (20.2432, 109) -- (20.2459, 109) -- (20.2486, 109) -- (20.2514, 111) -- (20.2541, 113) -- (20.2568, 114) -- (20.2596, 114) -- (20.2623, 115) -- (20.265, 118) -- (20.2678, 120) -- (20.2705, 122) -- (20.2732, 123) -- (20.276, 126) -- (20.2787, 128) -- (20.2814, 129) -- (20.2842, 129) -- (20.2869, 130) -- (20.2896, 132) -- (20.2923, 132) -- (20.2951, 134) -- (20.2978, 135) -- (20.3005, 135) -- (20.3033, 136) -- (20.306, 138) -- (20.3087, 140) -- (20.3115, 141) -- (20.3142, 142) -- (20.3169, 144) -- (20.3197, 144) -- (20.3224, 145) -- (20.3251, 148) -- (20.3279, 150) -- (20.3306, 150) -- (20.3333, 150) -- (20.3361, 152) -- (20.3388, 153) -- (20.3415, 153) -- (20.3443, 158) -- (20.347, 159) -- (20.3497, 163) -- (20.3525, 169) -- (20.3552, 170) -- (20.3579, 175) -- (20.3607, 176) -- (20.3634, 180) -- (20.3661, 180) -- (20.3689, 182) -- (20.3716, 185) -- (20.3743, 186) -- (20.377, 191) -- (20.3798, 192) -- (20.3825, 194) -- (20.3852, 194) -- (20.388, 196) -- (20.3907, 196) -- (20.3934, 197) -- (20.3962, 200) -- (20.3989, 202) -- (20.4016, 204) -- (20.4044, 204) -- (20.4071, 205) -- (20.4098, 206) -- (20.4126, 207) -- (20.4153, 208) -- (20.418, 209) -- (20.4208, 209) -- (20.4235, 209) -- (20.4262, 210) -- (20.429, 211) -- (20.4317, 211) -- (20.4344, 211) -- (20.4372, 211) -- (20.4399, 211) -- (20.4426, 215) -- (20.4454, 218) -- (20.4481, 221) -- (20.4508, 221) -- (20.4536, 221) -- (20.4563, 222) -- (20.459, 225) -- (20.4617, 226) -- (20.4645, 227) -- (20.4672, 228) -- (20.4699, 230) -- (20.4727, 231) -- (20.4754, 232) -- (20.4781, 232) -- (20.4809, 235) -- (20.4836, 242) -- (20.4863, 244) -- (20.4891, 245) -- (20.4918, 246) -- (20.4945, 249) -- (20.4973, 252) -- (20.5, 252) -- (20.5027, 254) -- (20.5055, 255) -- (20.5082, 258) -- (20.5109, 259) -- (20.5137, 260) -- (20.5164, 261) -- (20.5191, 261) -- (20.5219, 263) -- (20.5246, 264) -- (20.5273, 264) -- (20.5301, 264) -- (20.5328, 266) -- (20.5355, 266) -- (20.5383, 267) -- (20.541, 272) -- (20.5437, 273) -- (20.5464, 273) -- (20.5492, 273) -- (20.5519, 273) -- (20.5546, 278) -- (20.5574, 281) -- (20.5601, 284) -- (20.5628, 288) -- (20.5656, 294) -- (20.5683, 294) -- (20.571, 297) -- (20.5738, 298) -- (20.5765, 302) -- (20.5792, 308) -- (20.582, 313) -- (20.5847, 319) -- (20.5874, 319) -- (20.5902, 320) -- (20.5929, 325) -- (20.5956, 327) -- (20.5984, 331) -- (20.6011, 332) -- (20.6038, 334) -- (20.6066, 332) -- (20.6093, 332) -- (20.612, 335) -- (20.6148, 335) -- (20.6175, 335) -- (20.6202, 335) -- (20.623, 337) -- (20.6257, 338) -- (20.6284, 338) -- (20.6311, 338) -- (20.6339, 338) -- (20.6366, 337) -- (20.6393, 336) -- (20.6421, 336) -- (20.6448, 336) -- (20.6475, 338) -- (20.6503, 338) -- (20.653, 338) -- (20.6557, 339) -- (20.6585, 339) -- (20.6612, 339) -- (20.6639, 339) -- (20.6667, 339) -- (20.6694, 339) -- (20.6721, 340) -- (20.6749, 340) -- (20.6776, 340) -- (20.6803, 340) -- (20.6831, 340) -- (20.6858, 340) -- (20.6885, 340) -- (20.6913, 340) -- (20.694, 340) -- (20.6967, 341) -- (20.6995, 341) -- (20.7022, 341) -- (20.7049, 341) -- (20.7077, 341) -- (20.7104, 341) -- (20.7131, 341) -- (20.7158, 341) -- (20.7186, 341) -- (20.7213, 341) -- (20.724, 342) -- (20.7268, 342) -- (20.7295, 342) -- (20.7322, 342) -- (20.735, 342) -- (20.7377, 342) -- (20.7404, 342) -- (20.7432, 342) -- (20.7459, 342) -- (20.7486, 342) -- (20.7514, 342) -- (20.7541, 342) -- (20.7568, 342) -- (20.7623, 342) -- (20.765, 342) -- (20.7678, 343) -- (20.7705, 343) -- (20.7732, 343) -- (20.776, 343) -- (20.7787, 343) -- (20.7814, 342) -- (20.7842, 342) -- (20.7869, 341) -- (20.7896, 341) -- (20.7923, 341) -- (20.7951, 341) -- (20.7978, 341) -- (20.8005, 341) -- (20.8033, 339) -- (20.806, 339) -- (20.8087, 338) -- (20.8115, 338) -- (20.8142, 338) -- (20.8169, 338) -- (20.8197, 337) -- (20.8224, 338) -- (20.8251, 338) -- (20.8279, 338) -- (20.8306, 338) -- (20.8333, 338) -- (20.8361, 338) -- (20.8388, 338) -- (20.8415, 338) -- (20.8443, 338) -- (20.847, 338) -- (20.8497, 338) -- (20.8525, 337) -- (20.8552, 337) -- (20.8579, 337) -- (20.8607, 336) -- (20.8634, 337) -- (20.8661, 337) -- (20.8689, 337) -- (20.8716, 337) -- (20.8743, 337) -- (20.877, 336) -- (20.8798, 336) -- (20.8825, 336) -- (20.8852, 336) -- (20.888, 336) -- (20.8907, 336) -- (20.8934, 336) -- (20.8962, 336) -- (20.8989, 336) -- (20.9016, 336) -- (20.9044, 336) -- (20.9071, 336) -- (20.9098, 335) -- (20.9126, 335) -- (20.9153, 334) -- (20.918, 334) -- (20.9208, 333) -- (20.9235, 333) -- (20.9262, 333) -- (20.929, 329) -- (20.9317, 329) -- (20.9344, 329) -- (20.9372, 329) -- (20.9399, 329) -- (20.9426, 330) -- (20.9454, 330) -- (20.9481, 330) -- (20.9508, 330) -- (20.9536, 329) -- (20.9563, 329) -- (20.959, 328) -- (20.9617, 328) -- (20.9645, 328) -- (20.9672, 328) -- (20.9699, 327) -- (20.9727, 326) -- (20.9754, 325) -- (20.9781, 324) -- (20.9809, 324) -- (20.9836, 324) -- (20.9863, 324) -- (20.9891, 324) -- (20.9918, 323) -- (20.9945, 322) -- (20.9973, 322) -- (21, 321) -- (21.0027, 321) -- (21.0055, 321) -- (21.0082, 321) -- (21.011, 320) -- (21.0137, 320) -- (21.0164, 320) -- (21.0192, 320) -- (21.0219, 320) -- (21.0247, 319) -- (21.0274, 319) -- (21.0301, 319) -- (21.0329, 318) -- (21.0356, 316) -- (21.0384, 316) -- (21.0411, 315) -- (21.0438, 314) -- (21.0466, 313) -- (21.0493, 313) -- (21.0521, 312) -- (21.0548, 312) -- (21.0575, 312) -- (21.0603, 312) -- (21.063, 312) -- (21.0658, 312) -- (21.0685, 312) -- (21.0712, 312) -- (21.074, 311) -- (21.0767, 311) -- (21.0795, 311) -- (21.0822, 311) -- (21.0849, 310) -- (21.0877, 310) -- (21.0904, 309) -- (21.0932, 308) -- (21.0959, 308) -- (21.0986, 308) -- (21.1014, 308) -- (21.1041, 307) -- (21.1068, 307) -- (21.1096, 307) -- (21.1123, 307) -- (21.1151, 307) -- (21.1178, 305) -- (21.1205, 305) -- (21.1233, 304) -- (21.126, 303) -- (21.1288, 303) -- (21.1315, 302) -- (21.1342, 299) -- (21.1342, 0) -- (19.6466, 0) -- cycle;

==> data/tcf2-transition/quantcast/stacked/transition.tex <==
\draw (18.2932, 1) -- (18.2959, 1) -- (18.2986, 1) -- (18.3014, 1) -- (18.3041, 1) -- (18.3068, 1) -- (18.3096, 1) -- (18.3123, 1) -- (18.3151, 1) -- (18.3178, 1) -- (18.3205, 2) -- (18.3233, 2) -- (18.326, 2) -- (18.3288, 2) -- (18.3315, 2) -- (18.3342, 2) -- (18.337, 2) -- (18.3397, 2) -- (18.3425, 2) -- (18.3452, 2) -- (18.3479, 2) -- (18.3507, 2) -- (18.3534, 2) -- (18.3562, 3) -- (18.3589, 3) -- (18.3616, 3) -- (18.3644, 3) -- (18.3671, 5) -- (18.3699, 5) -- (18.3726, 6) -- (18.3753, 9) -- (18.3781, 11) -- (18.3808, 12) -- (18.3836, 14) -- (18.3863, 16) -- (18.389, 21) -- (18.3918, 37) -- (18.3945, 103) -- (18.3973, 198) -- (18.4, 268) -- (18.4027, 307) -- (18.4055, 341) -- (18.4082, 376) -- (18.411, 405) -- (18.4137, 431) -- (18.4164, 451) -- (18.4192, 479) -- (18.4219, 497) -- (18.4247, 513) -- (18.4274, 532) -- (18.4301, 549) -- (18.4329, 584) -- (18.4356, 615) -- (18.4384, 623) -- (18.4411, 641) -- (18.4438, 655) -- (18.4466, 669) -- (18.4493, 689) -- (18.4521, 706) -- (18.4548, 718) -- (18.4575, 727) -- (18.4603, 742) -- (18.463, 751) -- (18.4658, 766) -- (18.4685, 777) -- (18.4712, 789) -- (18.474, 804) -- (18.4767, 812) -- (18.4795, 821) -- (18.4822, 834) -- (18.4849, 844) -- (18.4877, 858) -- (18.4904, 873) -- (18.4932, 881) -- (18.4959, 893) -- (18.4986, 905) -- (18.5014, 924) -- (18.5041, 938) -- (18.5068, 950) -- (18.5096, 956) -- (18.5123, 967) -- (18.5151, 976) -- (18.5178, 985) -- (18.5205, 991) -- (18.5233, 1002) -- (18.526, 1011) -- (18.5288, 1023) -- (18.5315, 1035) -- (18.5342, 1043) -- (18.537, 1057) -- (18.5397, 1070) -- (18.5425, 1078) -- (18.5452, 1091) -- (18.5479, 1105) -- (18.5507, 1113) -- (18.5534, 1121) -- (18.5562, 1133) -- (18.5589, 1144) -- (18.5616, 1144) -- (18.5644, 1144) -- (18.5671, 1144) -- (18.5699, 1163) -- (18.5726, 1181) -- (18.5753, 1201) -- (18.5781, 1214) -- (18.5808, 1233) -- (18.5836, 1245) -- (18.5863, 1266) -- (18.589, 1281) -- (18.5918, 1288) -- (18.5945, 1300) -- (18.5973, 1311) -- (18.6, 1320) -- (18.6027, 1338) -- (18.6055, 1350) -- (18.6082, 1359) -- (18.611, 1374) -- (18.6137, 1384) -- (18.6164, 1398) -- (18.6192, 1404) -- (18.6219, 1409) -- (18.6247, 1420) -- (18.6274, 1432) -- (18.6301, 1446) -- (18.6329, 1457) -- (18.6356, 1471) -- (18.6384, 1484) -- (18.6411, 1499) -- (18.6438, 1505) -- (18.6466, 1514) -- (18.6493, 1524) -- (18.6521, 1538) -- (18.6548, 1549) -- (18.6575, 1558) -- (18.6603, 1572) -- (18.663, 1585) -- (18.6658, 1593) -- (18.6685, 1612) -- (18.6712, 1615) -- (18.674, 1621) -- (18.6767, 1634) -- (18.6795, 1649) -- (18.6822, 1663) -- (18.6849, 1677) -- (18.6877, 1689) -- (18.6904, 1701) -- (18.6932, 1719) -- (18.6959, 1732) -- (18.6986, 1752) -- (18.7014, 1760) -- (18.7041, 1770) -- (18.7068, 1784) -- (18.7096, 1792) -- (18.7123, 1806) -- (18.7151, 1825) -- (18.7178, 1842) -- (18.7205, 1858) -- (18.7233, 1876) -- (18.726, 1887) -- (18.7288, 1901) -- (18.7315, 1915) -- (18.7342, 1924) -- (18.737, 1936) -- (18.7397, 1946) -- (18.7425, 1953) -- (18.7452, 1962) -- (18.7479, 1978) -- (18.7507, 1988) -- (18.7534, 1994) -- (18.7562, 2008) -- (18.7589, 2013) -- (18.7616, 2025) -- (18.7644, 2037) -- (18.7671, 2051) -- (18.7699, 2061) -- (18.7726, 2071) -- (18.7753, 2074) -- (18.7781, 2082) -- (18.7808, 2095) -- (18.7836, 2098) -- (18.7863, 2108) -- (18.789, 2120) -- (18.7918, 2126) -- (18.7945, 2133) -- (18.7973, 2140) -- (18.8, 2149) -- (18.8027, 2160) -- (18.8055, 2167) -- (18.8082, 2176) -- (18.811, 2190) -- (18.8137, 2206) -- (18.8164, 2217) -- (18.8192, 2231) -- (18.8219, 2242) -- (18.8247, 2254) -- (18.8274, 2263) -- (18.8301, 2278) -- (18.8329, 2292) -- (18.8356, 2337) -- (18.8384, 2394) -- (18.8411, 2430) -- (18.8438, 2466) -- (18.8466, 2502) -- (18.8493, 2552) -- (18.8521, 2593) -- (18.8548, 2635) -- (18.8575, 2661) -- (18.8603, 2688) -- (18.863, 2718) -- (18.8658, 2754) -- (18.8685, 2785) -- (18.8712, 2812) -- (18.874, 2843) -- (18.8767, 2876) -- (18.8795, 2903) -- (18.8822, 2931) -- (18.8849, 2956) -- (18.8877, 2977) -- (18.8904, 2996) -- (18.8932, 3022) -- (18.8959, 3039) -- (18.8986, 3051) -- (18.9014, 3060) -- (18.9041, 3066) -- (18.9068, 3094) -- (18.9096, 3115) -- (18.9123, 3147) -- (18.9151, 3171) -- (18.9178, 3188) -- (18.9205, 3204) -- (18.9233, 3226) -- (18.926, 3251) -- (18.9288, 3274) -- (18.9315, 3287) -- (18.9342, 3305) -- (18.937, 3320) -- (18.9397, 3336) -- (18.9425, 3359) -- (18.9452, 3383) -- (18.9479, 3392) -- (18.9507, 3411) -- (18.9534, 3425) -- (18.9562, 3441) -- (18.9589, 3464) -- (18.9616, 3487) -- (18.9644, 3507) -- (18.9671, 3518) -- (18.9699, 3536) -- (18.9726, 3552) -- (18.9753, 3564) -- (18.9781, 3578) -- (18.9808, 3586) -- (18.9836, 3597) -- (18.9863, 3611) -- (18.989, 3632) -- (18.9918, 3637) -- (18.9945, 3643) -- (18.9973, 3654) -- (19, 3659) -- (19.0027, 3677) -- (19.0055, 3692) -- (19.0082, 3699) -- (19.011, 3707) -- (19.0137, 3715) -- (19.0164, 3728) -- (19.0192, 3746) -- (19.0219, 3758) -- (19.0247, 3776) -- (19.0274, 3796) -- (19.0301, 3806) -- (19.0329, 3813) -- (19.0356, 3833) -- (19.0384, 3860) -- (19.0411, 3876) -- (19.0438, 3884) -- (19.0466, 3898) -- (19.0493, 3911) -- (19.0521, 3925) -- (19.0548, 3940) -- (19.0575, 3961) -- (19.0603, 3984) -- (19.063, 4006) -- (19.0658, 4035) -- (19.0685, 4048) -- (19.0712, 4064) -- (19.074, 4076) -- (19.0767, 4087) -- (19.0795, 4102) -- (19.0822, 4120) -- (19.0849, 4145) -- (19.0877, 4167) -- (19.0904, 4186) -- (19.0932, 4200) -- (19.0959, 4216) -- (19.0986, 4232) -- (19.1014, 4259) -- (19.1041, 4274) -- (19.1068, 4298) -- (19.1096, 4311) -- (19.1123, 4339) -- (19.1151, 4366) -- (19.1178, 4390) -- (19.1205, 4426) -- (19.1233, 4452) -- (19.126, 4478) -- (19.1288, 4503) -- (19.1315, 4523) -- (19.1342, 4543) -- (19.137, 4578) -- (19.1397, 4608) -- (19.1425, 4642) -- (19.1452, 4664) -- (19.1479, 4690) -- (19.1507, 4708) -- (19.1534, 4731) -- (19.1562, 4753) -- (19.1589, 4780) -- (19.1616, 4810) -- (19.1644, 4834) -- (19.1671, 4856) -- (19.1699, 4881) -- (19.1726, 4905) -- (19.1753, 4919) -- (19.1781, 4930) -- (19.1808, 4963) -- (19.1836, 4977) -- (19.1863, 4989) -- (19.189, 5003) -- (19.1918, 5022) -- (19.1945, 5042) -- (19.1973, 5061) -- (19.2, 5087) -- (19.2027, 5104) -- (19.2055, 5122) -- (19.2082, 5150) -- (19.211, 5169) -- (19.2137, 5194) -- (19.2164, 5212) -- (19.2192, 5234) -- (19.2219, 5246) -- (19.2247, 5266) -- (19.2274, 5290) -- (19.2301, 5308) -- (19.2329, 5334) -- (19.2356, 5375) -- (19.2384, 5404) -- (19.2411, 5420) -- (19.2438, 5436) -- (19.2466, 5454) -- (19.2493, 5468) -- (19.2521, 5483) -- (19.2548, 5508) -- (19.2575, 5529) -- (19.2603, 5545) -- (19.263, 5556) -- (19.2658, 5575) -- (19.2685, 5588) -- (19.2712, 5615) -- (19.274, 5626) -- (19.2767, 5653) -- (19.2795, 5664) -- (19.2822, 5685) -- (19.2849, 5706) -- (19.2877, 5724) -- (19.2904, 5743) -- (19.2932, 5755) -- (19.2959, 5771) -- (19.2986, 5782) -- (19.3014, 5786) -- (19.3041, 5801) -- (19.3068, 5817) -- (19.3096, 5831) -- (19.3123, 5842) -- (19.3151, 5873) -- (19.3178, 5885) -- (19.3205, 5905) -- (19.3233, 5913) -- (19.326, 5922) -- (19.3288, 5931) -- (19.3315, 5937) -- (19.3342, 5941) -- (19.337, 5945) -- (19.3397, 5946) -- (19.3425, 5959) -- (19.3452, 5966) -- (19.3479, 5971) -- (19.3507, 5979) -- (19.3534, 5994) -- (19.3562, 6002) -- (19.3589, 6005) -- (19.3616, 6016) -- (19.3644, 6025) -- (19.3671, 6041) -- (19.3699, 6049) -- (19.3726, 6057) -- (19.3753, 6067) -- (19.3781, 6075) -- (19.3808, 6081) -- (19.3836, 6085) -- (19.3863, 6087) -- (19.389, 6085) -- (19.3918, 6092) -- (19.3945, 6107) -- (19.3973, 6114) -- (19.4, 6123) -- (19.4027, 6134) -- (19.4055, 6138) -- (19.4082, 6148) -- (19.411, 6163) -- (19.4137, 6173) -- (19.4164, 6179) -- (19.4192, 6182) -- (19.4219, 6184) -- (19.4247, 6198) -- (19.4274, 6217) -- (19.4301, 6226) -- (19.4329, 6231) -- (19.4356, 6236) -- (19.4384, 6238) -- (19.4411, 6247) -- (19.4438, 6254) -- (19.4466, 6253) -- (19.4493, 6259) -- (19.4521, 6264) -- (19.4548, 6274) -- (19.4575, 6278) -- (19.4603, 6277) -- (19.463, 6286) -- (19.4658, 6291) -- (19.4685, 6308) -- (19.4712, 6315) -- (19.474, 6324) -- (19.4767, 6331) -- (19.4795, 6333) -- (19.4822, 6346) -- (19.4849, 6356) -- (19.4877, 6370) -- (19.4904, 6379) -- (19.4932, 6380) -- (19.4959, 6392) -- (19.4986, 6398) -- (19.5014, 6403) -- (19.5041, 6408) -- (19.5068, 6415) -- (19.5096, 6426) -- (19.5123, 6426) -- (19.5151, 6438) -- (19.5178, 6435) -- (19.5205, 6443) -- (19.5233, 6456) -- (19.526, 6466) -- (19.5288, 6471) -- (19.5315, 6465) -- (19.5342, 6468) -- (19.537, 6473) -- (19.5397, 6482) -- (19.5425, 6484) -- (19.5452, 6495) -- (19.5479, 6495) -- (19.5507, 6496) -- (19.5534, 6504) -- (19.5562, 6501) -- (19.5589, 6506) -- (19.5616, 6515) -- (19.5644, 6522) -- (19.5671, 6530) -- (19.5699, 6530) -- (19.5726, 6548) -- (19.5753, 6562) -- (19.5781, 6561) -- (19.5808, 6574) -- (19.5836, 6577) -- (19.5863, 6584) -- (19.589, 6581) -- (19.5918, 6596) -- (19.5945, 6598) -- (19.5973, 6598) -- (19.6, 6607) -- (19.6027, 6612) -- (19.6055, 6621) -- (19.6082, 6625) -- (19.611, 6622) -- (19.6137, 6621) -- (19.6164, 6625) -- (19.6192, 6635) -- (19.6219, 6636) -- (19.6247, 6647) -- (19.6274, 6648) -- (19.6301, 6644) -- (19.6329, 6647) -- (19.6356, 6653) -- (19.6384, 6663) -- (19.6411, 6677) -- (19.6438, 6684) -- (19.6466, 6678) -- (19.6493, 6686) -- (19.6521, 6684) -- (19.6548, 6679) -- (19.6575, 6679) -- (19.6603, 6680) -- (19.663, 6677) -- (19.6658, 6676) -- (19.6685, 6680) -- (19.6712, 6688) -- (19.674, 6696) -- (19.6767, 6698) -- (19.6795, 6708) -- (19.6822, 6709) -- (19.6849, 6715) -- (19.6877, 6720) -- (19.6904, 6721) -- (19.6932, 6725) -- (19.6959, 6737) -- (19.6986, 6744) -- (19.7014, 6752) -- (19.7041, 6745) -- (19.7068, 6743) -- (19.7096, 6741) -- (19.7123, 6747) -- (19.7151, 6748) -- (19.7178, 6754) -- (19.7205, 6750) -- (19.7233, 6745) -- (19.726, 6744) -- (19.7288, 6746) -- (19.7315, 6756) -- (19.7342, 6755) -- (19.737, 6751) -- (19.7397, 6755) -- (19.7425, 6758) -- (19.7452, 6761) -- (19.7479, 6774) -- (19.7507, 6769) -- (19.7534, 6777) -- (19.7562, 6782) -- (19.7589, 6790) -- (19.7616, 6776) -- (19.7644, 6771) -- (19.7671, 6772) -- (19.7699, 6772) -- (19.7726, 6763) -- (19.7753, 6769) -- (19.7781, 6772) -- (19.7808, 6769) -- (19.7836, 6793) -- (19.7863, 6806) -- (19.789, 6805) -- (19.7918, 6829) -- (19.7945, 6848) -- (19.7973, 6862) -- (19.8, 6870) -- (19.8027, 6868) -- (19.8055, 6880) -- (19.8082, 6883) -- (19.811, 6876) -- (19.8137, 6883) -- (19.8164, 6893) -- (19.8192, 6895) -- (19.8219, 6899) -- (19.8247, 6909) -- (19.8274, 6919) -- (19.8301, 6930) -- (19.8329, 6940) -- (19.8356, 6943) -- (19.8384, 6950) -- (19.8411, 6953) -- (19.8438, 6966) -- (19.8466, 6965) -- (19.8493, 6959) -- (19.8521, 6965) -- (19.8548, 6965) -- (19.8575, 6966) -- (19.8603, 6962) -- (19.863, 6965) -- (19.8658, 6973) -- (19.8685, 6980) -- (19.8712, 6980) -- (19.874, 6977) -- (19.8767, 6976) -- (19.8795, 6984) -- (19.8822, 6994) -- (19.8849, 7046) -- (19.8877, 7053) -- (19.8904, 7050) -- (19.8932, 7052) -- (19.8959, 7052) -- (19.8986, 7047) -- (19.9014, 7039) -- (19.9041, 7043) -- (19.9068, 7046) -- (19.9096, 7053) -- (19.9123, 7058) -- (19.9151, 7054) -- (19.9178, 7063) -- (19.9205, 7081) -- (19.9233, 7097) -- (19.926, 7089) -- (19.9288, 7090) -- (19.9315, 7096) -- (19.9342, 7099) -- (19.937, 7100) -- (19.9397, 7105) -- (19.9425, 7112) -- (19.9452, 7110) -- (19.9479, 7120) -- (19.9507, 7114) -- (19.9534, 7116) -- (19.9562, 7119) -- (19.9589, 7123) -- (19.9616, 7128) -- (19.9644, 7137) -- (19.9671, 7138) -- (19.9699, 7146) -- (19.9726, 7152) -- (19.9753, 7156) -- (19.9781, 7156) -- (19.9808, 7158) -- (19.9836, 7161) -- (19.9863, 7169) -- (19.989, 7167) -- (19.9918, 7162) -- (19.9945, 7160) -- (19.9973, 7157) -- (20, 7160) -- (20.0027, 7168) -- (20.0055, 7168) -- (20.0082, 7178) -- (20.0109, 7169) -- (20.0137, 7177) -- (20.0164, 7170) -- (20.0191, 7181) -- (20.0219, 7189) -- (20.0246, 7198) -- (20.0273, 7209) -- (20.0301, 7204) -- (20.0328, 7206) -- (20.0355, 7205) -- (20.0383, 7211) -- (20.041, 7216) -- (20.0437, 7231) -- (20.0464, 7231) -- (20.0492, 7229) -- (20.0519, 7233) -- (20.0546, 7231) -- (20.0574, 7238) -- (20.0601, 7238) -- (20.0628, 7246) -- (20.0656, 7256) -- (20.0683, 7256) -- (20.071, 7256) -- (20.0738, 7270) -- (20.0765, 7272) -- (20.0792, 7275) -- (20.082, 7276) -- (20.0847, 7278) -- (20.0874, 7276) -- (20.0902, 7283) -- (20.0929, 7282) -- (20.0956, 7289) -- (20.0984, 7293) -- (20.1011, 7291) -- (20.1038, 7296) -- (20.1066, 7302) -- (20.1093, 7300) -- (20.112, 7303) -- (20.1148, 7306) -- (20.1175, 7319) -- (20.1202, 7320) -- (20.123, 7321) -- (20.1257, 7322) -- (20.1284, 7322) -- (20.1311, 7320) -- (20.1339, 7330) -- (20.1366, 7322) -- (20.1393, 7335) -- (20.1421, 7337) -- (20.1448, 7336) -- (20.1475, 7331) -- (20.1503, 7338) -- (20.153, 7346) -- (20.1557, 7353) -- (20.1585, 7363) -- (20.1612, 7374) -- (20.1639, 7372) -- (20.1667, 7377) -- (20.1694, 7378) -- (20.1721, 7382) -- (20.1749, 7387) -- (20.1776, 7392) -- (20.1803, 7397) -- (20.1831, 7403) -- (20.1858, 7404) -- (20.1885, 7405) -- (20.1913, 7405) -- (20.194, 7410) -- (20.1967, 7417) -- (20.1995, 7424) -- (20.2022, 7426) -- (20.2049, 7434) -- (20.2077, 7439) -- (20.2104, 7445) -- (20.2131, 7457) -- (20.2158, 7462) -- (20.2186, 7475) -- (20.2213, 7484) -- (20.224, 7479) -- (20.2268, 7477) -- (20.2295, 7489) -- (20.2322, 7501) -- (20.235, 7516) -- (20.2377, 7523) -- (20.2404, 7526) -- (20.2432, 7522) -- (20.2459, 7532) -- (20.2486, 7538) -- (20.2514, 7543) -- (20.2541, 7560) -- (20.2568, 7568) -- (20.2596, 7575) -- (20.2623, 7580) -- (20.265, 7587) -- (20.2678, 7591) -- (20.2705, 7594) -- (20.2732, 7605) -- (20.276, 7620) -- (20.2787, 7617) -- (20.2814, 7621) -- (20.2842, 7629) -- (20.2869, 7630) -- (20.2896, 7628) -- (20.2923, 7635) -- (20.2951, 7638) -- (20.2978, 7648) -- (20.3005, 7648) -- (20.3033, 7649) -- (20.306, 7654) -- (20.3087, 7653) -- (20.3115, 7653) -- (20.3142, 7653) -- (20.3169, 7662) -- (20.3197, 7653) -- (20.3224, 7655) -- (20.3251, 7659) -- (20.3279, 7668) -- (20.3306, 7657) -- (20.3333, 7662) -- (20.3361, 7656) -- (20.3388, 7657) -- (20.3415, 7651) -- (20.3443, 7650) -- (20.347, 7653) -- (20.3497, 7661) -- (20.3525, 7662) -- (20.3552, 7659) -- (20.3579, 7654) -- (20.3607, 7648) -- (20.3634, 7649) -- (20.3661, 7644) -- (20.3689, 7644) -- (20.3716, 7652) -- (20.3743, 7645) -- (20.377, 7673) -- (20.3798, 7662) -- (20.3825, 7637) -- (20.3852, 7638) -- (20.388, 7646) -- (20.3907, 7633) -- (20.3934, 7627) -- (20.3962, 7622) -- (20.3989, 7594) -- (20.4016, 7591) -- (20.4044, 7582) -- (20.4071, 7584) -- (20.4098, 7575) -- (20.4126, 7515) -- (20.4153, 7444) -- (20.418, 7380) -- (20.4208, 7366) -- (20.4235, 7359) -- (20.4262, 7406) -- (20.429, 7436) -- (20.4317, 7448) -- (20.4344, 7453) -- (20.4372, 7449) -- (20.4399, 7447) -- (20.4426, 7446) -- (20.4454, 7457) -- (20.4481, 7452) -- (20.4508, 7442) -- (20.4536, 7454) -- (20.4563, 7446) -- (20.459, 7442) -- (20.4617, 7443) -- (20.4645, 7434) -- (20.4672, 7426) -- (20.4699, 7408) -- (20.4727, 7411) -- (20.4754, 7408) -- (20.4781, 7401) -- (20.4809, 7399) -- (20.4836, 7402) -- (20.4863, 7401) -- (20.4891, 7392) -- (20.4918, 7400) -- (20.4945, 7375) -- (20.4973, 7371) -- (20.5, 7350) -- (20.5027, 7345) -- (20.5055, 7332) -- (20.5082, 7324) -- (20.5109, 7318) -- (20.5137, 7295) -- (20.5164, 7293) -- (20.5191, 7267) -- (20.5219, 7269) -- (20.5246, 7259) -- (20.5273, 7254) -- (20.5301, 7241) -- (20.5328, 7222) -- (20.5355, 7210) -- (20.5383, 7192) -- (20.541, 7193) -- (20.5437, 7186) -- (20.5464, 7162) -- (20.5492, 7183) -- (20.5519, 7169) -- (20.5546, 7160) -- (20.5574, 7137) -- (20.5601, 7125) -- (20.5628, 7105) -- (20.5656, 7096) -- (20.5683, 7083) -- (20.571, 7055) -- (20.5738, 7029) -- (20.5765, 6989) -- (20.5792, 6958) -- (20.582, 6917) -- (20.5847, 6881) -- (20.5874, 6843) -- (20.5902, 6831) -- (20.5929, 6797) -- (20.5956, 6771) -- (20.5984, 6726) -- (20.6011, 6703) -- (20.6038, 6674) -- (20.6066, 6646) -- (20.6093, 6608) -- (20.612, 6550) -- (20.6148, 6484) -- (20.6175, 6385) -- (20.6202, 6324) -- (20.623, 6248) -- (20.6257, 6189) -- (20.6284, 6129) -- (20.6311, 6064) -- (20.6339, 6004) -- (20.6366, 5958) -- (20.6393, 5907) -- (20.6421, 5867) -- (20.6448, 5826) -- (20.6475, 5789) -- (20.6503, 5746) -- (20.653, 5713) -- (20.6557, 5665) -- (20.6585, 5646) -- (20.6612, 5616) -- (20.6639, 5589) -- (20.6667, 5551) -- (20.6694, 5517) -- (20.6721, 5448) -- (20.6749, 5439) -- (20.6776, 5413) -- (20.6803, 5379) -- (20.6831, 5340) -- (20.6858, 5320) -- (20.6885, 5290) -- (20.6913, 5262) -- (20.694, 5237) -- (20.6967, 5228) -- (20.6995, 5212) -- (20.7022, 5179) -- (20.7049, 5141) -- (20.7077, 5139) -- (20.7104, 5103) -- (20.7131, 5084) -- (20.7158, 5059) -- (20.7186, 5034) -- (20.7213, 5002) -- (20.724, 4977) -- (20.7268, 4944) -- (20.7295, 4917) -- (20.7322, 4887) -- (20.735, 4872) -- (20.7377, 4851) -- (20.7404, 4811) -- (20.7432, 4779) -- (20.7459, 4756) -- (20.7486, 4750) -- (20.7514, 4716) -- (20.7541, 4707) -- (20.7568, 4694) -- (20.7596, 4691) -- (20.7623, 4652) -- (20.765, 4609) -- (20.7678, 4570) -- (20.7705, 4546) -- (20.7732, 4530) -- (20.776, 4501) -- (20.7787, 4459) -- (20.7814, 4448) -- (20.7842, 4414) -- (20.7869, 4390) -- (20.7896, 4369) -- (20.7923, 4351) -- (20.7951, 4320) -- (20.7978, 4269) -- (20.8005, 4239) -- (20.8033, 4202) -- (20.806, 4169) -- (20.8087, 4139) -- (20.8115, 4114) -- (20.8142, 4087) -- (20.8169, 4056) -- (20.8197, 4033) -- (20.8224, 3992) -- (20.8251, 3973) -- (20.8279, 3938) -- (20.8306, 3918) -- (20.8333, 3906) -- (20.8361, 3883) -- (20.8388, 3871) -- (20.8415, 3845) -- (20.8443, 3809) -- (20.847, 3793) -- (20.8497, 3761) -- (20.8525, 3747) -- (20.8552, 3714) -- (20.8579, 3689) -- (20.8607, 3657) -- (20.8634, 3641) -- (20.8661, 3616) -- (20.8689, 3606) -- (20.8716, 3443) -- (20.8743, 3401) -- (20.877, 3366) -- (20.8798, 3358) -- (20.8825, 3331) -- (20.8852, 3305) -- (20.888, 3301) -- (20.8907, 3289) -- (20.8934, 3254) -- (20.8962, 3222) -- (20.8989, 3196) -- (20.9016, 3175) -- (20.9044, 3158) -- (20.9071, 3133) -- (20.9098, 3108) -- (20.9126, 3065) -- (20.9153, 3042) -- (20.918, 3019) -- (20.9208, 2994) -- (20.9235, 2975) -- (20.9262, 2911) -- (20.929, 2879) -- (20.9317, 2853) -- (20.9344, 2826) -- (20.9372, 2804) -- (20.9399, 2792) -- (20.9426, 2785) -- (20.9454, 2773) -- (20.9481, 2756) -- (20.9508, 2734) -- (20.9536, 2716) -- (20.9563, 2703) -- (20.959, 2685) -- (20.9617, 2665) -- (20.9645, 2663) -- (20.9672, 2647) -- (20.9699, 2620) -- (20.9727, 2598) -- (20.9754, 2585) -- (20.9781, 2566) -- (20.9809, 2552) -- (20.9836, 2547) -- (20.9863, 2525) -- (20.9891, 2505) -- (20.9918, 2477) -- (20.9945, 2470) -- (20.9973, 2468) -- (21, 2452) -- (21.0027, 2446) -- (21.0055, 2426) -- (21.0082, 2404) -- (21.011, 2377) -- (21.0137, 2364) -- (21.0164, 2342) -- (21.0192, 2339) -- (21.0219, 2339) -- (21.0247, 2325) -- (21.0274, 2301) -- (21.0301, 2288) -- (21.0329, 2276) -- (21.0356, 2253) -- (21.0384, 2238) -- (21.0411, 2216) -- (21.0438, 2199) -- (21.0466, 2169) -- (21.0493, 2148) -- (21.0521, 2133) -- (21.0548, 2110) -- (21.0575, 2090) -- (21.0603, 2077) -- (21.063, 2055) -- (21.0658, 2029) -- (21.0685, 2003) -- (21.0712, 1979) -- (21.074, 1946) -- (21.0767, 1929) -- (21.0795, 1916) -- (21.0822, 1892) -- (21.0849, 1860) -- (21.0877, 1836) -- (21.0904, 1813) -- (21.0932, 1783) -- (21.0959, 1776) -- (21.0986, 1759) -- (21.1014, 1751) -- (21.1041, 1716) -- (21.1068, 1676) -- (21.1096, 1661) -- (21.1123, 1644) -- (21.1151, 1634) -- (21.1178, 1626) -- (21.1205, 1613) -- (21.1233, 1586) -- (21.126, 1575) -- (21.1288, 1551) -- (21.1315, 1541) -- (21.1342, 1519) -- (21.1342, 0) -- (18.2932, 0) -- cycle;

==> data/tcf2-transition/quantcast/stacked/v1.tex <==
\draw (18.2932, 1) -- (18.2959, 1) -- (18.2986, 1) -- (18.3014, 1) -- (18.3041, 1) -- (18.3068, 1) -- (18.3096, 1) -- (18.3123, 1) -- (18.3151, 1) -- (18.3178, 1) -- (18.3205, 2) -- (18.3233, 2) -- (18.326, 2) -- (18.3288, 2) -- (18.3315, 2) -- (18.3342, 2) -- (18.337, 2) -- (18.3397, 2) -- (18.3425, 2) -- (18.3452, 2) -- (18.3479, 2) -- (18.3507, 2) -- (18.3534, 2) -- (18.3562, 3) -- (18.3589, 3) -- (18.3616, 3) -- (18.3644, 3) -- (18.3671, 5) -- (18.3699, 5) -- (18.3726, 6) -- (18.3753, 9) -- (18.3781, 11) -- (18.3808, 12) -- (18.3836, 14) -- (18.3863, 16) -- (18.389, 21) -- (18.3918, 37) -- (18.3945, 103) -- (18.3973, 197) -- (18.4, 267) -- (18.4027, 305) -- (18.4055, 338) -- (18.4082, 372) -- (18.411, 400) -- (18.4137, 426) -- (18.4164, 446) -- (18.4192, 474) -- (18.4219, 491) -- (18.4247, 506) -- (18.4274, 525) -- (18.4301, 542) -- (18.4329, 577) -- (18.4356, 608) -- (18.4384, 615) -- (18.4411, 633) -- (18.4438, 647) -- (18.4466, 661) -- (18.4493, 681) -- (18.4521, 696) -- (18.4548, 706) -- (18.4575, 714) -- (18.4603, 728) -- (18.463, 737) -- (18.4658, 751) -- (18.4685, 760) -- (18.4712, 772) -- (18.474, 787) -- (18.4767, 795) -- (18.4795, 803) -- (18.4822, 811) -- (18.4849, 821) -- (18.4877, 834) -- (18.4904, 848) -- (18.4932, 855) -- (18.4959, 866) -- (18.4986, 877) -- (18.5014, 892) -- (18.5041, 903) -- (18.5068, 915) -- (18.5096, 918) -- (18.5123, 927) -- (18.5151, 935) -- (18.5178, 936) -- (18.5205, 935) -- (18.5233, 943) -- (18.526, 956) -- (18.5288, 972) -- (18.5315, 989) -- (18.5342, 1000) -- (18.537, 1017) -- (18.5397, 1032) -- (18.5425, 1040) -- (18.5452, 1055) -- (18.5479, 1073) -- (18.5507, 1085) -- (18.5534, 1091) -- (18.5562, 1102) -- (18.5589, 1113) -- (18.5616, 1113) -- (18.5644, 1113) -- (18.5671, 1113) -- (18.5699, 1134) -- (18.5726, 1152) -- (18.5753, 1172) -- (18.5781, 1184) -- (18.5808, 1203) -- (18.5836, 1216) -- (18.5863, 1238) -- (18.589, 1252) -- (18.5918, 1259) -- (18.5945, 1273) -- (18.5973, 1283) -- (18.6, 1294) -- (18.6027, 1311) -- (18.6055, 1324) -- (18.6082, 1333) -- (18.611, 1348) -- (18.6137, 1358) -- (18.6164, 1373) -- (18.6192, 1378) -- (18.6219, 1382) -- (18.6247, 1393) -- (18.6274, 1405) -- (18.6301, 1419) -- (18.6329, 1427) -- (18.6356, 1441) -- (18.6384, 1454) -- (18.6411, 1469) -- (18.6438, 1476) -- (18.6466, 1484) -- (18.6493, 1497) -- (18.6521, 1511) -- (18.6548, 1522) -- (18.6575, 1532) -- (18.6603, 1547) -- (18.663, 1559) -- (18.6658, 1568) -- (18.6685, 1587) -- (18.6712, 1591) -- (18.674, 1597) -- (18.6767, 1610) -- (18.6795, 1626) -- (18.6822, 1640) -- (18.6849, 1654) -- (18.6877, 1666) -- (18.6904, 1678) -- (18.6932, 1696) -- (18.6959, 1710) -- (18.6986, 1730) -- (18.7014, 1738) -- (18.7041, 1748) -- (18.7068, 1762) -- (18.7096, 1770) -- (18.7123, 1784) -- (18.7151, 1803) -- (18.7178, 1820) -- (18.7205, 1836) -- (18.7233, 1854) -- (18.726, 1865) -- (18.7288, 1879) -- (18.7315, 1892) -- (18.7342, 1900) -- (18.737, 1912) -- (18.7397, 1921) -- (18.7425, 1928) -- (18.7452, 1937) -- (18.7479, 1952) -- (18.7507, 1962) -- (18.7534, 1967) -- (18.7562, 1981) -- (18.7589, 1985) -- (18.7616, 1997) -- (18.7644, 2009) -- (18.7671, 2022) -- (18.7699, 2032) -- (18.7726, 2042) -- (18.7753, 2045) -- (18.7781, 2053) -- (18.7808, 2066) -- (18.7836, 2069) -- (18.7863, 2079) -- (18.789, 2091) -- (18.7918, 2096) -- (18.7945, 2103) -- (18.7973, 2110) -- (18.8, 2119) -- (18.8027, 2130) -- (18.8055, 2137) -- (18.8082, 2146) -- (18.811, 2160) -- (18.8137, 2176) -- (18.8164, 2187) -- (18.8192, 2200) -- (18.8219, 2211) -- (18.8247, 2223) -- (18.8274, 2232) -- (18.8301, 2247) -- (18.8329, 2261) -- (18.8356, 2306) -- (18.8384, 2363) -- (18.8411, 2399) -- (18.8438, 2435) -- (18.8466, 2472) -- (18.8493, 2522) -- (18.8521, 2563) -- (18.8548, 2605) -- (18.8575, 2631) -- (18.8603, 2658) -- (18.863, 2686) -- (18.8658, 2721) -- (18.8685, 2751) -- (18.8712, 2777) -- (18.874, 2808) -- (18.8767, 2840) -- (18.8795, 2867) -- (18.8822, 2893) -- (18.8849, 2915) -- (18.8877, 2936) -- (18.8904, 2955) -- (18.8932, 2980) -- (18.8959, 2995) -- (18.8986, 3005) -- (18.9014, 3009) -- (18.9041, 3015) -- (18.9068, 3044) -- (18.9096, 3064) -- (18.9123, 3096) -- (18.9151, 3120) -- (18.9178, 3140) -- (18.9205, 3157) -- (18.9233, 3178) -- (18.926, 3203) -- (18.9288, 3225) -- (18.9315, 3237) -- (18.9342, 3255) -- (18.937, 3269) -- (18.9397, 3285) -- (18.9425, 3307) -- (18.9452, 3330) -- (18.9479, 3339) -- (18.9507, 3357) -- (18.9534, 3369) -- (18.9562, 3383) -- (18.9589, 3401) -- (18.9616, 3426) -- (18.9644, 3446) -- (18.9671, 3457) -- (18.9699, 3478) -- (18.9726, 3495) -- (18.9753, 3508) -- (18.9781, 3521) -- (18.9808, 3529) -- (18.9836, 3540) -- (18.9863, 3553) -- (18.989, 3575) -- (18.9918, 3579) -- (18.9945, 3585) -- (18.9973, 3596) -- (19, 3601) -- (19.0027, 3619) -- (19.0055, 3634) -- (19.0082, 3640) -- (19.011, 3648) -- (19.0137, 3656) -- (19.0164, 3669) -- (19.0192, 3686) -- (19.0219, 3699) -- (19.0247, 3714) -- (19.0274, 3733) -- (19.0301, 3745) -- (19.0329, 3752) -- (19.0356, 3772) -- (19.0384, 3797) -- (19.0411, 3814) -- (19.0438, 3822) -- (19.0466, 3835) -- (19.0493, 3846) -- (19.0521, 3859) -- (19.0548, 3872) -- (19.0575, 3890) -- (19.0603, 3910) -- (19.063, 3932) -- (19.0658, 3964) -- (19.0685, 3978) -- (19.0712, 3995) -- (19.074, 4006) -- (19.0767, 4015) -- (19.0795, 4030) -- (19.0822, 4048) -- (19.0849, 4073) -- (19.0877, 4093) -- (19.0904, 4112) -- (19.0932, 4125) -- (19.0959, 4141) -- (19.0986, 4156) -- (19.1014, 4182) -- (19.1041, 4197) -- (19.1068, 4221) -- (19.1096, 4234) -- (19.1123, 4260) -- (19.1151, 4285) -- (19.1178, 4310) -- (19.1205, 4346) -- (19.1233, 4373) -- (19.126, 4399) -- (19.1288, 4424) -- (19.1315, 4443) -- (19.1342, 4463) -- (19.137, 4497) -- (19.1397, 4526) -- (19.1425, 4559) -- (19.1452, 4581) -- (19.1479, 4606) -- (19.1507, 4623) -- (19.1534, 4645) -- (19.1562, 4667) -- (19.1589, 4694) -- (19.1616, 4724) -- (19.1644, 4746) -- (19.1671, 4768) -- (19.1699, 4792) -- (19.1726, 4813) -- (19.1753, 4826) -- (19.1781, 4838) -- (19.1808, 4870) -- (19.1836, 4884) -- (19.1863, 4894) -- (19.189, 4902) -- (19.1918, 4921) -- (19.1945, 4940) -- (19.1973, 4956) -- (19.2, 4980) -- (19.2027, 4995) -- (19.2055, 5015) -- (19.2082, 5040) -- (19.211, 5055) -- (19.2137, 5078) -- (19.2164, 5091) -- (19.2192, 5109) -- (19.2219, 5111) -- (19.2247, 5120) -- (19.2274, 5124) -- (19.2301, 5137) -- (19.2329, 5165) -- (19.2356, 5212) -- (19.2384, 5269) -- (19.2411, 5282) -- (19.2438, 5303) -- (19.2466, 5323) -- (19.2493, 5336) -- (19.2521, 5351) -- (19.2548, 5377) -- (19.2575, 5397) -- (19.2603, 5406) -- (19.263, 5415) -- (19.2658, 5428) -- (19.2685, 5441) -- (19.2712, 5468) -- (19.274, 5481) -- (19.2767, 5516) -- (19.2795, 5524) -- (19.2822, 5546) -- (19.2849, 5567) -- (19.2877, 5586) -- (19.2904, 5604) -- (19.2932, 5618) -- (19.2959, 5634) -- (19.2986, 5646) -- (19.3014, 5653) -- (19.3041, 5666) -- (19.3068, 5683) -- (19.3096, 5696) -- (19.3123, 5706) -- (19.3151, 5737) -- (19.3178, 5747) -- (19.3205, 5766) -- (19.3233, 5774) -- (19.326, 5784) -- (19.3288, 5791) -- (19.3315, 5797) -- (19.3342, 5801) -- (19.337, 5803) -- (19.3397, 5803) -- (19.3425, 5814) -- (19.3452, 5819) -- (19.3479, 5825) -- (19.3507, 5832) -- (19.3534, 5848) -- (19.3562, 5856) -- (19.3589, 5861) -- (19.3616, 5872) -- (19.3644, 5881) -- (19.3671, 5895) -- (19.3699, 5904) -- (19.3726, 5908) -- (19.3753, 5915) -- (19.3781, 5922) -- (19.3808, 5926) -- (19.3836, 5929) -- (19.3863, 5931) -- (19.389, 5929) -- (19.3918, 5937) -- (19.3945, 5946) -- (19.3973, 5951) -- (19.4, 5955) -- (19.4027, 5964) -- (19.4055, 5967) -- (19.4082, 5977) -- (19.411, 5990) -- (19.4137, 5999) -- (19.4164, 6004) -- (19.4192, 6003) -- (19.4219, 6005) -- (19.4247, 6017) -- (19.4274, 6035) -- (19.4301, 6042) -- (19.4329, 6047) -- (19.4356, 6050) -- (19.4384, 6050) -- (19.4411, 6057) -- (19.4438, 6062) -- (19.4466, 6061) -- (19.4493, 6070) -- (19.4521, 6075) -- (19.4548, 6081) -- (19.4575, 6079) -- (19.4603, 6077) -- (19.463, 6083) -- (19.4658, 6090) -- (19.4685, 6105) -- (19.4712, 6112) -- (19.474, 6124) -- (19.4767, 6126) -- (19.4795, 6130) -- (19.4822, 6144) -- (19.4849, 6156) -- (19.4877, 6169) -- (19.4904, 6178) -- (19.4932, 6181) -- (19.4959, 6191) -- (19.4986, 6194) -- (19.5014, 6198) -- (19.5041, 6203) -- (19.5068, 6208) -- (19.5096, 6219) -- (19.5123, 6222) -- (19.5151, 6233) -- (19.5178, 6228) -- (19.5205, 6236) -- (19.5233, 6247) -- (19.526, 6258) -- (19.5288, 6262) -- (19.5315, 6255) -- (19.5342, 6254) -- (19.537, 6260) -- (19.5397, 6267) -- (19.5425, 6269) -- (19.5452, 6281) -- (19.5479, 6277) -- (19.5507, 6279) -- (19.5534, 6285) -- (19.5562, 6283) -- (19.5589, 6289) -- (19.5616, 6297) -- (19.5644, 6306) -- (19.5671, 6312) -- (19.5699, 6312) -- (19.5726, 6328) -- (19.5753, 6340) -- (19.5781, 6341) -- (19.5808, 6353) -- (19.5836, 6357) -- (19.5863, 6364) -- (19.589, 6362) -- (19.5918, 6376) -- (19.5945, 6379) -- (19.5973, 6377) -- (19.6, 6384) -- (19.6027, 6388) -- (19.6055, 6397) -- (19.6082, 6397) -- (19.611, 6385) -- (19.6137, 6386) -- (19.6164, 6388) -- (19.6192, 6400) -- (19.6219, 6404) -- (19.6247, 6412) -- (19.6274, 6411) -- (19.6301, 6407) -- (19.6329, 6408) -- (19.6356, 6415) -- (19.6384, 6424) -- (19.6411, 6440) -- (19.6438, 6446) -- (19.6466, 6438) -- (19.6493, 6448) -- (19.6521, 6441) -- (19.6548, 6436) -- (19.6575, 6433) -- (19.6603, 6432) -- (19.663, 6428) -- (19.6658, 6429) -- (19.6685, 6430) -- (19.6712, 6435) -- (19.674, 6445) -- (19.6767, 6445) -- (19.6795, 6454) -- (19.6822, 6457) -- (19.6849, 6464) -- (19.6877, 6469) -- (19.6904, 6469) -- (19.6932, 6470) -- (19.6959, 6485) -- (19.6986, 6492) -- (19.7014, 6498) -- (19.7041, 6493) -- (19.7068, 6487) -- (19.7096, 6485) -- (19.7123, 6490) -- (19.7151, 6490) -- (19.7178, 6496) -- (19.7205, 6491) -- (19.7233, 6485) -- (19.726, 6484) -- (19.7288, 6486) -- (19.7315, 6494) -- (19.7342, 6492) -- (19.737, 6487) -- (19.7397, 6490) -- (19.7425, 6490) -- (19.7452, 6494) -- (19.7479, 6505) -- (19.7507, 6498) -- (19.7534, 6506) -- (19.7562, 6508) -- (19.7589, 6516) -- (19.7616, 6502) -- (19.7644, 6492) -- (19.7671, 6491) -- (19.7699, 6487) -- (19.7726, 6473) -- (19.7753, 6478) -- (19.7781, 6481) -- (19.7808, 6478) -- (19.7836, 6500) -- (19.7863, 6516) -- (19.789, 6513) -- (19.7918, 6537) -- (19.7945, 6551) -- (19.7973, 6565) -- (19.8, 6572) -- (19.8027, 6566) -- (19.8055, 6577) -- (19.8082, 6581) -- (19.811, 6570) -- (19.8137, 6574) -- (19.8164, 6580) -- (19.8192, 6579) -- (19.8219, 6576) -- (19.8247, 6589) -- (19.8274, 6597) -- (19.8301, 6609) -- (19.8329, 6620) -- (19.8356, 6622) -- (19.8384, 6627) -- (19.8411, 6627) -- (19.8438, 6637) -- (19.8466, 6629) -- (19.8493, 6624) -- (19.8521, 6632) -- (19.8548, 6632) -- (19.8575, 6632) -- (19.8603, 6625) -- (19.863, 6627) -- (19.8658, 6629) -- (19.8685, 6632) -- (19.8712, 6626) -- (19.874, 6624) -- (19.8767, 6620) -- (19.8795, 6626) -- (19.8822, 6638) -- (19.8849, 6688) -- (19.8877, 6692) -- (19.8904, 6683) -- (19.8932, 6681) -- (19.8959, 6677) -- (19.8986, 6668) -- (19.9014, 6656) -- (19.9041, 6658) -- (19.9068, 6655) -- (19.9096, 6661) -- (19.9123, 6663) -- (19.9151, 6659) -- (19.9178, 6670) -- (19.9205, 6677) -- (19.9233, 6686) -- (19.926, 6675) -- (19.9288, 6670) -- (19.9315, 6675) -- (19.9342, 6676) -- (19.937, 6678) -- (19.9397, 6681) -- (19.9425, 6685) -- (19.9452, 6679) -- (19.9479, 6683) -- (19.9507, 6675) -- (19.9534, 6678) -- (19.9562, 6679) -- (19.9589, 6682) -- (19.9616, 6686) -- (19.9644, 6687) -- (19.9671, 6685) -- (19.9699, 6690) -- (19.9726, 6695) -- (19.9753, 6694) -- (19.9781, 6689) -- (19.9808, 6690) -- (19.9836, 6690) -- (19.9863, 6698) -- (19.989, 6697) -- (19.9918, 6688) -- (19.9945, 6682) -- (19.9973, 6675) -- (20, 6675) -- (20.0027, 6680) -- (20.0055, 6675) -- (20.0082, 6682) -- (20.0109, 6670) -- (20.0137, 6675) -- (20.0164, 6669) -- (20.0191, 6677) -- (20.0219, 6680) -- (20.0246, 6688) -- (20.0273, 6696) -- (20.0301, 6686) -- (20.0328, 6681) -- (20.0355, 6679) -- (20.0383, 6678) -- (20.041, 6678) -- (20.0437, 6679) -- (20.0464, 6675) -- (20.0492, 6666) -- (20.0519, 6661) -- (20.0546, 6662) -- (20.0574, 6671) -- (20.0601, 6670) -- (20.0628, 6683) -- (20.0656, 6692) -- (20.0683, 6691) -- (20.071, 6686) -- (20.0738, 6694) -- (20.0765, 6695) -- (20.0792, 6695) -- (20.082, 6697) -- (20.0847, 6697) -- (20.0874, 6693) -- (20.0902, 6698) -- (20.0929, 6694) -- (20.0956, 6691) -- (20.0984, 6691) -- (20.1011, 6685) -- (20.1038, 6684) -- (20.1066, 6685) -- (20.1093, 6674) -- (20.112, 6663) -- (20.1148, 6670) -- (20.1175, 6666) -- (20.1202, 6663) -- (20.123, 6658) -- (20.1257, 6661) -- (20.1284, 6661) -- (20.1311, 6660) -- (20.1339, 6667) -- (20.1366, 6655) -- (20.1393, 6667) -- (20.1421, 6666) -- (20.1448, 6664) -- (20.1475, 6656) -- (20.1503, 6663) -- (20.153, 6668) -- (20.1557, 6680) -- (20.1585, 6689) -- (20.1612, 6698) -- (20.1639, 6694) -- (20.1667, 6697) -- (20.1694, 6697) -- (20.1721, 6695) -- (20.1749, 6700) -- (20.1776, 6701) -- (20.1803, 6702) -- (20.1831, 6700) -- (20.1858, 6699) -- (20.1885, 6701) -- (20.1913, 6702) -- (20.194, 6706) -- (20.1967, 6708) -- (20.1995, 6714) -- (20.2022, 6714) -- (20.2049, 6720) -- (20.2077, 6720) -- (20.2104, 6726) -- (20.2131, 6734) -- (20.2158, 6738) -- (20.2186, 6746) -- (20.2213, 6752) -- (20.224, 6746) -- (20.2268, 6740) -- (20.2295, 6747) -- (20.2322, 6760) -- (20.235, 6771) -- (20.2377, 6771) -- (20.2404, 6772) -- (20.2432, 6760) -- (20.2459, 6768) -- (20.2486, 6769) -- (20.2514, 6769) -- (20.2541, 6785) -- (20.2568, 6783) -- (20.2596, 6786) -- (20.2623, 6790) -- (20.265, 6800) -- (20.2678, 6803) -- (20.2705, 6802) -- (20.2732, 6812) -- (20.276, 6828) -- (20.2787, 6820) -- (20.2814, 6820) -- (20.2842, 6825) -- (20.2869, 6818) -- (20.2896, 6810) -- (20.2923, 6813) -- (20.2951, 6815) -- (20.2978, 6821) -- (20.3005, 6819) -- (20.3033, 6821) -- (20.306, 6823) -- (20.3087, 6813) -- (20.3115, 6813) -- (20.3142, 6810) -- (20.3169, 6812) -- (20.3197, 6799) -- (20.3224, 6795) -- (20.3251, 6788) -- (20.3279, 6793) -- (20.3306, 6781) -- (20.3333, 6775) -- (20.3361, 6767) -- (20.3388, 6761) -- (20.3415, 6751) -- (20.3443, 6743) -- (20.347, 6739) -- (20.3497, 6742) -- (20.3525, 6732) -- (20.3552, 6727) -- (20.3579, 6715) -- (20.3607, 6705) -- (20.3634, 6698) -- (20.3661, 6685) -- (20.3689, 6687) -- (20.3716, 6685) -- (20.3743, 6679) -- (20.377, 6709) -- (20.3798, 6643) -- (20.3825, 6601) -- (20.3852, 6584) -- (20.388, 6581) -- (20.3907, 6559) -- (20.3934, 6545) -- (20.3962, 6518) -- (20.3989, 6481) -- (20.4016, 6471) -- (20.4044, 6450) -- (20.4071, 6443) -- (20.4098, 6414) -- (20.4126, 6356) -- (20.4153, 6268) -- (20.418, 6198) -- (20.4208, 6175) -- (20.4235, 6150) -- (20.4262, 6196) -- (20.429, 6212) -- (20.4317, 6218) -- (20.4344, 6192) -- (20.4372, 6182) -- (20.4399, 6176) -- (20.4426, 6160) -- (20.4454, 6159) -- (20.4481, 6155) -- (20.4508, 6146) -- (20.4536, 6128) -- (20.4563, 6116) -- (20.459, 6102) -- (20.4617, 6102) -- (20.4645, 6084) -- (20.4672, 6071) -- (20.4699, 6059) -- (20.4727, 6037) -- (20.4754, 6028) -- (20.4781, 6013) -- (20.4809, 6007) -- (20.4836, 5989) -- (20.4863, 5971) -- (20.4891, 5972) -- (20.4918, 5928) -- (20.4945, 5895) -- (20.4973, 5865) -- (20.5, 5849) -- (20.5027, 5840) -- (20.5055, 5815) -- (20.5082, 5800) -- (20.5109, 5760) -- (20.5137, 5745) -- (20.5164, 5731) -- (20.5191, 5710) -- (20.5219, 5698) -- (20.5246, 5687) -- (20.5273, 5650) -- (20.5301, 5636) -- (20.5328, 5614) -- (20.5355, 5581) -- (20.5383, 5547) -- (20.541, 5533) -- (20.5437, 5495) -- (20.5464, 5468) -- (20.5492, 5427) -- (20.5519, 5387) -- (20.5546, 5368) -- (20.5574, 5329) -- (20.5601, 5304) -- (20.5628, 5262) -- (20.5656, 5238) -- (20.5683, 5211) -- (20.571, 5167) -- (20.5738, 5129) -- (20.5765, 5091) -- (20.5792, 5058) -- (20.582, 5022) -- (20.5847, 4990) -- (20.5874, 4952) -- (20.5902, 4906) -- (20.5929, 4867) -- (20.5956, 4817) -- (20.5984, 4776) -- (20.6011, 4729) -- (20.6038, 4688) -- (20.6066, 4630) -- (20.6093, 4570) -- (20.612, 4497) -- (20.6148, 4441) -- (20.6175, 4382) -- (20.6202, 4357) -- (20.623, 4330) -- (20.6257, 4300) -- (20.6284, 4263) -- (20.6311, 4247) -- (20.6339, 4217) -- (20.6366, 4209) -- (20.6393, 4203) -- (20.6421, 4186) -- (20.6448, 4163) -- (20.6475, 4145) -- (20.6503, 4122) -- (20.653, 4112) -- (20.6557, 4098) -- (20.6585, 4090) -- (20.6612, 4078) -- (20.6639, 4067) -- (20.6667, 4035) -- (20.6694, 4006) -- (20.6721, 3978) -- (20.6749, 3969) -- (20.6776, 3955) -- (20.6803, 3940) -- (20.6831, 3941) -- (20.6858, 3927) -- (20.6885, 3917) -- (20.6913, 3909) -- (20.694, 3904) -- (20.6967, 3894) -- (20.6995, 3877) -- (20.7022, 3866) -- (20.7049, 3841) -- (20.7077, 3823) -- (20.7104, 3809) -- (20.7131, 3805) -- (20.7158, 3791) -- (20.7186, 3778) -- (20.7213, 3765) -- (20.724, 3741) -- (20.7268, 3728) -- (20.7295, 3703) -- (20.7322, 3694) -- (20.735, 3679) -- (20.7377, 3663) -- (20.7404, 3639) -- (20.7432, 3616) -- (20.7459, 3604) -- (20.7486, 3588) -- (20.7514, 3568) -- (20.7541, 3549) -- (20.7568, 3522) -- (20.7596, 3508) -- (20.7623, 3510) -- (20.765, 3491) -- (20.7678, 3460) -- (20.7705, 3442) -- (20.7732, 3427) -- (20.776, 3405) -- (20.7787, 3388) -- (20.7814, 3386) -- (20.7842, 3360) -- (20.7869, 3347) -- (20.7896, 3329) -- (20.7923, 3314) -- (20.7951, 3296) -- (20.7978, 3283) -- (20.8005, 3261) -- (20.8033, 3246) -- (20.806, 3231) -- (20.8087, 3218) -- (20.8115, 3208) -- (20.8142, 3189) -- (20.8169, 3182) -- (20.8197, 3172) -- (20.8224, 3156) -- (20.8251, 3145) -- (20.8279, 3128) -- (20.8306, 3111) -- (20.8333, 3103) -- (20.8361, 3091) -- (20.8388, 3077) -- (20.8415, 3057) -- (20.8443, 3042) -- (20.847, 3028) -- (20.8497, 3013) -- (20.8525, 2999) -- (20.8552, 2980) -- (20.8579, 2966) -- (20.8607, 2949) -- (20.8634, 2936) -- (20.8661, 2925) -- (20.8689, 2910) -- (20.8716, 2752) -- (20.8743, 2723) -- (20.877, 2710) -- (20.8798, 2706) -- (20.8825, 2685) -- (20.8852, 2673) -- (20.888, 2663) -- (20.8907, 2655) -- (20.8934, 2632) -- (20.8962, 2609) -- (20.8989, 2588) -- (20.9016, 2571) -- (20.9044, 2562) -- (20.9071, 2544) -- (20.9098, 2526) -- (20.9126, 2507) -- (20.9153, 2495) -- (20.918, 2475) -- (20.9208, 2467) -- (20.9235, 2460) -- (20.9262, 2459) -- (20.929, 2443) -- (20.9317, 2423) -- (20.9344, 2407) -- (20.9372, 2398) -- (20.9399, 2388) -- (20.9426, 2376) -- (20.9454, 2366) -- (20.9481, 2353) -- (20.9508, 2353) -- (20.9536, 2342) -- (20.9563, 2332) -- (20.959, 2319) -- (20.9617, 2312) -- (20.9645, 2302) -- (20.9672, 2291) -- (20.9699, 2283) -- (20.9727, 2266) -- (20.9754, 2253) -- (20.9781, 2233) -- (20.9809, 2218) -- (20.9836, 2212) -- (20.9863, 2197) -- (20.9891, 2190) -- (20.9918, 2179) -- (20.9945, 2173) -- (20.9973, 2166) -- (21, 2156) -- (21.0027, 2147) -- (21.0055, 2138) -- (21.0082, 2132) -- (21.011, 2114) -- (21.0137, 2105) -- (21.0164, 2085) -- (21.0192, 2081) -- (21.0219, 2078) -- (21.0247, 2064) -- (21.0274, 2057) -- (21.0301, 2044) -- (21.0329, 2034) -- (21.0356, 2011) -- (21.0384, 2003) -- (21.0411, 1980) -- (21.0438, 1960) -- (21.0466, 1952) -- (21.0493, 1934) -- (21.0521, 1922) -- (21.0548, 1892) -- (21.0575, 1873) -- (21.0603, 1861) -- (21.063, 1843) -- (21.0658, 1828) -- (21.0685, 1812) -- (21.0712, 1794) -- (21.074, 1770) -- (21.0767, 1759) -- (21.0795, 1755) -- (21.0822, 1735) -- (21.0849, 1719) -- (21.0877, 1702) -- (21.0904, 1686) -- (21.0932, 1669) -- (21.0959, 1659) -- (21.0986, 1651) -- (21.1014, 1644) -- (21.1041, 1623) -- (21.1068, 1592) -- (21.1096, 1575) -- (21.1123, 1570) -- (21.1151, 1563) -- (21.1178, 1555) -- (21.1205, 1547) -- (21.1233, 1541) -- (21.126, 1539) -- (21.1288, 1528) -- (21.1315, 1523) -- (21.1342, 1519) -- (21.1342, 0) -- (18.2932, 0) -- cycle;

==> data/tcf2-transition/quantcast/stacked/v2-new.tex <==
\draw (18.2932, 1) -- (18.2959, 1) -- (18.2986, 1) -- (18.3014, 1) -- (18.3041, 1) -- (18.3068, 1) -- (18.3096, 1) -- (18.3123, 1) -- (18.3151, 1) -- (18.3178, 1) -- (18.3205, 2) -- (18.3233, 2) -- (18.326, 2) -- (18.3288, 2) -- (18.3315, 2) -- (18.3342, 2) -- (18.337, 2) -- (18.3397, 2) -- (18.3425, 2) -- (18.3452, 2) -- (18.3479, 2) -- (18.3507, 2) -- (18.3534, 2) -- (18.3562, 3) -- (18.3589, 3) -- (18.3616, 3) -- (18.3644, 3) -- (18.3671, 5) -- (18.3699, 5) -- (18.3726, 6) -- (18.3753, 9) -- (18.3781, 11) -- (18.3808, 12) -- (18.3836, 14) -- (18.3863, 16) -- (18.389, 21) -- (18.3918, 37) -- (18.3945, 103) -- (18.3973, 198) -- (18.4, 268) -- (18.4027, 307) -- (18.4055, 341) -- (18.4082, 376) -- (18.411, 405) -- (18.4137, 431) -- (18.4164, 451) -- (18.4192, 479) -- (18.4219, 497) -- (18.4247, 513) -- (18.4274, 532) -- (18.4301, 549) -- (18.4329, 584) -- (18.4356, 615) -- (18.4384, 623) -- (18.4411, 641) -- (18.4438, 655) -- (18.4466, 669) -- (18.4493, 689) -- (18.4521, 706) -- (18.4548, 718) -- (18.4575, 727) -- (18.4603, 742) -- (18.463, 751) -- (18.4658, 766) -- (18.4685, 777) -- (18.4712, 789) -- (18.474, 804) -- (18.4767, 812) -- (18.4795, 821) -- (18.4822, 834) -- (18.4849, 844) -- (18.4877, 858) -- (18.4904, 873) -- (18.4932, 881) -- (18.4959, 893) -- (18.4986, 905) -- (18.5014, 924) -- (18.5041, 938) -- (18.5068, 950) -- (18.5096, 956) -- (18.5123, 967) -- (18.5151, 976) -- (18.5178, 985) -- (18.5205, 991) -- (18.5233, 1002) -- (18.526, 1011) -- (18.5288, 1023) -- (18.5315, 1035) -- (18.5342, 1043) -- (18.537, 1057) -- (18.5397, 1070) -- (18.5425, 1078) -- (18.5452, 1091) -- (18.5479, 1105) -- (18.5507, 1113) -- (18.5534, 1121) -- (18.5562, 1133) -- (18.5589, 1144) -- (18.5616, 1144) -- (18.5644, 1144) -- (18.5671, 1144) -- (18.5699, 1163) -- (18.5726, 1181) -- (18.5753, 1201) -- (18.5781, 1214) -- (18.5808, 1233) -- (18.5836, 1245) -- (18.5863, 1266) -- (18.589, 1281) -- (18.5918, 1288) -- (18.5945, 1300) -- (18.5973, 1311) -- (18.6, 1320) -- (18.6027, 1338) -- (18.6055, 1350) -- (18.6082, 1359) -- (18.611, 1374) -- (18.6137, 1384) -- (18.6164, 1398) -- (18.6192, 1404) -- (18.6219, 1409) -- (18.6247, 1420) -- (18.6274, 1432) -- (18.6301, 1446) -- (18.6329, 1457) -- (18.6356, 1471) -- (18.6384, 1484) -- (18.6411, 1499) -- (18.6438, 1505) -- (18.6466, 1514) -- (18.6493, 1524) -- (18.6521, 1538) -- (18.6548, 1549) -- (18.6575, 1558) -- (18.6603, 1572) -- (18.663, 1585) -- (18.6658, 1593) -- (18.6685, 1612) -- (18.6712, 1615) -- (18.674, 1621) -- (18.6767, 1634) -- (18.6795, 1649) -- (18.6822, 1663) -- (18.6849, 1677) -- (18.6877, 1689) -- (18.6904, 1701) -- (18.6932, 1719) -- (18.6959, 1732) -- (18.6986, 1752) -- (18.7014, 1760) -- (18.7041, 1770) -- (18.7068, 1784) -- (18.7096, 1792) -- (18.7123, 1806) -- (18.7151, 1825) -- (18.7178, 1842) -- (18.7205, 1858) -- (18.7233, 1876) -- (18.726, 1887) -- (18.7288, 1901) -- (18.7315, 1915) -- (18.7342, 1924) -- (18.737, 1936) -- (18.7397, 1946) -- (18.7425, 1953) -- (18.7452, 1962) -- (18.7479, 1978) -- (18.7507, 1988) -- (18.7534, 1994) -- (18.7562, 2008) -- (18.7589, 2013) -- (18.7616, 2025) -- (18.7644, 2037) -- (18.7671, 2051) -- (18.7699, 2061) -- (18.7726, 2071) -- (18.7753, 2074) -- (18.7781, 2082) -- (18.7808, 2095) -- (18.7836, 2098) -- (18.7863, 2108) -- (18.789, 2120) -- (18.7918, 2126) -- (18.7945, 2133) -- (18.7973, 2140) -- (18.8, 2149) -- (18.8027, 2160) -- (18.8055, 2167) -- (18.8082, 2176) -- (18.811, 2190) -- (18.8137, 2206) -- (18.8164, 2217) -- (18.8192, 2231) -- (18.8219, 2242) -- (18.8247, 2254) -- (18.8274, 2263) -- (18.8301, 2278) -- (18.8329, 2292) -- (18.8356, 2337) -- (18.8384, 2394) -- (18.8411, 2430) -- (18.8438, 2466) -- (18.8466, 2502) -- (18.8493, 2552) -- (18.8521, 2593) -- (18.8548, 2635) -- (18.8575, 2661) -- (18.8603, 2688) -- (18.863, 2718) -- (18.8658, 2754) -- (18.8685, 2785) -- (18.8712, 2812) -- (18.874, 2843) -- (18.8767, 2876) -- (18.8795, 2903) -- (18.8822, 2931) -- (18.8849, 2956) -- (18.8877, 2977) -- (18.8904, 2996) -- (18.8932, 3022) -- (18.8959, 3039) -- (18.8986, 3051) -- (18.9014, 3060) -- (18.9041, 3066) -- (18.9068, 3094) -- (18.9096, 3115) -- (18.9123, 3147) -- (18.9151, 3171) -- (18.9178, 3188) -- (18.9205, 3204) -- (18.9233, 3226) -- (18.926, 3251) -- (18.9288, 3274) -- (18.9315, 3287) -- (18.9342, 3305) -- (18.937, 3320) -- (18.9397, 3336) -- (18.9425, 3359) -- (18.9452, 3383) -- (18.9479, 3392) -- (18.9507, 3411) -- (18.9534, 3425) -- (18.9562, 3441) -- (18.9589, 3464) -- (18.9616, 3487) -- (18.9644, 3507) -- (18.9671, 3518) -- (18.9699, 3536) -- (18.9726, 3552) -- (18.9753, 3564) -- (18.9781, 3578) -- (18.9808, 3586) -- (18.9836, 3597) -- (18.9863, 3611) -- (18.989, 3632) -- (18.9918, 3637) -- (18.9945, 3643) -- (18.9973, 3654) -- (19, 3659) -- (19.0027, 3677) -- (19.0055, 3692) -- (19.0082, 3699) -- (19.011, 3707) -- (19.0137, 3715) -- (19.0164, 3728) -- (19.0192, 3746) -- (19.0219, 3758) -- (19.0247, 3776) -- (19.0274, 3796) -- (19.0301, 3806) -- (19.0329, 3813) -- (19.0356, 3833) -- (19.0384, 3860) -- (19.0411, 3876) -- (19.0438, 3884) -- (19.0466, 3898) -- (19.0493, 3911) -- (19.0521, 3925) -- (19.0548, 3940) -- (19.0575, 3961) -- (19.0603, 3984) -- (19.063, 4006) -- (19.0658, 4035) -- (19.0685, 4048) -- (19.0712, 4064) -- (19.074, 4076) -- (19.0767, 4087) -- (19.0795, 4102) -- (19.0822, 4120) -- (19.0849, 4145) -- (19.0877, 4167) -- (19.0904, 4186) -- (19.0932, 4200) -- (19.0959, 4216) -- (19.0986, 4232) -- (19.1014, 4259) -- (19.1041, 4274) -- (19.1068, 4298) -- (19.1096, 4312) -- (19.1123, 4340) -- (19.1151, 4367) -- (19.1178, 4391) -- (19.1205, 4427) -- (19.1233, 4453) -- (19.126, 4479) -- (19.1288, 4504) -- (19.1315, 4524) -- (19.1342, 4544) -- (19.137, 4579) -- (19.1397, 4609) -- (19.1425, 4643) -- (19.1452, 4665) -- (19.1479, 4691) -- (19.1507, 4709) -- (19.1534, 4732) -- (19.1562, 4754) -- (19.1589, 4781) -- (19.1616, 4811) -- (19.1644, 4835) -- (19.1671, 4858) -- (19.1699, 4883) -- (19.1726, 4907) -- (19.1753, 4921) -- (19.1781, 4933) -- (19.1808, 4967) -- (19.1836, 4981) -- (19.1863, 4993) -- (19.189, 5007) -- (19.1918, 5026) -- (19.1945, 5046) -- (19.1973, 5065) -- (19.2, 5091) -- (19.2027, 5108) -- (19.2055, 5127) -- (19.2082, 5155) -- (19.211, 5174) -- (19.2137, 5199) -- (19.2164, 5217) -- (19.2192, 5239) -- (19.2219, 5251) -- (19.2247, 5271) -- (19.2274, 5295) -- (19.2301, 5313) -- (19.2329, 5339) -- (19.2356, 5380) -- (19.2384, 5410) -- (19.2411, 5425) -- (19.2438, 5442) -- (19.2466, 5460) -- (19.2493, 5474) -- (19.2521, 5489) -- (19.2548, 5515) -- (19.2575, 5535) -- (19.2603, 5551) -- (19.263, 5563) -- (19.2658, 5582) -- (19.2685, 5597) -- (19.2712, 5625) -- (19.274, 5639) -- (19.2767, 5673) -- (19.2795, 5685) -- (19.2822, 5706) -- (19.2849, 5728) -- (19.2877, 5747) -- (19.2904, 5766) -- (19.2932, 5780) -- (19.2959, 5797) -- (19.2986, 5809) -- (19.3014, 5815) -- (19.3041, 5829) -- (19.3068, 5846) -- (19.3096, 5860) -- (19.3123, 5871) -- (19.3151, 5902) -- (19.3178, 5914) -- (19.3205, 5934) -- (19.3233, 5943) -- (19.326, 5954) -- (19.3288, 5961) -- (19.3315, 5968) -- (19.3342, 5972) -- (19.337, 5976) -- (19.3397, 5978) -- (19.3425, 5989) -- (19.3452, 5996) -- (19.3479, 6002) -- (19.3507, 6009) -- (19.3534, 6025) -- (19.3562, 6035) -- (19.3589, 6039) -- (19.3616, 6050) -- (19.3644, 6059) -- (19.3671, 6075) -- (19.3699, 6084) -- (19.3726, 6092) -- (19.3753, 6102) -- (19.3781, 6111) -- (19.3808, 6117) -- (19.3836, 6121) -- (19.3863, 6123) -- (19.389, 6121) -- (19.3918, 6129) -- (19.3945, 6145) -- (19.3973, 6152) -- (19.4, 6161) -- (19.4027, 6172) -- (19.4055, 6177) -- (19.4082, 6187) -- (19.411, 6202) -- (19.4137, 6212) -- (19.4164, 6218) -- (19.4192, 6221) -- (19.4219, 6223) -- (19.4247, 6238) -- (19.4274, 6256) -- (19.4301, 6265) -- (19.4329, 6270) -- (19.4356, 6275) -- (19.4384, 6277) -- (19.4411, 6286) -- (19.4438, 6293) -- (19.4466, 6293) -- (19.4493, 6300) -- (19.4521, 6305) -- (19.4548, 6315) -- (19.4575, 6319) -- (19.4603, 6318) -- (19.463, 6327) -- (19.4658, 6333) -- (19.4685, 6350) -- (19.4712, 6357) -- (19.474, 6366) -- (19.4767, 6373) -- (19.4795, 6376) -- (19.4822, 6389) -- (19.4849, 6399) -- (19.4877, 6413) -- (19.4904, 6422) -- (19.4932, 6423) -- (19.4959, 6436) -- (19.4986, 6441) -- (19.5014, 6447) -- (19.5041, 6452) -- (19.5068, 6459) -- (19.5096, 6471) -- (19.5123, 6474) -- (19.5151, 6486) -- (19.5178, 6484) -- (19.5205, 6492) -- (19.5233, 6505) -- (19.526, 6515) -- (19.5288, 6520) -- (19.5315, 6514) -- (19.5342, 6517) -- (19.537, 6522) -- (19.5397, 6531) -- (19.5425, 6533) -- (19.5452, 6544) -- (19.5479, 6544) -- (19.5507, 6547) -- (19.5534, 6555) -- (19.5562, 6554) -- (19.5589, 6559) -- (19.5616, 6568) -- (19.5644, 6576) -- (19.5671, 6583) -- (19.5699, 6583) -- (19.5726, 6599) -- (19.5753, 6612) -- (19.5781, 6611) -- (19.5808, 6624) -- (19.5836, 6628) -- (19.5863, 6635) -- (19.589, 6632) -- (19.5918, 6647) -- (19.5945, 6650) -- (19.5973, 6649) -- (19.6, 6658) -- (19.6027, 6664) -- (19.6055, 6674) -- (19.6082, 6678) -- (19.611, 6674) -- (19.6137, 6676) -- (19.6164, 6681) -- (19.6192, 6693) -- (19.6219, 6698) -- (19.6247, 6709) -- (19.6274, 6713) -- (19.6301, 6709) -- (19.6329, 6712) -- (19.6356, 6718) -- (19.6384, 6728) -- (19.6411, 6742) -- (19.6438, 6751) -- (19.6466, 6744) -- (19.6493, 6752) -- (19.6521, 6750) -- (19.6548, 6746) -- (19.6575, 6751) -- (19.6603, 6760) -- (19.663, 6771) -- (19.6658, 6782) -- (19.6685, 6786) -- (19.6712, 6794) -- (19.674, 6803) -- (19.6767, 6804) -- (19.6795, 6815) -- (19.6822, 6815) -- (19.6849, 6823) -- (19.6877, 6828) -- (19.6904, 6830) -- (19.6932, 6835) -- (19.6959, 6848) -- (19.6986, 6859) -- (19.7014, 6876) -- (19.7041, 6878) -- (19.7068, 6877) -- (19.7096, 6875) -- (19.7123, 6884) -- (19.7151, 6888) -- (19.7178, 6895) -- (19.7205, 6894) -- (19.7233, 6889) -- (19.726, 6889) -- (19.7288, 6891) -- (19.7315, 6901) -- (19.7342, 6901) -- (19.737, 6898) -- (19.7397, 6902) -- (19.7425, 6905) -- (19.7452, 6911) -- (19.7479, 6925) -- (19.7507, 6921) -- (19.7534, 6931) -- (19.7562, 6938) -- (19.7589, 6948) -- (19.7616, 6935) -- (19.7644, 6931) -- (19.7671, 6931) -- (19.7699, 6932) -- (19.7726, 6924) -- (19.7753, 6933) -- (19.7781, 6936) -- (19.7808, 6934) -- (19.7836, 6959) -- (19.7863, 6974) -- (19.789, 6976) -- (19.7918, 7001) -- (19.7945, 7022) -- (19.7973, 7035) -- (19.8, 7043) -- (19.8027, 7041) -- (19.8055, 7053) -- (19.8082, 7058) -- (19.811, 7050) -- (19.8137, 7059) -- (19.8164, 7070) -- (19.8192, 7074) -- (19.8219, 7079) -- (19.8247, 7089) -- (19.8274, 7100) -- (19.8301, 7112) -- (19.8329, 7123) -- (19.8356, 7127) -- (19.8384, 7132) -- (19.8411, 7137) -- (19.8438, 7149) -- (19.8466, 7149) -- (19.8493, 7145) -- (19.8521, 7153) -- (19.8548, 7154) -- (19.8575, 7156) -- (19.8603, 7155) -- (19.863, 7158) -- (19.8658, 7166) -- (19.8685, 7174) -- (19.8712, 7173) -- (19.874, 7170) -- (19.8767, 7169) -- (19.8795, 7180) -- (19.8822, 7190) -- (19.8849, 7245) -- (19.8877, 7254) -- (19.8904, 7254) -- (19.8932, 7254) -- (19.8959, 7254) -- (19.8986, 7248) -- (19.9014, 7240) -- (19.9041, 7245) -- (19.9068, 7248) -- (19.9096, 7257) -- (19.9123, 7262) -- (19.9151, 7262) -- (19.9178, 7272) -- (19.9205, 7290) -- (19.9233, 7307) -- (19.926, 7300) -- (19.9288, 7301) -- (19.9315, 7307) -- (19.9342, 7310) -- (19.937, 7312) -- (19.9397, 7316) -- (19.9425, 7322) -- (19.9452, 7321) -- (19.9479, 7330) -- (19.9507, 7324) -- (19.9534, 7327) -- (19.9562, 7329) -- (19.9589, 7333) -- (19.9616, 7339) -- (19.9644, 7347) -- (19.9671, 7348) -- (19.9699, 7355) -- (19.9726, 7362) -- (19.9753, 7366) -- (19.9781, 7365) -- (19.9808, 7367) -- (19.9836, 7370) -- (19.9863, 7378) -- (19.989, 7379) -- (19.9918, 7372) -- (19.9945, 7369) -- (19.9973, 7367) -- (20, 7372) -- (20.0027, 7379) -- (20.0055, 7379) -- (20.0082, 7388) -- (20.0109, 7380) -- (20.0137, 7388) -- (20.0164, 7382) -- (20.0191, 7394) -- (20.0219, 7403) -- (20.0246, 7414) -- (20.0273, 7427) -- (20.0301, 7424) -- (20.0328, 7425) -- (20.0355, 7426) -- (20.0383, 7434) -- (20.041, 7447) -- (20.0437, 7459) -- (20.0464, 7462) -- (20.0492, 7466) -- (20.0519, 7471) -- (20.0546, 7469) -- (20.0574, 7477) -- (20.0601, 7479) -- (20.0628, 7491) -- (20.0656, 7500) -- (20.0683, 7502) -- (20.071, 7506) -- (20.0738, 7519) -- (20.0765, 7524) -- (20.0792, 7529) -- (20.082, 7533) -- (20.0847, 7537) -- (20.0874, 7539) -- (20.0902, 7547) -- (20.0929, 7547) -- (20.0956, 7554) -- (20.0984, 7559) -- (20.1011, 7557) -- (20.1038, 7563) -- (20.1066, 7569) -- (20.1093, 7570) -- (20.112, 7574) -- (20.1148, 7579) -- (20.1175, 7592) -- (20.1202, 7595) -- (20.123, 7598) -- (20.1257, 7602) -- (20.1284, 7603) -- (20.1311, 7603) -- (20.1339, 7613) -- (20.1366, 7608) -- (20.1393, 7621) -- (20.1421, 7623) -- (20.1448, 7624) -- (20.1475, 7621) -- (20.1503, 7631) -- (20.153, 7642) -- (20.1557, 7650) -- (20.1585, 7660) -- (20.1612, 7672) -- (20.1639, 7670) -- (20.1667, 7675) -- (20.1694, 7680) -- (20.1721, 7683) -- (20.1749, 7689) -- (20.1776, 7695) -- (20.1803, 7702) -- (20.1831, 7708) -- (20.1858, 7716) -- (20.1885, 7721) -- (20.1913, 7721) -- (20.194, 7728) -- (20.1967, 7736) -- (20.1995, 7764) -- (20.2022, 7782) -- (20.2049, 7803) -- (20.2077, 7816) -- (20.2104, 7833) -- (20.2131, 7857) -- (20.2158, 7873) -- (20.2186, 7894) -- (20.2213, 7908) -- (20.224, 7908) -- (20.2268, 7909) -- (20.2295, 7930) -- (20.2322, 7956) -- (20.235, 7981) -- (20.2377, 7991) -- (20.2404, 7996) -- (20.2432, 7998) -- (20.2459, 8011) -- (20.2486, 8022) -- (20.2514, 8031) -- (20.2541, 8052) -- (20.2568, 8066) -- (20.2596, 8074) -- (20.2623, 8083) -- (20.265, 8095) -- (20.2678, 8109) -- (20.2705, 8121) -- (20.2732, 8136) -- (20.276, 8152) -- (20.2787, 8152) -- (20.2814, 8156) -- (20.2842, 8166) -- (20.2869, 8170) -- (20.2896, 8169) -- (20.2923, 8176) -- (20.2951, 8185) -- (20.2978, 8195) -- (20.3005, 8197) -- (20.3033, 8203) -- (20.306, 8208) -- (20.3087, 8208) -- (20.3115, 8212) -- (20.3142, 8213) -- (20.3169, 8221) -- (20.3197, 8215) -- (20.3224, 8217) -- (20.3251, 8224) -- (20.3279, 8235) -- (20.3306, 8225) -- (20.3333, 8232) -- (20.3361, 8227) -- (20.3388, 8229) -- (20.3415, 8222) -- (20.3443, 8223) -- (20.347, 8228) -- (20.3497, 8243) -- (20.3525, 8249) -- (20.3552, 8251) -- (20.3579, 8248) -- (20.3607, 8246) -- (20.3634, 8253) -- (20.3661, 8255) -- (20.3689, 8269) -- (20.3716, 8280) -- (20.3743, 8281) -- (20.377, 8327) -- (20.3798, 8317) -- (20.3825, 8301) -- (20.3852, 8315) -- (20.388, 8337) -- (20.3907, 8339) -- (20.3934, 8344) -- (20.3962, 8337) -- (20.3989, 8322) -- (20.4016, 8330) -- (20.4044, 8332) -- (20.4071, 8334) -- (20.4098, 8327) -- (20.4126, 8269) -- (20.4153, 8193) -- (20.418, 8137) -- (20.4208, 8129) -- (20.4235, 8134) -- (20.4262, 8207) -- (20.429, 8239) -- (20.4317, 8269) -- (20.4344, 8265) -- (20.4372, 8265) -- (20.4399, 8274) -- (20.4426, 8280) -- (20.4454, 8295) -- (20.4481, 8301) -- (20.4508, 8300) -- (20.4536, 8306) -- (20.4563, 8304) -- (20.459, 8305) -- (20.4617, 8322) -- (20.4645, 8323) -- (20.4672, 8320) -- (20.4699, 8319) -- (20.4727, 8321) -- (20.4754, 8325) -- (20.4781, 8331) -- (20.4809, 8335) -- (20.4836, 8348) -- (20.4863, 8358) -- (20.4891, 8362) -- (20.4918, 8363) -- (20.4945, 8352) -- (20.4973, 8360) -- (20.5, 8363) -- (20.5027, 8371) -- (20.5055, 8372) -- (20.5082, 8368) -- (20.5109, 8372) -- (20.5137, 8364) -- (20.5164, 8370) -- (20.5191, 8371) -- (20.5219, 8382) -- (20.5246, 8381) -- (20.5273, 8364) -- (20.5301, 8363) -- (20.5328, 8362) -- (20.5355, 8362) -- (20.5383, 8362) -- (20.541, 8370) -- (20.5437, 8362) -- (20.5464, 8350) -- (20.5492, 8365) -- (20.5519, 8370) -- (20.5546, 8391) -- (20.5574, 8400) -- (20.5601, 8410) -- (20.5628, 8421) -- (20.5656, 8434) -- (20.5683, 8440) -- (20.571, 8446) -- (20.5738, 8458) -- (20.5765, 8463) -- (20.5792, 8475) -- (20.582, 8478) -- (20.5847, 8471) -- (20.5874, 8480) -- (20.5902, 8484) -- (20.5929, 8488) -- (20.5956, 8489) -- (20.5984, 8498) -- (20.6011, 8501) -- (20.6038, 8503) -- (20.6066, 8523) -- (20.6093, 8536) -- (20.612, 8551) -- (20.6148, 8583) -- (20.6175, 8607) -- (20.6202, 8635) -- (20.623, 8650) -- (20.6257, 8663) -- (20.6284, 8674) -- (20.6311, 8689) -- (20.6339, 8700) -- (20.6366, 8720) -- (20.6393, 8765) -- (20.6421, 8787) -- (20.6448, 8801) -- (20.6475, 8815) -- (20.6503, 8828) -- (20.653, 8844) -- (20.6557, 8855) -- (20.6585, 8878) -- (20.6612, 8900) -- (20.6639, 8921) -- (20.6667, 8932) -- (20.6694, 8934) -- (20.6721, 8955) -- (20.6749, 8967) -- (20.6776, 8982) -- (20.6803, 8983) -- (20.6831, 9015) -- (20.6858, 9050) -- (20.6885, 9067) -- (20.6913, 9082) -- (20.694, 9109) -- (20.6967, 9135) -- (20.6995, 9137) -- (20.7022, 9142) -- (20.7049, 9159) -- (20.7077, 9175) -- (20.7104, 9189) -- (20.7131, 9203) -- (20.7158, 9211) -- (20.7186, 9212) -- (20.7213, 9216) -- (20.724, 9218) -- (20.7268, 9240) -- (20.7295, 9253) -- (20.7322, 9276) -- (20.735, 9290) -- (20.7377, 9293) -- (20.7404, 9291) -- (20.7432, 9306) -- (20.7459, 9326) -- (20.7486, 9350) -- (20.7514, 9367) -- (20.7541, 9373) -- (20.7568, 9364) -- (20.7596, 9353) -- (20.7623, 9373) -- (20.765, 9389) -- (20.7678, 9394) -- (20.7705, 9416) -- (20.7732, 9416) -- (20.776, 9415) -- (20.7787, 9421) -- (20.7814, 9441) -- (20.7842, 9454) -- (20.7869, 9471) -- (20.7896, 9486) -- (20.7923, 9497) -- (20.7951, 9501) -- (20.7978, 9516) -- (20.8005, 9523) -- (20.8033, 9532) -- (20.806, 9548) -- (20.8087, 9561) -- (20.8115, 9569) -- (20.8142, 9569) -- (20.8169, 9582) -- (20.8197, 9597) -- (20.8224, 9613) -- (20.8251, 9642) -- (20.8279, 9658) -- (20.8306, 9661) -- (20.8333, 9666) -- (20.8361, 9675) -- (20.8388, 9694) -- (20.8415, 9694) -- (20.8443, 9712) -- (20.847, 9718) -- (20.8497, 9720) -- (20.8525, 9720) -- (20.8552, 9719) -- (20.8579, 9726) -- (20.8607, 9737) -- (20.8634, 9748) -- (20.8661, 9756) -- (20.8689, 9759) -- (20.8716, 9608) -- (20.8743, 9590) -- (20.877, 9592) -- (20.8798, 9596) -- (20.8825, 9595) -- (20.8852, 9610) -- (20.888, 9614) -- (20.8907, 9614) -- (20.8934, 9610) -- (20.8962, 9604) -- (20.8989, 9611) -- (20.9016, 9613) -- (20.9044, 9620) -- (20.9071, 9621) -- (20.9098, 9615) -- (20.9126, 9611) -- (20.9153, 9623) -- (20.918, 9620) -- (20.9208, 9627) -- (20.9235, 9649) -- (20.9262, 9677) -- (20.929, 9689) -- (20.9317, 9699) -- (20.9344, 9703) -- (20.9372, 9704) -- (20.9399, 9714) -- (20.9426, 9729) -- (20.9454, 9736) -- (20.9481, 9736) -- (20.9508, 9744) -- (20.9536, 9760) -- (20.9563, 9764) -- (20.959, 9766) -- (20.9617, 9778) -- (20.9645, 9784) -- (20.9672, 9788) -- (20.9699, 9792) -- (20.9727, 9791) -- (20.9754, 9789) -- (20.9781, 9780) -- (20.9809, 9775) -- (20.9836, 9772) -- (20.9863, 9765) -- (20.9891, 9769) -- (20.9918, 9766) -- (20.9945, 9776) -- (20.9973, 9779) -- (21, 9775) -- (21.0027, 9779) -- (21.0055, 9781) -- (21.0082, 9777) -- (21.011, 9772) -- (21.0137, 9779) -- (21.0164, 9761) -- (21.0192, 9768) -- (21.0219, 9781) -- (21.0247, 9776) -- (21.0274, 9780) -- (21.0301, 9774) -- (21.0329, 9769) -- (21.0356, 9763) -- (21.0384, 9764) -- (21.0411, 9754) -- (21.0438, 9749) -- (21.0466, 9747) -- (21.0493, 9741) -- (21.0521, 9737) -- (21.0548, 9725) -- (21.0575, 9719) -- (21.0603, 9720) -- (21.063, 9711) -- (21.0658, 9700) -- (21.0685, 9691) -- (21.0712, 9688) -- (21.074, 9686) -- (21.0767, 9687) -- (21.0795, 9693) -- (21.0822, 9684) -- (21.0849, 9683) -- (21.0877, 9676) -- (21.0904, 9675) -- (21.0932, 9674) -- (21.0959, 9676) -- (21.0986, 9676) -- (21.1014, 9665) -- (21.1041, 9657) -- (21.1068, 9631) -- (21.1096, 9622) -- (21.1123, 9617) -- (21.1151, 9622) -- (21.1178, 9624) -- (21.1205, 9615) -- (21.1233, 9609) -- (21.126, 9616) -- (21.1288, 9615) -- (21.1315, 9617) -- (21.1342, 9614) -- (21.1342, 0) -- (18.2932, 0) -- cycle;

==> data/tcf2-transition/quantcast/stacked/v2-switch.tex <==
\draw (18.2932, 1) -- (18.2959, 1) -- (18.2986, 1) -- (18.3014, 1) -- (18.3041, 1) -- (18.3068, 1) -- (18.3096, 1) -- (18.3123, 1) -- (18.3151, 1) -- (18.3178, 1) -- (18.3205, 2) -- (18.3233, 2) -- (18.326, 2) -- (18.3288, 2) -- (18.3315, 2) -- (18.3342, 2) -- (18.337, 2) -- (18.3397, 2) -- (18.3425, 2) -- (18.3452, 2) -- (18.3479, 2) -- (18.3507, 2) -- (18.3534, 2) -- (18.3562, 3) -- (18.3589, 3) -- (18.3616, 3) -- (18.3644, 3) -- (18.3671, 5) -- (18.3699, 5) -- (18.3726, 6) -- (18.3753, 9) -- (18.3781, 11) -- (18.3808, 12) -- (18.3836, 14) -- (18.3863, 16) -- (18.389, 21) -- (18.3918, 37) -- (18.3945, 103) -- (18.3973, 198) -- (18.4, 268) -- (18.4027, 307) -- (18.4055, 341) -- (18.4082, 376) -- (18.411, 405) -- (18.4137, 431) -- (18.4164, 451) -- (18.4192, 479) -- (18.4219, 497) -- (18.4247, 513) -- (18.4274, 532) -- (18.4301, 549) -- (18.4329, 584) -- (18.4356, 615) -- (18.4384, 623) -- (18.4411, 641) -- (18.4438, 655) -- (18.4466, 669) -- (18.4493, 689) -- (18.4521, 706) -- (18.4548, 718) -- (18.4575, 727) -- (18.4603, 742) -- (18.463, 751) -- (18.4658, 766) -- (18.4685, 777) -- (18.4712, 789) -- (18.474, 804) -- (18.4767, 812) -- (18.4795, 821) -- (18.4822, 834) -- (18.4849, 844) -- (18.4877, 858) -- (18.4904, 873) -- (18.4932, 881) -- (18.4959, 893) -- (18.4986, 905) -- (18.5014, 924) -- (18.5041, 938) -- (18.5068, 950) -- (18.5096, 956) -- (18.5123, 967) -- (18.5151, 976) -- (18.5178, 985) -- (18.5205, 991) -- (18.5233, 1002) -- (18.526, 1011) -- (18.5288, 1023) -- (18.5315, 1035) -- (18.5342, 1043) -- (18.537, 1057) -- (18.5397, 1070) -- (18.5425, 1078) -- (18.5452, 1091) -- (18.5479, 1105) -- (18.5507, 1113) -- (18.5534, 1121) -- (18.5562, 1133) -- (18.5589, 1144) -- (18.5616, 1144) -- (18.5644, 1144) -- (18.5671, 1144) -- (18.5699, 1163) -- (18.5726, 1181) -- (18.5753, 1201) -- (18.5781, 1214) -- (18.5808, 1233) -- (18.5836, 1245) -- (18.5863, 1266) -- (18.589, 1281) -- (18.5918, 1288) -- (18.5945, 1300) -- (18.5973, 1311) -- (18.6, 1320) -- (18.6027, 1338) -- (18.6055, 1350) -- (18.6082, 1359) -- (18.611, 1374) -- (18.6137, 1384) -- (18.6164, 1398) -- (18.6192, 1404) -- (18.6219, 1409) -- (18.6247, 1420) -- (18.6274, 1432) -- (18.6301, 1446) -- (18.6329, 1457) -- (18.6356, 1471) -- (18.6384, 1484) -- (18.6411, 1499) -- (18.6438, 1505) -- (18.6466, 1514) -- (18.6493, 1524) -- (18.6521, 1538) -- (18.6548, 1549) -- (18.6575, 1558) -- (18.6603, 1572) -- (18.663, 1585) -- (18.6658, 1593) -- (18.6685, 1612) -- (18.6712, 1615) -- (18.674, 1621) -- (18.6767, 1634) -- (18.6795, 1649) -- (18.6822, 1663) -- (18.6849, 1677) -- (18.6877, 1689) -- (18.6904, 1701) -- (18.6932, 1719) -- (18.6959, 1732) -- (18.6986, 1752) -- (18.7014, 1760) -- (18.7041, 1770) -- (18.7068, 1784) -- (18.7096, 1792) -- (18.7123, 1806) -- (18.7151, 1825) -- (18.7178, 1842) -- (18.7205, 1858) -- (18.7233, 1876) -- (18.726, 1887) -- (18.7288, 1901) -- (18.7315, 1915) -- (18.7342, 1924) -- (18.737, 1936) -- (18.7397, 1946) -- (18.7425, 1953) -- (18.7452, 1962) -- (18.7479, 1978) -- (18.7507, 1988) -- (18.7534, 1994) -- (18.7562, 2008) -- (18.7589, 2013) -- (18.7616, 2025) -- (18.7644, 2037) -- (18.7671, 2051) -- (18.7699, 2061) -- (18.7726, 2071) -- (18.7753, 2074) -- (18.7781, 2082) -- (18.7808, 2095) -- (18.7836, 2098) -- (18.7863, 2108) -- (18.789, 2120) -- (18.7918, 2126) -- (18.7945, 2133) -- (18.7973, 2140) -- (18.8, 2149) -- (18.8027, 2160) -- (18.8055, 2167) -- (18.8082, 2176) -- (18.811, 2190) -- (18.8137, 2206) -- (18.8164, 2217) -- (18.8192, 2231) -- (18.8219, 2242) -- (18.8247, 2254) -- (18.8274, 2263) -- (18.8301, 2278) -- (18.8329, 2292) -- (18.8356, 2337) -- (18.8384, 2394) -- (18.8411, 2430) -- (18.8438, 2466) -- (18.8466, 2502) -- (18.8493, 2552) -- (18.8521, 2593) -- (18.8548, 2635) -- (18.8575, 2661) -- (18.8603, 2688) -- (18.863, 2718) -- (18.8658, 2754) -- (18.8685, 2785) -- (18.8712, 2812) -- (18.874, 2843) -- (18.8767, 2876) -- (18.8795, 2903) -- (18.8822, 2931) -- (18.8849, 2956) -- (18.8877, 2977) -- (18.8904, 2996) -- (18.8932, 3022) -- (18.8959, 3039) -- (18.8986, 3051) -- (18.9014, 3060) -- (18.9041, 3066) -- (18.9068, 3094) -- (18.9096, 3115) -- (18.9123, 3147) -- (18.9151, 3171) -- (18.9178, 3188) -- (18.9205, 3204) -- (18.9233, 3226) -- (18.926, 3251) -- (18.9288, 3274) -- (18.9315, 3287) -- (18.9342, 3305) -- (18.937, 3320) -- (18.9397, 3336) -- (18.9425, 3359) -- (18.9452, 3383) -- (18.9479, 3392) -- (18.9507, 3411) -- (18.9534, 3425) -- (18.9562, 3441) -- (18.9589, 3464) -- (18.9616, 3487) -- (18.9644, 3507) -- (18.9671, 3518) -- (18.9699, 3536) -- (18.9726, 3552) -- (18.9753, 3564) -- (18.9781, 3578) -- (18.9808, 3586) -- (18.9836, 3597) -- (18.9863, 3611) -- (18.989, 3632) -- (18.9918, 3637) -- (18.9945, 3643) -- (18.9973, 3654) -- (19, 3659) -- (19.0027, 3677) -- (19.0055, 3692) -- (19.0082, 3699) -- (19.011, 3707) -- (19.0137, 3715) -- (19.0164, 3728) -- (19.0192, 3746) -- (19.0219, 3758) -- (19.0247, 3776) -- (19.0274, 3796) -- (19.0301, 3806) -- (19.0329, 3813) -- (19.0356, 3833) -- (19.0384, 3860) -- (19.0411, 3876) -- (19.0438, 3884) -- (19.0466, 3898) -- (19.0493, 3911) -- (19.0521, 3925) -- (19.0548, 3940) -- (19.0575, 3961) -- (19.0603, 3984) -- (19.063, 4006) -- (19.0658, 4035) -- (19.0685, 4048) -- (19.0712, 4064) -- (19.074, 4076) -- (19.0767, 4087) -- (19.0795, 4102) -- (19.0822, 4120) -- (19.0849, 4145) -- (19.0877, 4167) -- (19.0904, 4186) -- (19.0932, 4200) -- (19.0959, 4216) -- (19.0986, 4232) -- (19.1014, 4259) -- (19.1041, 4274) -- (19.1068, 4298) -- (19.1096, 4312) -- (19.1123, 4340) -- (19.1151, 4367) -- (19.1178, 4391) -- (19.1205, 4427) -- (19.1233, 4453) -- (19.126, 4479) -- (19.1288, 4504) -- (19.1315, 4524) -- (19.1342, 4544) -- (19.137, 4579) -- (19.1397, 4609) -- (19.1425, 4643) -- (19.1452, 4665) -- (19.1479, 4691) -- (19.1507, 4709) -- (19.1534, 4732) -- (19.1562, 4754) -- (19.1589, 4781) -- (19.1616, 4811) -- (19.1644, 4835) -- (19.1671, 4858) -- (19.1699, 4883) -- (19.1726, 4907) -- (19.1753, 4921) -- (19.1781, 4933) -- (19.1808, 4967) -- (19.1836, 4981) -- (19.1863, 4993) -- (19.189, 5007) -- (19.1918, 5026) -- (19.1945, 5046) -- (19.1973, 5065) -- (19.2, 5091) -- (19.2027, 5108) -- (19.2055, 5127) -- (19.2082, 5155) -- (19.211, 5174) -- (19.2137, 5199) -- (19.2164, 5217) -- (19.2192, 5239) -- (19.2219, 5251) -- (19.2247, 5271) -- (19.2274, 5295) -- (19.2301, 5313) -- (19.2329, 5339) -- (19.2356, 5380) -- (19.2384, 5410) -- (19.2411, 5425) -- (19.2438, 5442) -- (19.2466, 5460) -- (19.2493, 5474) -- (19.2521, 5489) -- (19.2548, 5515) -- (19.2575, 5535) -- (19.2603, 5551) -- (19.263, 5563) -- (19.2658, 5582) -- (19.2685, 5597) -- (19.2712, 5625) -- (19.274, 5639) -- (19.2767, 5673) -- (19.2795, 5685) -- (19.2822, 5706) -- (19.2849, 5728) -- (19.2877, 5747) -- (19.2904, 5766) -- (19.2932, 5780) -- (19.2959, 5797) -- (19.2986, 5809) -- (19.3014, 5815) -- (19.3041, 5829) -- (19.3068, 5846) -- (19.3096, 5860) -- (19.3123, 5871) -- (19.3151, 5902) -- (19.3178, 5914) -- (19.3205, 5934) -- (19.3233, 5943) -- (19.326, 5954) -- (19.3288, 5961) -- (19.3315, 5967) -- (19.3342, 5971) -- (19.337, 5975) -- (19.3397, 5977) -- (19.3425, 5988) -- (19.3452, 5995) -- (19.3479, 6001) -- (19.3507, 6008) -- (19.3534, 6023) -- (19.3562, 6032) -- (19.3589, 6036) -- (19.3616, 6047) -- (19.3644, 6056) -- (19.3671, 6072) -- (19.3699, 6081) -- (19.3726, 6089) -- (19.3753, 6099) -- (19.3781, 6108) -- (19.3808, 6114) -- (19.3836, 6118) -- (19.3863, 6120) -- (19.389, 6118) -- (19.3918, 6126) -- (19.3945, 6142) -- (19.3973, 6149) -- (19.4, 6158) -- (19.4027, 6169) -- (19.4055, 6174) -- (19.4082, 6184) -- (19.411, 6199) -- (19.4137, 6209) -- (19.4164, 6215) -- (19.4192, 6218) -- (19.4219, 6220) -- (19.4247, 6235) -- (19.4274, 6253) -- (19.4301, 6262) -- (19.4329, 6267) -- (19.4356, 6272) -- (19.4384, 6274) -- (19.4411, 6283) -- (19.4438, 6290) -- (19.4466, 6290) -- (19.4493, 6297) -- (19.4521, 6302) -- (19.4548, 6312) -- (19.4575, 6316) -- (19.4603, 6315) -- (19.463, 6324) -- (19.4658, 6330) -- (19.4685, 6347) -- (19.4712, 6354) -- (19.474, 6363) -- (19.4767, 6370) -- (19.4795, 6373) -- (19.4822, 6386) -- (19.4849, 6396) -- (19.4877, 6410) -- (19.4904, 6419) -- (19.4932, 6420) -- (19.4959, 6433) -- (19.4986, 6438) -- (19.5014, 6444) -- (19.5041, 6449) -- (19.5068, 6456) -- (19.5096, 6468) -- (19.5123, 6471) -- (19.5151, 6483) -- (19.5178, 6480) -- (19.5205, 6488) -- (19.5233, 6501) -- (19.526, 6511) -- (19.5288, 6516) -- (19.5315, 6510) -- (19.5342, 6513) -- (19.537, 6518) -- (19.5397, 6527) -- (19.5425, 6529) -- (19.5452, 6540) -- (19.5479, 6540) -- (19.5507, 6543) -- (19.5534, 6551) -- (19.5562, 6549) -- (19.5589, 6554) -- (19.5616, 6563) -- (19.5644, 6571) -- (19.5671, 6578) -- (19.5699, 6578) -- (19.5726, 6594) -- (19.5753, 6607) -- (19.5781, 6606) -- (19.5808, 6619) -- (19.5836, 6623) -- (19.5863, 6630) -- (19.589, 6627) -- (19.5918, 6642) -- (19.5945, 6645) -- (19.5973, 6644) -- (19.6, 6653) -- (19.6027, 6659) -- (19.6055, 6668) -- (19.6082, 6672) -- (19.611, 6668) -- (19.6137, 6670) -- (19.6164, 6675) -- (19.6192, 6686) -- (19.6219, 6690) -- (19.6247, 6701) -- (19.6274, 6700) -- (19.6301, 6696) -- (19.6329, 6699) -- (19.6356, 6705) -- (19.6384, 6715) -- (19.6411, 6729) -- (19.6438, 6737) -- (19.6466, 6730) -- (19.6493, 6738) -- (19.6521, 6736) -- (19.6548, 6732) -- (19.6575, 6732) -- (19.6603, 6734) -- (19.663, 6730) -- (19.6658, 6729) -- (19.6685, 6733) -- (19.6712, 6740) -- (19.674, 6749) -- (19.6767, 6750) -- (19.6795, 6761) -- (19.6822, 6761) -- (19.6849, 6768) -- (19.6877, 6774) -- (19.6904, 6776) -- (19.6932, 6780) -- (19.6959, 6792) -- (19.6986, 6800) -- (19.7014, 6808) -- (19.7041, 6804) -- (19.7068, 6801) -- (19.7096, 6799) -- (19.7123, 6805) -- (19.7151, 6806) -- (19.7178, 6812) -- (19.7205, 6809) -- (19.7233, 6804) -- (19.726, 6804) -- (19.7288, 6806) -- (19.7315, 6816) -- (19.7342, 6815) -- (19.737, 6812) -- (19.7397, 6815) -- (19.7425, 6818) -- (19.7452, 6821) -- (19.7479, 6835) -- (19.7507, 6830) -- (19.7534, 6838) -- (19.7562, 6844) -- (19.7589, 6853) -- (19.7616, 6840) -- (19.7644, 6836) -- (19.7671, 6836) -- (19.7699, 6836) -- (19.7726, 6827) -- (19.7753, 6834) -- (19.7781, 6837) -- (19.7808, 6834) -- (19.7836, 6858) -- (19.7863, 6871) -- (19.789, 6870) -- (19.7918, 6894) -- (19.7945, 6913) -- (19.7973, 6926) -- (19.8, 6934) -- (19.8027, 6932) -- (19.8055, 6944) -- (19.8082, 6949) -- (19.811, 6941) -- (19.8137, 6949) -- (19.8164, 6958) -- (19.8192, 6960) -- (19.8219, 6964) -- (19.8247, 6974) -- (19.8274, 6985) -- (19.8301, 6996) -- (19.8329, 7006) -- (19.8356, 7009) -- (19.8384, 7014) -- (19.8411, 7018) -- (19.8438, 7030) -- (19.8466, 7030) -- (19.8493, 7026) -- (19.8521, 7035) -- (19.8548, 7036) -- (19.8575, 7038) -- (19.8603, 7036) -- (19.863, 7038) -- (19.8658, 7045) -- (19.8685, 7053) -- (19.8712, 7052) -- (19.874, 7049) -- (19.8767, 7048) -- (19.8795, 7056) -- (19.8822, 7066) -- (19.8849, 7118) -- (19.8877, 7125) -- (19.8904, 7124) -- (19.8932, 7124) -- (19.8959, 7124) -- (19.8986, 7118) -- (19.9014, 7110) -- (19.9041, 7115) -- (19.9068, 7117) -- (19.9096, 7125) -- (19.9123, 7129) -- (19.9151, 7127) -- (19.9178, 7136) -- (19.9205, 7154) -- (19.9233, 7170) -- (19.926, 7163) -- (19.9288, 7164) -- (19.9315, 7170) -- (19.9342, 7173) -- (19.937, 7175) -- (19.9397, 7179) -- (19.9425, 7185) -- (19.9452, 7184) -- (19.9479, 7193) -- (19.9507, 7187) -- (19.9534, 7190) -- (19.9562, 7192) -- (19.9589, 7196) -- (19.9616, 7202) -- (19.9644, 7210) -- (19.9671, 7211) -- (19.9699, 7218) -- (19.9726, 7224) -- (19.9753, 7228) -- (19.9781, 7227) -- (19.9808, 7229) -- (19.9836, 7232) -- (19.9863, 7240) -- (19.989, 7241) -- (19.9918, 7234) -- (19.9945, 7231) -- (19.9973, 7228) -- (20, 7233) -- (20.0027, 7239) -- (20.0055, 7239) -- (20.0082, 7248) -- (20.0109, 7240) -- (20.0137, 7248) -- (20.0164, 7242) -- (20.0191, 7253) -- (20.0219, 7261) -- (20.0246, 7272) -- (20.0273, 7284) -- (20.0301, 7280) -- (20.0328, 7281) -- (20.0355, 7280) -- (20.0383, 7286) -- (20.041, 7295) -- (20.0437, 7305) -- (20.0464, 7305) -- (20.0492, 7302) -- (20.0519, 7306) -- (20.0546, 7304) -- (20.0574, 7312) -- (20.0601, 7312) -- (20.0628, 7320) -- (20.0656, 7329) -- (20.0683, 7329) -- (20.071, 7332) -- (20.0738, 7344) -- (20.0765, 7346) -- (20.0792, 7350) -- (20.082, 7353) -- (20.0847, 7355) -- (20.0874, 7354) -- (20.0902, 7361) -- (20.0929, 7361) -- (20.0956, 7367) -- (20.0984, 7371) -- (20.1011, 7369) -- (20.1038, 7374) -- (20.1066, 7380) -- (20.1093, 7379) -- (20.112, 7381) -- (20.1148, 7385) -- (20.1175, 7398) -- (20.1202, 7398) -- (20.123, 7399) -- (20.1257, 7401) -- (20.1284, 7401) -- (20.1311, 7400) -- (20.1339, 7410) -- (20.1366, 7403) -- (20.1393, 7416) -- (20.1421, 7418) -- (20.1448, 7418) -- (20.1475, 7413) -- (20.1503, 7421) -- (20.153, 7429) -- (20.1557, 7436) -- (20.1585, 7446) -- (20.1612, 7458) -- (20.1639, 7456) -- (20.1667, 7461) -- (20.1694, 7463) -- (20.1721, 7466) -- (20.1749, 7471) -- (20.1776, 7477) -- (20.1803, 7483) -- (20.1831, 7487) -- (20.1858, 7490) -- (20.1885, 7491) -- (20.1913, 7491) -- (20.194, 7496) -- (20.1967, 7502) -- (20.1995, 7511) -- (20.2022, 7513) -- (20.2049, 7521) -- (20.2077, 7526) -- (20.2104, 7533) -- (20.2131, 7545) -- (20.2158, 7549) -- (20.2186, 7561) -- (20.2213, 7569) -- (20.224, 7564) -- (20.2268, 7561) -- (20.2295, 7573) -- (20.2322, 7585) -- (20.235, 7600) -- (20.2377, 7608) -- (20.2404, 7610) -- (20.2432, 7608) -- (20.2459, 7617) -- (20.2486, 7621) -- (20.2514, 7626) -- (20.2541, 7643) -- (20.2568, 7652) -- (20.2596, 7658) -- (20.2623, 7663) -- (20.265, 7673) -- (20.2678, 7679) -- (20.2705, 7682) -- (20.2732, 7695) -- (20.276, 7709) -- (20.2787, 7706) -- (20.2814, 7710) -- (20.2842, 7717) -- (20.2869, 7718) -- (20.2896, 7717) -- (20.2923, 7723) -- (20.2951, 7727) -- (20.2978, 7736) -- (20.3005, 7737) -- (20.3033, 7741) -- (20.306, 7744) -- (20.3087, 7743) -- (20.3115, 7745) -- (20.3142, 7746) -- (20.3169, 7753) -- (20.3197, 7745) -- (20.3224, 7746) -- (20.3251, 7750) -- (20.3279, 7760) -- (20.3306, 7750) -- (20.3333, 7754) -- (20.3361, 7748) -- (20.3388, 7749) -- (20.3415, 7742) -- (20.3443, 7741) -- (20.347, 7744) -- (20.3497, 7753) -- (20.3525, 7756) -- (20.3552, 7755) -- (20.3579, 7751) -- (20.3607, 7746) -- (20.3634, 7748) -- (20.3661, 7744) -- (20.3689, 7749) -- (20.3716, 7756) -- (20.3743, 7754) -- (20.377, 7790) -- (20.3798, 7779) -- (20.3825, 7764) -- (20.3852, 7769) -- (20.388, 7781) -- (20.3907, 7774) -- (20.3934, 7773) -- (20.3962, 7763) -- (20.3989, 7744) -- (20.4016, 7745) -- (20.4044, 7741) -- (20.4071, 7741) -- (20.4098, 7733) -- (20.4126, 7674) -- (20.4153, 7597) -- (20.418, 7537) -- (20.4208, 7528) -- (20.4235, 7525) -- (20.4262, 7588) -- (20.429, 7616) -- (20.4317, 7636) -- (20.4344, 7631) -- (20.4372, 7627) -- (20.4399, 7630) -- (20.4426, 7632) -- (20.4454, 7643) -- (20.4481, 7647) -- (20.4508, 7638) -- (20.4536, 7643) -- (20.4563, 7639) -- (20.459, 7636) -- (20.4617, 7644) -- (20.4645, 7639) -- (20.4672, 7633) -- (20.4699, 7627) -- (20.4727, 7623) -- (20.4754, 7620) -- (20.4781, 7620) -- (20.4809, 7621) -- (20.4836, 7628) -- (20.4863, 7633) -- (20.4891, 7630) -- (20.4918, 7625) -- (20.4945, 7613) -- (20.4973, 7612) -- (20.5, 7611) -- (20.5027, 7614) -- (20.5055, 7613) -- (20.5082, 7604) -- (20.5109, 7602) -- (20.5137, 7589) -- (20.5164, 7587) -- (20.5191, 7581) -- (20.5219, 7589) -- (20.5246, 7584) -- (20.5273, 7567) -- (20.5301, 7560) -- (20.5328, 7553) -- (20.5355, 7546) -- (20.5383, 7537) -- (20.541, 7540) -- (20.5437, 7532) -- (20.5464, 7519) -- (20.5492, 7525) -- (20.5519, 7519) -- (20.5546, 7527) -- (20.5574, 7522) -- (20.5601, 7524) -- (20.5628, 7524) -- (20.5656, 7527) -- (20.5683, 7526) -- (20.571, 7519) -- (20.5738, 7514) -- (20.5765, 7509) -- (20.5792, 7511) -- (20.582, 7505) -- (20.5847, 7491) -- (20.5874, 7485) -- (20.5902, 7479) -- (20.5929, 7477) -- (20.5956, 7465) -- (20.5984, 7457) -- (20.6011, 7450) -- (20.6038, 7443) -- (20.6066, 7442) -- (20.6093, 7436) -- (20.612, 7426) -- (20.6148, 7425) -- (20.6175, 7414) -- (20.6202, 7412) -- (20.623, 7399) -- (20.6257, 7390) -- (20.6284, 7371) -- (20.6311, 7365) -- (20.6339, 7351) -- (20.6366, 7346) -- (20.6393, 7343) -- (20.6421, 7339) -- (20.6448, 7326) -- (20.6475, 7310) -- (20.6503, 7296) -- (20.653, 7293) -- (20.6557, 7282) -- (20.6585, 7281) -- (20.6612, 7277) -- (20.6639, 7268) -- (20.6667, 7256) -- (20.6694, 7242) -- (20.6721, 7230) -- (20.6749, 7231) -- (20.6776, 7227) -- (20.6803, 7214) -- (20.6831, 7215) -- (20.6858, 7215) -- (20.6885, 7206) -- (20.6913, 7199) -- (20.694, 7198) -- (20.6967, 7201) -- (20.6995, 7194) -- (20.7022, 7181) -- (20.7049, 7168) -- (20.7077, 7165) -- (20.7104, 7152) -- (20.7131, 7146) -- (20.7158, 7136) -- (20.7186, 7127) -- (20.7213, 7115) -- (20.724, 7101) -- (20.7268, 7098) -- (20.7295, 7087) -- (20.7322, 7082) -- (20.735, 7078) -- (20.7377, 7064) -- (20.7404, 7042) -- (20.7432, 7027) -- (20.7459, 7022) -- (20.7486, 7012) -- (20.7514, 7005) -- (20.7541, 6996) -- (20.7568, 6977) -- (20.7596, 6967) -- (20.7623, 6962) -- (20.765, 6948) -- (20.7678, 6925) -- (20.7705, 6915) -- (20.7732, 6904) -- (20.776, 6883) -- (20.7787, 6870) -- (20.7814, 6867) -- (20.7842, 6851) -- (20.7869, 6840) -- (20.7896, 6828) -- (20.7923, 6815) -- (20.7951, 6796) -- (20.7978, 6782) -- (20.8005, 6766) -- (20.8033, 6752) -- (20.806, 6738) -- (20.8087, 6726) -- (20.8115, 6713) -- (20.8142, 6698) -- (20.8169, 6690) -- (20.8197, 6680) -- (20.8224, 6664) -- (20.8251, 6662) -- (20.8279, 6649) -- (20.8306, 6635) -- (20.8333, 6627) -- (20.8361, 6609) -- (20.8388, 6604) -- (20.8415, 6590) -- (20.8443, 6572) -- (20.847, 6562) -- (20.8497, 6549) -- (20.8525, 6537) -- (20.8552, 6516) -- (20.8579, 6499) -- (20.8607, 6482) -- (20.8634, 6473) -- (20.8661, 6469) -- (20.8689, 6454) -- (20.8716, 6300) -- (20.8743, 6267) -- (20.877, 6256) -- (20.8798, 6251) -- (20.8825, 6232) -- (20.8852, 6224) -- (20.888, 6213) -- (20.8907, 6205) -- (20.8934, 6183) -- (20.8962, 6159) -- (20.8989, 6147) -- (20.9016, 6129) -- (20.9044, 6117) -- (20.9071, 6103) -- (20.9098, 6088) -- (20.9126, 6068) -- (20.9153, 6057) -- (20.918, 6037) -- (20.9208, 6027) -- (20.9235, 6017) -- (20.9262, 6012) -- (20.929, 5997) -- (20.9317, 5985) -- (20.9344, 5972) -- (20.9372, 5963) -- (20.9399, 5957) -- (20.9426, 5953) -- (20.9454, 5946) -- (20.9481, 5934) -- (20.9508, 5923) -- (20.9536, 5918) -- (20.9563, 5908) -- (20.959, 5899) -- (20.9617, 5889) -- (20.9645, 5886) -- (20.9672, 5878) -- (20.9699, 5864) -- (20.9727, 5853) -- (20.9754, 5838) -- (20.9781, 5822) -- (20.9809, 5809) -- (20.9836, 5802) -- (20.9863, 5789) -- (20.9891, 5773) -- (20.9918, 5763) -- (20.9945, 5756) -- (20.9973, 5749) -- (21, 5739) -- (21.0027, 5729) -- (21.0055, 5719) -- (21.0082, 5703) -- (21.011, 5689) -- (21.0137, 5681) -- (21.0164, 5666) -- (21.0192, 5658) -- (21.0219, 5660) -- (21.0247, 5645) -- (21.0274, 5635) -- (21.0301, 5620) -- (21.0329, 5612) -- (21.0356, 5593) -- (21.0384, 5578) -- (21.0411, 5554) -- (21.0438, 5537) -- (21.0466, 5525) -- (21.0493, 5511) -- (21.0521, 5495) -- (21.0548, 5476) -- (21.0575, 5461) -- (21.0603, 5448) -- (21.063, 5427) -- (21.0658, 5408) -- (21.0685, 5388) -- (21.0712, 5369) -- (21.074, 5347) -- (21.0767, 5335) -- (21.0795, 5320) -- (21.0822, 5303) -- (21.0849, 5281) -- (21.0877, 5260) -- (21.0904, 5241) -- (21.0932, 5220) -- (21.0959, 5208) -- (21.0986, 5197) -- (21.1014, 5185) -- (21.1041, 5159) -- (21.1068, 5117) -- (21.1096, 5096) -- (21.1123, 5077) -- (21.1151, 5064) -- (21.1178, 5055) -- (21.1205, 5040) -- (21.1233, 5018) -- (21.126, 5009) -- (21.1288, 4993) -- (21.1315, 4977) -- (21.1342, 4963) -- (21.1342, 0) -- (18.2932, 0) -- cycle;

==> data/tcf2-transition/tcf_adoption_by_third_parties/tcf1_stacked.tex <==
\draw (0,0.000314434) -- (0.30103,0.00206826) -- (0.477121,0.00534079) -- (0.60206,0.0125898) -- (0.69897,0.0238887) -- (0.778151,0.0350078) -- (0.845098,0.0519665) -- (0.90309,0.0656871) -- (0.954243,0.0737667) -- (1,0.0844069) -- (1.04139,0.099083) -- (1.07918,0.113411) -- (1.11394,0.123492) -- (1.14613,0.127823) -- (1.17609,0.127717) -- (1.20412,0.125617) -- (1.23045,0.123524) -- (1.25527,0.122443) -- (1.27875,0.12236) -- (1.30103,0.122771) -- (1.32222,0.12336) -- (1.34242,0.124183) -- (1.36173,0.125414) -- (1.38021,0.127055) -- (1.39794,0.128895) -- (1.41497,0.130657) -- (1.43136,0.132148) -- (1.44716,0.133322) -- (1.4624,0.134252) -- (1.47712,0.13507) -- (1.49136,0.13592) -- (1.50515,0.136928) -- (1.51851,0.138182) -- (1.53148,0.139731) -- (1.54407,0.141583) -- (1.5563,0.143709) -- (1.5682,0.146061) -- (1.57978,0.148592) -- (1.59106,0.151269) -- (1.60206,0.154086) -- (1.61278,0.157059) -- (1.62325,0.16021) -- (1.63347,0.163546) -- (1.64345,0.167046) -- (1.65321,0.170647) -- (1.66276,0.174245) -- (1.6721,0.177711) -- (1.68124,0.180906) -- (1.6902,0.183707) -- (1.69897,0.186025) -- (1.70757,0.18782) -- (1.716,0.189102) -- (1.72428,0.189933) -- (1.73239,0.190409) -- (1.74036,0.190646) -- (1.74819,0.19077) -- (1.75587,0.190896) -- (1.76343,0.191121) -- (1.77085,0.191516) -- (1.77815,0.192122) -- (1.78533,0.192952) -- (1.79239,0.193987) -- (1.79934,0.195186) -- (1.80618,0.196487) -- (1.81291,0.197816) -- (1.81954,0.199093) -- (1.82607,0.200239) -- (1.83251,0.201185) -- (1.83885,0.201876) -- (1.8451,0.202273) -- (1.85126,0.202361) -- (1.85733,0.202146) -- (1.86332,0.201651) -- (1.86923,0.200922) -- (1.87506,0.200014) -- (1.88081,0.198998) -- (1.88649,0.197946) -- (1.89209,0.196937) -- (1.89763,0.196046) -- (1.90309,0.195344) -- (1.90849,0.194895) -- (1.91381,0.194753) -- (1.91908,0.194961) -- (1.92428,0.195549) -- (1.92942,0.196535) -- (1.9345,0.197924) -- (1.93952,0.199709) -- (1.94448,0.201873) -- (1.94939,0.204387) -- (1.95424,0.207216) -- (1.95904,0.210318) -- (1.96379,0.213645) -- (1.96848,0.21715) -- (1.97313,0.220782) -- (1.97772,0.224494) -- (1.98227,0.22824) -- (1.98677,0.231977) -- (1.99123,0.23567) -- (1.99564,0.239286) -- (2,0.242799)

==> data/tcf2-transition/tcf_adoption_by_third_parties/tcf2.tex <==
\draw (0,0.000112709) -- (0.30103,0.00163181) -- (0.477121,0.00432365) -- (0.60206,0.010771) -- (0.69897,0.0218825) -- (0.778151,0.0326973) -- (0.845098,0.0490532) -- (0.90309,0.0622803) -- (0.954243,0.069977) -- (1,0.0801677) -- (1.04139,0.0943298) -- (1.07918,0.10812) -- (1.11394,0.117603) -- (1.14613,0.121188) -- (1.17609,0.120142) -- (1.20412,0.116923) -- (1.23045,0.113586) -- (1.25527,0.1112) -- (1.27875,0.109804) -- (1.30103,0.108913) -- (1.32222,0.108207) -- (1.34242,0.107749) -- (1.36173,0.10773) -- (1.38021,0.108179) -- (1.39794,0.108904) -- (1.41497,0.10963) -- (1.43136,0.110159) -- (1.44716,0.11044) -- (1.4624,0.11055) -- (1.47712,0.110627) -- (1.49136,0.110824) -- (1.50515,0.111267) -- (1.51851,0.112042) -- (1.53148,0.113188) -- (1.54407,0.114699) -- (1.5563,0.116536) -- (1.5682,0.11864) -- (1.57978,0.12095) -- (1.59106,0.123426) -- (1.60206,0.126049) -- (1.61278,0.128825) -- (1.62325,0.131769) -- (1.63347,0.134882) -- (1.64345,0.138142) -- (1.65321,0.141487) -- (1.66276,0.144822) -- (1.6721,0.148023) -- (1.68124,0.150964) -- (1.6902,0.153531) -- (1.69897,0.155641) -- (1.70757,0.157259) -- (1.716,0.158395) -- (1.72428,0.159107) -- (1.73239,0.159483) -- (1.74036,0.159635) -- (1.74819,0.159676) -- (1.75587,0.159714) -- (1.76343,0.159838) -- (1.77085,0.160115) -- (1.77815,0.160582) -- (1.78533,0.161246) -- (1.79239,0.162088) -- (1.79934,0.163065) -- (1.80618,0.164111) -- (1.81291,0.16515) -- (1.81954,0.166098) -- (1.82607,0.166872) -- (1.83251,0.167397) -- (1.83885,0.167611) -- (1.8451,0.16747) -- (1.85126,0.166952) -- (1.85733,0.166055) -- (1.86332,0.164799) -- (1.86923,0.163222) -- (1.87506,0.161376) -- (1.88081,0.159327) -- (1.88649,0.157147) -- (1.89209,0.154912) -- (1.89763,0.152698) -- (1.90309,0.150576) -- (1.90849,0.148613) -- (1.91381,0.146868) -- (1.91908,0.145387) -- (1.92428,0.144207) -- (1.92942,0.143354) -- (1.9345,0.142843) -- (1.93952,0.142674) -- (1.94448,0.14284) -- (1.94939,0.143325) -- (1.95424,0.144102) -- (1.95904,0.14514) -- (1.96379,0.146403) -- (1.96848,0.14785) -- (1.97313,0.149441) -- (1.97772,0.151134) -- (1.98227,0.152889) -- (1.98677,0.15467) -- (1.99123,0.156442) -- (1.99564,0.158176) -- (2,0.159847)

==> fig/common.tex <==
\providecommand{\paperroot}{..}

\makeatletter
\def\input@path{{\paperroot/}}
\makeatother
\usepackage[big]{dgruyter_NEW}
%
\makeatletter
\p@=1pt
\makeatother
\AtBeginDocument{\baretabulars}

%

\usepackage{tikz}
\usepackage{booktabs}
\usepackage{chngcntr}
\usepackage{stfloats}


\usetikzlibrary{calc}
\usetikzlibrary{fpu}
\usetikzlibrary{decorations}
\usetikzlibrary{fadings}

\tikzset{>=stealth}

\tikzstyle{event} = [
	inner sep=1pt,
	font=\scriptsize,
]
\definecolor{eventline-color}{HTML}{FF9C75}
\tikzstyle{eventline} = [
	draw=eventline-color,
%
%
%
]

%
%
\definecolor{v1-color}{HTML}{00588B}
\definecolor{transition-color}{HTML}{009B95}
\definecolor{v2-switch-color}{HTML}{53CC67}
\definecolor{v2-new-color}{HTML}{FDE333}

%
\definecolor{quantcast-color}{HTML}{56B4E9}
\definecolor{onetrust-color}{HTML}{009E73}
\definecolor{sourcepoint-color}{HTML}{CC79A7}
\definecolor{liveramp-color}{HTML}{0072B2}
\definecolor{google-color}{HTML}{F0E442}
\definecolor{other-color}{HTML}{E69F00}
%
%
%

\definecolor{p3p-color}{HTML}{56B4E9}
\definecolor{dnt-color}{HTML}{009E73}
\definecolor{gpc-color}{HTML}{CC79A7}
\definecolor{nai-color}{HTML}{D55E00}


%
%
\definecolor{legint-color}{HTML}{91008D}
\definecolor{flexible-color}{HTML}{D24E71}
\definecolor{consent-color}{HTML}{EDA200}
\definecolor{noClaim-color}{HTML}{DAFF47}
\definecolor{notInList-color}{HTML}{CCFFCC} %


\definecolor{signal-color}{HTML}{0072B2}
\definecolor{feedback-color}{HTML}{E69F00}
\definecolor{tracking-color}{HTML}{D55E00}


\newcommand{\tcfone}{TCF~1.x}
\newcommand{\tcftwo}{TCF~2.0}
\newcommand{\tcfonex}{TCF~1.x}
\newcommand{\tcftwox}{TCF~2.x}

%

\providecommand{\naiMembers}{91}
\providecommand{\naiOptOutParticipants}{75}

\makeatletter

\newcommand{\bignum}[1]{%
	\pgfkeys{/pgf/fpu=true}%
	\pgfmathparse{#1}%
	\pgfmathprintnumber[fixed]{\pgfmathresult}%
	\pgfkeys{/pgf/fpu=false}%
}

%
\newcommand{\timeaxisx}{2.35cm}
\newcommand{\timeaxis}{
	\draw[->] (18,0) -- (21+2.5/12,0);
	\foreach \year in {18,19,20,21} {
		\pgfmathparse{\year < 21}
		\ifnum \pgfmathresult > 0
			\draw (\year,-15pt) node [right, inner ysep=0] {\small20\year~$\rightarrow$};
		\fi
		\foreach \imonth/\month in {0/J,1/F,2/M,3/A,4/M,5/J,6/J,7/A,8/S,9/O,10/N,11/D}{
			\pgfmathparse{(\year > 18 || \imonth >= 0) && (\year < 21 || \imonth < 2)}
			\ifnum \pgfmathresult > 0
				\draw (\year + \imonth/12,0)++(1/24,0) node [below] {\tiny \month};
					\draw (\year + \imonth/12,0) -- ++(0,-3pt); 
			\fi
		}
		\draw (\year,0) -- ++(0,-6pt); 
	}
	\draw (21+3/12,-15pt) node [left, inner ysep=0] {\small2021};
}
\makeatother
